Long-Term Optimal Delivery Planning for Replacing the Liquefied Petroleum Gas Cylinder

In the daily operation of liquefied petroleum gas service, gas providers visit customers and replace cylinders if the gas is about to run out. For a long time, frequent visits to customers were required because they could not determine the amount of remaining gas without a staff visit and observation. To solve this problem, smart meters are started to be employed to acquire gas consumption more frequently without visiting customers. In this study, we construct a system to optimize plans for cylinder replacement, and evaluate it with a large-scale field test. We propose an algorithm to create a replacement plan with three steps: estimating the replacement date, acquiring the customer list for replacement, and determining the delivery route. A more accurate estimation of the replacement date can be acquired with a smart meter, which is used for making a customer list for replacement. The formulation for making a customer list enables the gas provider to replace cylinders some days before the date when the gas would run out. It can suppress the concentration of replacements on certain days. Large-scale verification experiments were performed with more than 1,000 customers in Chiba prefecture in Japan. In the field test, the gas provider incorporated the system into its replacement operations. Moreover, the replacement plans developed by the proposed system were compared with that by the gas provider. Our system reduced the number of gas cylinders with gas shortage, the number of visits without replacement due to plenty of gas remaining, and the working duration per customer, which shows that our system benefits both gas providers and customers.

==> history/transportation_research_partC/Conclusion.tex <==
\section{Conclusion\label{sec:conclusion}}
In this paper, we tackle the efficient delivery planning for replacing gas cylinders with preventing the gas shortage and non-replacement visits.
To maintain a liquefied petroleum gas service, gas providers visit each customer to check the gas meter and replace the gas cylinder depending on the remaining gas.
For efficient delivery planning, it is essential to forecast future gas consumption and develop an efficient delivery plan.
Our main idea is to categorize all customers into three groups: high-risk, moderate-risk, and low-risk customers by focusing on the urgency to be out of gas. 
We construct an algorithm to maximize the number of delivery for moderate-risk customers while ensuring delivery to high-risk customers. 
Long-term optimal delivery planning is realized by achieving workload balancing per day. 

This algorithm is composed of three steps.
The first step is to forecast the daily gas consumption.
Recently, we can now monitor the daily gas consumption of each house owing to the development and spread of smart meters. 
However, approximately two-thirds of customers do not have such meters due to smart meters' limited installation. 
This paper proposes a method to forecast daily gas consumption when there is an imbalance in the data acquisition frequency.
The second step is to optimize the delivery list.
Because the results of demand forecasting are used as inputs to the optimization problem, we have to consider the influence of forecast error for making the delivery plan. 
In particular, when the forecast usage is much lower than the actual usage, a gas shortage will occur.
To tackle this issue, we propose a new method for calculating the risk of running out of gas by considering the forecast errors.
It enables us that the customer whose usages are difficult to be forecast is delivered earlier, which can prevent the gas shortages.
We then solve the optimization problems to acquire a delivery list for realizing the long-term optimal delivery plan.
Finally, we solve the delivery route optimization to obtain the visiting order and determine whether customers should be visited. 
To apply the real world's situation, we design the framework to obtain the solution in any case.

Numerical experiments are conducted with the real gas usage in Chiba prefecture.
Experiments for complementary algorithms and demand forecast experiment with the different settings of data missing assuming the real unpredictable situation.
Moreover, to evaluate demand forecast to utilize the delivery plan, we evaluate the demand forecast results per day.
The result of both experiments shows that the proposing method can more precisely complement and forecast compared to baselines.
A verification experiment for delivery planning conducts in Chiba prefecture in Japan shows the effectiveness of our algorithm.
We succeed in reducing the number of gas shortages, and our model can make an efficient delivery plan like the gas provider.
During the field test, where the gas provider incorporates our framework in their service, the proposed model records better evaluation metrics than the gas provider's delivery plan.

Our proposed model is a new generic framework for building an optimal vehicle routing plan based on the demand forecast. 
It consists of a complement algorithm, demand forecast, delivery list optimization, and delivery route optimization to realize a long-term optimal delivery plan by setting the priority. 
Because other industries have problems that can be solved by demand forecast and delivery planning, such as optimizing grocery delivery or oil delivery, our model has a significant potential to solve real-world delivery problems.


==> history/transportation_research_partC/DeliveryList/src/DLGreedy.tex <==
\subsubsection{Greedy Algorithm\label{sec:DLGreedy}}

The \emph{DLGreedy} algorithm is a simple algorithm that delivers as many moderate-risk customers as possible, in addition to high-risk customers.
Its procedure is summarized in Algorithm~\ref{alg:DLGreedy}.

\begin{algorithm}                      
\caption{\emph{DLGreedy} : Delivery Customers with High-risk Customers}         
\label{alg:DLGreedy}                          
\begin{algorithmic}   
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE Division of high-risk customer $\mathcal{C}_1^*, \ldots, \mathcal{C}_m^*$, Set of moderate-risk customer $\mathcal{C}^{'}$ ($n := |\mathcal{C}^{'}|$), and $r_{\alpha, C}(D)$ : value of risk function of customer $C$, where $\alpha$ and $D$ are hyperparameters
\ENSURE Delivery list $\mathcal{C}^{(1)}, \ldots, \mathcal{C}^{(m)}$
\STATE Sort $\mathcal{C}^{'}$ based on the value of risk function $r_{\alpha, C}(D)$
\STATE $\mathcal{C}_{-1} \gets \mathcal{C}'$
\FOR{$i = 1$ to $m$}
\STATE $\mathcal{C}^{(i)} \gets \mathcal{C}_i^*$
\FOR{$j = 1$ to $n$}
\STATE $C \gets C_j \in \mathcal{C}^{'}$
\IF{$C \notin \mathcal{C}_{-1}$ and $P(\mathcal{C}^{(i)} \cup \{C\})$ is True}
\STATE $\mathcal{C}^{(i)}  \gets \mathcal{C}^{(i)}  \cup \{C\}$
\STATE $\mathcal{C}_{-1} \gets \mathcal{C}_{-1} \setminus \{C\}$
\ENDIF
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> history/transportation_research_partC/DeliveryList/src/TruckConstraint.tex <==
\subsection{Capacity Constraint for the Truck Availability\label{sec:truck_constraint}}

This section describes the constraint that ensures that the selected customers can be delivered using a single truck for carrying all cylinders.
We have to consider both the weight and space constraints. 
There are two different sized cylinders in our setting: large and small.
% The medium and small cylinders can be regarded as being the same size.


\subsubsection{Weight Constraint}
As a simple constraint, the total weight of the cylinder must be smaller than the weight limitation, which can be easily written as a linear constraint.
Note that we take care of the cylinder weights by summing the weight of the gas and the weight of the cylinders.

Let $x_C$ be a binary variable gets 1 if and only if $C$ is selected in the delivery list.
Let $W$ be the maximum loading capacity of truck.
Then the weight constraint can be written as follows,
\begin{equation}
    \sum_{C} \rm{cn}^{(C)}\rm{cw}^{(C)}x_C \le W
\end{equation}


\subsubsection{Space Constraint}
The table indicates that the number of medium and small cylinders can be loaded under a large cylinder to be loaded.
An example is shown in Table~\ref{tab:space_limit}.


\begin{table}[htbp]
\begin{center}
\begin{tabular}{l||rrrrrrr}
Large cylinder                     & 34 & 33 & 32 & 31 & 30 & \ldots & 0   \\ \hline
Small cylinder & 0  & 1  & 3  & 4  & 5  & \ldots  & 45
\end{tabular}
\caption{The maximum number of small cylinders that can be loaded under the given number of large cylinders}
\label{tab:space_limit}
\end{center}
\end{table}

When we acquire the delivery list using an integer optimization problem, we have to transform the table into a linear constraint.
One of the ways to achieve this is to regard the table as a piecewise linear function. 
However, more variables are needed when we solve an integer optimization problem.
% Therefore, we would like to obtain an approximately linear function to limit the feasible region, which can be visualized in Figure \ref{fig:truckApprox}.
% Let $y = ax + b$ be the approximate target function, and $x, y$ be the number of large cylinders and the number of the small cylinders, respectively.
Therefore, as shown in Figure~\ref{fig:truckApprox}, we would like to obtain an approximately linear function $y \le a x + b$ to limit the number of small cylinders, where $x$ and $y$ be the number of large and small cylinders, respectively.
% In more detail, we consider a constraint limiting the number of the small cylinders $y$ by $y \le a x + b$, where $x$ is the number of large cylinders.
Let $\left(x_i, y\left(x_i\right)\right)$ be the pair of the number of large cylinders $x_i$ and the maximum number of small cylinders $y(x_i)$ under given $x_i$ as shown in Table~\ref{tab:space_limit}.
The number of the small cylinders  $y$ must be smaller than $y\left(x\right)$.
If $a$ and $b$ are set to satisfy $a x_i +b \le y\left(x_i\right)$ for all $i$, then we can have $y \le a x + b\le y\left(x\right)$.
In the following, we write $y\left(x_i\right)$ as $y_i$ for simplicity.



\begin{figure}
    \centering
    \includegraphics[width=15cm]{5:DeliveryList/figs/getTruckSpace_ApproxFunc.png}
    \caption{Approximation line covering all possible dots. Every circle dot indicates the limitation of maximum number of small cylinder to be loaded under given the number of large cylinder. Approximation line must not exceed every triangle marker.}
    \label{fig:truckApprox}
\end{figure}


The problem used to obtain the parameters $a, b$ of the linear function is as follows:
\begin{problem}
\label{prob:basic_approx_space_constraint}
(Basic : Approximating Space Constraints)
\[
\begin{aligned}
& \underset{a,b}{minimize} && \sum_{i}z_i \\
& && a x_i + b \le y_i && & \text{(1)}
\\
& && z_i \ge {\rm max}\{0, y_i - (a x_i + b)\}  && & \text{(2)}
\\
& && z_i \in \mathbb{Z}
\end{aligned}
\]
\end{problem}

The objective function indicates that the missing lattice point when using the linear function is as small as possible.
The first constraint ensures that the linear target function does not expand the feasible region regarding the space constraint.
The second constraint expresses the number of missing lattice points in the original feasible region, which is directly utilized for the objective function.

\begin{problem}
\label{prob:proposed_approx_space_constraint}
(Proposed : Approximating Space Constraints)
\[
\begin{aligned}
& \underset{a,b}{minimize} && \sum_{i}z_i \\
& && a x_i + b \le y_i + 1 - \varepsilon \ (1 \gg \varepsilon > 0) && & \text{(1)'}
\\
& && z_i \ge {\rm max}\{0, y_i - (a x_i + b)\}  && & \text{(2)}
\\
& && z_i \in \mathbb{Z}
\end{aligned}
\]
\end{problem} 

We can relax one constraint by keeping the original dots.
The results are shown in Figure~\ref{fig:truckApprox}.
The original one and updated lines are indicated in the red line and blue line, respectively.
When we change the formulation from Problem~\ref{prob:basic_approx_space_constraint} to Problem~\ref{prob:proposed_approx_space_constraint}, the number of missing dots decrease from 46 to 22.

Let $a^*, b^*$ be the optimal solutions of Problem~\ref{prob:proposed_approx_space_constraint}, and
let the customers with large cylinder be $\mathcal{C}_{\rm Large}$.
Then the space constraint can be written as follows,
% \begin{align*}
%     \sum_{C \in \mathcal{C}_{\rm Large}} {\rm cn}^{(C)}x_C &= 45t_2  \\
%     \sum_{C \in \mathcal{C}_{\rm Large}^{\mathsf{c}}} {\rm cn}^{(C)}x_C &\le b^{*}\times t_1 + (45 a^{*} + b^*) \ t_2  \\
%     t_1 + t_2 &= 1\\
%     t_1, t_2 &\in [0,1]
% \end{align*}

% \begin{align*}
% \left\{
% \begin{array}{llll}
%     \sum_{C \in \mathcal{C}_{\rm Large}} {\rm cn}^{(C)}x_C = 35t_2  \\
%     \sum_{C \in \mathcal{C}_{\rm Large}^{\mathsf{c}}} {\rm cn}^{(C)}x_C \le b^{*}\times 45.99t_1 + (35 a^{*} + b^*) \ t_2  \\
%     t_1 + t_2 = 1\\
%     t_1, t_2 \in [0,1]
% \end{array}
% \right.
% \end{align*}


\begin{align*}
\left\{
\begin{array}{lll}
    \left(\sum_{C \in \mathcal{C}_{\rm Large}^{c}} {\rm cn}^{(C)}x_C\right)
    \le 
    a^{*} \left(\sum_{C \in \mathcal{C}_{\rm Large}} {\rm cn}^{(C)}x_C\right) + b^{*}\\
    \left(\sum_{C \in \mathcal{C}_{\rm Large}} {\rm cn}^{(C)}x_C\right) \le M_{{\rm Large}}\\
    % \sum_{C \in \mathcal{C}_{\rm Small}} {\rm cn}^{(C)}x_C \le 45\\
    x_C \in \{0, 1\}
\end{array}
\right.
\end{align*}
, where
$x_C =
    \left\{
    \begin{array}{ll}
        1 & \text{Customer} \ C \ \text{is selected in the delivery list.} \\
        0 & \text{o.w.}
    \end{array}
    \right.$
    , and $M_{{\rm Large}}$ is the maximum number of the large cylinders carried on a truck.
% .
% }
% \color{black}

==> history/transportation_research_partC/DeliveryList/src/anchor_based.tex <==
\begin{algorithm}                      
\caption{Divide High-Risk Customer based on Anchor-based Algorithm}         
\label{alg2}                          
\begin{algorithmic}   
\label{alg:anchor-based}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE High-risk customers $\mathcal{C}^*$, distance function $d$
and truck feasible function $P$
\ENSURE The division of high-risk customers $\mathcal{C}_1^*, \ldots, \mathcal{C}_k^*$
\IF{$P(\mathcal{C}^*)$ is True}
\STATE $\mathcal{C}_1^* \gets \mathcal{C}^*$
\RETURN
\ELSE
\STATE $k \gets 2$
\STATE Feasible $\gets$ False
\WHILE{Feasible is False}
\STATE $\mathcal{C}_1^*,\ldots,\mathcal{C}_k^*, {\rm Feasible} \gets subBinPacking(\mathcal{C}^*, k) \quad$ (see Algorithm~\ref{alg:subBinPacking})
\STATE $k \gets k + 1$
\ENDWHILE
\ENDIF
\end{algorithmic}
\end{algorithm}


\begin{algorithm}                      
\caption{(subBinPacking) Search the Division under Given the Number of Trucks}         
\label{alg:subBinPacking}                          
\begin{algorithmic}  
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE High-risk customers $\mathcal{C}^*$, distance function $d$
, truck feasible function $P$ and number of truck $k$
\ENSURE The division of high-risk customers $\mathcal{C}_1^*, \ldots, \mathcal{C}_k^*$, and feasibility
\STATE $\hat{\mathcal{C}} \gets \underset{\mathcal{C} \subset \mathcal{C}^*, |\mathcal{C}| = k}{\rm argmax} \ \underset{C,C' \in \mathcal{C}, C \neq C'}{\rm min} d(C,C')$
\STATE $i \gets 1$
\FOR{$C \in \hat{\mathcal{C}}$}
\STATE $\mathcal{C}_i^* \gets \{C\}$
\STATE $i \gets i + 1$
\ENDFOR
\STATE $\bar{\mathcal{C}} \gets Sort(\mathcal{C}^* \setminus \hat{\mathcal{C}})$ based on the function $g(C) := V_{\hat{C} \in \mathcal{C}^*}\left[\min\left(d(C,\hat{C}), d(\hat{C}, C)\right)\right]$
\STATE Feasible $\gets$ True
\FOR{$\bar{C} \in \bar{\mathcal{C}}$}
\STATE Sort TruckList based on the distance between target customer $\bar{C}$ and each division $\mathcal{C}_1^*, \ldots, \mathcal{C}_k^*$
\STATE Load $\gets$ False
\FOR{$j$ in TruckList}
\IF{$P(\mathcal{C}_j^* \cup \{\bar{C}\})$ is True}
\STATE $\mathcal{C}_j^* \gets \mathcal{C}_j^* \cup \{\bar{C}\}$
\STATE Load $\gets$ True
\STATE \textbf{break}
\ENDIF
\ENDFOR
\IF{Load is False}
\STATE Feasible $\gets$ False
\STATE \textbf{break}
\ENDIF
\ENDFOR
\RETURN $\mathcal{C}_1^*, \ldots, \mathcal{C}_k^*$, Feasible
\end{algorithmic}
\end{algorithm}

==> history/transportation_research_partC/DeliveryList/src/divide_trip.tex <==
\subsection{Trip Division for High-risk Customers\label{sec:divideTrip}}

% Under this situation, we must repeat how the staff leaves the delivery base when visiting the customers to exchange their cylinders.
We call a {\it trip} the process by which the truck leaves the base, delivers the gas cylinders, and returns to the base.
When we have a considerable number of customers to deliver in a single day, it becomes impossible to deliver to all of them using only one truck.
Therefore, many trips are needed to complete the delivery to the high-risk customers.
In this chapter, we aim to obtain the optimal division of high-risk customers.

The reasonable division of high-risk customers satisfies the following three conditions.
\begin{enumerate}
    \item The number of divisions is as small as possible.
    \item Each subset of high-risk customers is gathered in terms of location.
    \item Each subset of high-risk customers satisfies the truck constraint described in Section~\ref{sec:truck_constraint}. 
\end{enumerate}

To tackle the problems, we propose two algorithms.

\subsubsection{Updated Next-Fit Algorithm}
We focus on the first condition, which is similar to the bin packing problem.
The well-known algorithms for bin packing are the next-fit algorithm, first-fit algorithm, and first-fit decreasing algorithm.
When processing the next item using the next-fit algorithm, we check whether it fits in the same bin as the last item. 
If it does not fit, we prepare a new bin.
With the first-fit algorithm, when processing the next item, the previous bins are scanned in order, and the item is placed in the first bin that fits. 
We start a new bin only if it does not fit in any of the existing bins. 
With the first-fit decreasing algorithm, we first sort the input sequence and place the large items. 
After that, we apply the first fit algorithm for picking the items.

To achieve the second condition, we sort the customers based on their geospatial information.
After that, we apply the next-fit algorithm. 
The reason for not applying the first-fit algorithm and the first-fit decreasing algorithm is described later.
% The proposed algorithm is summarized as follows:
The proposed algorithm is summarized in Algorithm \ref{alg:updated_NF}.

\input{5:DeliveryList/src/updated_NF}

Next, we demonstrate why the next-fit algorithm is more suitable than the first-fit algorithm and the first-fit decreasing algorithm.
The main reason for such suitability is that this algorithm is harmful under the second condition. 
It is because there is a difference between the number and size of the cylinder for each customer.
% We show more details of this along with the reason in the following.


In short, the first algorithm is summarized as follows,
\begin{enumerate}
    \item We search for the two customers whose distance is longest among high-risk customers.
    % \item We make a projection of all customers along the line between the two customers and index them, aligning the projection.
    \item We sort the customers by relative positions among the customer, and the two customers picked up in the first step.
    \item We apply the next-fit algorithm with the sorted customers using the above approach.
\end{enumerate}

\subsubsection{Find Anchor and Numbering based on the Variance of the Distance to the Anchors (FAVA)}

We point out the weakness of the first algorithm and propose another algorithm for dividing high-risk customers.
The first point is the geospatial variance.
Because each customer is ordered after being projected, vector rejections are ignored, as shown in the left part of Figure~\ref{fig:weakness_NF}.
The second weakness is derived from the next-fit algorithm.
In the next-fit algorithm, each item is first checked to be loaded from the truck where the last item is loaded.
Even if the distance between the last customer and the current customer is far, there is a chance that they belong to the same {\it trip}, as shown in the right part of Figure~\ref{fig:weakness_NF}.

\begin{figure}
    \centering
    \includegraphics[width=12cm]{5:DeliveryList/figs/problem_NF.png}
    \caption{Weakness of Algorithm~\ref{alg:updated_NF}. When customers have the same shape, it indicates that they belong to the same trip.}
    \label{fig:weakness_NF}
\end{figure}

Based on these investigations, we propose another algorithm.
First, we extract customers as anchor customers whose number is the same as the number of trucks. 
The anchor customers are the first consumers to be loaded onto each truck. 
They should be as far from each other as possible.
Next, we consider splitting the non-anchor customers. 
There are two types of customers: those that will take a certain distance to load onto any truck and those extremely close to the anchor and will cost more if not loaded onto a specific truck.
Therefore, we sort the non-anchor customers based on the variance of their distances to the anchors and determine their affiliation from the customers with the largest distance variance.
We check each truck's availability in order of the distance between the customer and the division for each customer.

The first weakness of the last algorithm corresponds to the indication of the anchor-customer and the ordering customers based on the variance between the target customer and the current divisions.
The second weakness is improved by the searching method applied after each customer is chosen without considering the projection.
The details of the algorithm are summarized in Algorithms~\ref{alg:anchor-based} and~\ref{alg:subBinPacking}.

\input{5:DeliveryList/src/anchor_based}

%Simple example of the output of proposed two algorithms is demonstrated in figure xxx.

In the next section, we demonstrate the acquisition of the delivery list.
In Sections~\ref{sec:DLGreedy},~\ref{sec:maxRisk},~\ref{sec:minBB}, and~\ref{sec:multiBB} we utilize both the number of divisions and each subset of high-risk customers.

==> history/transportation_research_partC/DeliveryList/src/dl_main.tex <==
\section{Delivery List Optimization\label{sec:delivery_list}}

This chapter describes the extraction of high-risk and moderate-risk customers and the acquisition of target customers to be delivered when considering reasonable constraints such as truck loading constraints.

\input{5:DeliveryList/src/risk_func}

\input{5:DeliveryList/src/TruckConstraint}

\input{5:DeliveryList/src/divide_trip}

\subsection{Proposed Models to Acquire the Optimal Delivery List\label{sec:DLmodel}}
Given the high- and moderate-risk customers, we would like to acquire the delivery list.

\input{5:DeliveryList/src/DLGreedy}

\input{5:DeliveryList/src/maxRisk}

\input{5:DeliveryList/src/minBB}

\input{5:DeliveryList/src/multiBB}

\subsection{Post Processing}
After the delivery list is provided, we extract the lowest gas rate for each trip. 
Then, a minor trip ID is given in the order of its value.
A user of this framework can input the maximum number of trips.
When the number of trips exceeds the input maximum number of trips, we extract the number of input maximum number of trips based on the ID of trips.


==> history/transportation_research_partC/DeliveryList/src/maxRisk.tex <==
\subsubsection{Maximize the Summation of Risk of Gas Shortage\label{sec:maxRisk}}

\paragraph{Motivation}

As the basic concept of our approach, we deliver as many moderate-risk customers as possible while ensuring the delivery of high-risk customers.
We consider deliveries to moderate-risk customers during the process of making deliveries to high-risk customers.
These deliveries do not lead to extremely inefficient delivery routes.
Moreover, we would like to visit those who have a higher risk compared to other moderate-risk customers.
We call this model the {\it maxRisk} model.


\paragraph{Preprocessing}

We extract moderate-risk customers such that they do not hinder the delivery route.
Because our model pursues delivery to high-risk customers, selecting moderate-risk customers along the way to high-risk customers is a reasonable approach.
To realize this concept, we prepare ellipses whose focuses are on high-risk customers, and we extract the moderate-risk customers included in the ellipse.
% In an ellipse, traced by a point moving in a plane so that the sum of its distances from two other points is constant.
% It can be regarded as the delivery to moderate-risk customers included in the ellipse does not make a delivery route too long.
% Because in an ellipse, a point moving in such a way that the sums of its distances from two fixed points are a constant, every
Based on the definition of an ellipse, delivering one moderate-risk customer on the ellipse in the middle of the delivery to two essential customers does not change the total distance heavily.
% Let $C_0$ and $C_1$ be the high-risk customers, and we consider whether the customer $C$ is included in the ellipse whose focuses are $C_0$ and $C_1$.
% When we denote $l : \mathcal{C} \times \mathcal{C} \to \mathbb{R}$ the distance function between two points and prepare the hyperparameter $\gamma$, we can judge the $C$'s inclusion of ellipse with following conditions,
% \begin{equation}
%     C \in EL_{C_0, C_1} \iff  \le l(C,C_1) + 
% \end{equation}
Let $C_0$ and $C_1$ be the high-risk customers, and we consider whether the customer $C$ is included in the ellipse whose focuses are $C_0$ and $C_1$.
Let $l$ be the summation of the distances between a point on the ellipse, and the two focuses $C_0$ and $C_1$.
When we insert $C$ between the deliveries $C_0$ and $C_1$, the increased distance is less than $l$.
% By changing $l$, we can adjust the customers to be input the {\it maxRisk} problem.
% The distance increased by addition of $C$ between $C_0$ and $C_1$ is about less than $l$.
Therefore, it does not make a delivery route too long because these visits can be done by on the way of delivery for high-risk customers.
% allowing two high-risk customers to be visited in a row.
% Let $C_0$ and $C_1$ be the high-risk customers, and we consider whether the customer $C$ 
% We can judge the customer in the 
% In the experiment, we prepare $k (< |\mathcal{C}^*|)$ ellipses under given pair of high-risk customers.

The above procedure is written mathematically as follows.
Under given two high-risk customers, $C_0$ and $C_1$, let an ellipse whose focuses are $C_0$ and $C_1$ as $EL_{C_0, C_1}$.
When we denote the $k$-nearest neighbor high-risk customers from $C$ as $N_C(k) \subset \mathcal{C}^*$, the extracted moderate-risk customers to be input the Problem~\ref{prob:maxRisk}, $\mathcal{C}^*_{\rm candidate}$ can be written as follows
\begin{equation}
    % \mathcal{C}^*_{candidate} = \{C \in \mathcal{C}^{'} |  
    % C \in \cup_{C_0 \in \mathcal{C}^*}\cup_{C_1 \in N_{C_0}(k)} EL_{C_0,C_1} \}
    \mathcal{C}^*_{candidate} = \{C \in \mathcal{C}^{'} | \exists (C_0, C_1) \in \mathcal{C}^* \times N_{C_0}(k) \ {\rm such} \ {\rm that} \ C {\rm~is} \ {\rm in} \ EL_{C_0, C_1} \}
\end{equation}

When a moderate-risk customer is included in an ellipse, the customer is picked up and input into the Problem~\ref{prob:maxRisk}.

\paragraph{Formulation}

We denote the variable used in the maxRisk model as follows,
\begin{enumerate}
\item Variables
    \begin{itemize}
        \item $x_C=
        \left\{
            \begin{array}{ll}
                1 & \text{Customer} \ C \ \text{is selected in the delivery list.} \\
                0 & \text{o.w.}
            \end{array}
        \right.$
    \end{itemize}
\item Constants
    \begin{itemize}
        \item $r_{\alpha, C}(D)$ : The value of risk function of customer $C$ after $D$ days with threshold of remaining gas $\alpha$.
    \end{itemize}
\end{enumerate}

We formulate this problem as an integer optimization problem in Problem~\ref{prob:maxRisk}.
% Before notating the formulation, we describe how to extract the moderate-risk customers.
% The extracted moderate-risk customers should not be pained for making an efficient delivery plan while delivering to high-risk customers.
% To realize the motivation, we utilize the elliptic curve to extract moderate-risk customers.

\begin{problem}
\label{prob:maxRisk}
maxRisk: Acquiring the Maximum Summation of Risk for Gas Shortage
\[
\begin{aligned}
& \underset{x}{\rm maximize} && \sum_{C\in \mathcal{C}^{'}}r_{\alpha, C}(D)^2 x_C \ (D : \text{target date to make the delivery list}) \\
& && x_C = 1 \ (\forall C \in \mathcal{C}^*) && & \text{(1)}
\\
& && x_C \in \{0,1\} \ (\forall C \in \mathcal{C}^*_{\rm candidate}) && & \text{(2)}
\\
& && \text{(Truck Capacity constraint and weight constraint explained in Section~\ref{sec:truck_constraint})}
\end{aligned}
\]
\end{problem}

We describe the reason for multiplying one’s risk function in the objective function.
When there are two options for extracting moderate-risk customers, we would like to obtain the set where the highest customer exists.
To realize this motivation, we prepare a convex function for coefficients of the objective function.
In our experiment, we input the squared value of the risk function to the problem.
The following proposition supports the validity of the above statement.


\begin{prop}
Given $w \le x \le y \le z \ (w,x,y,z \in \mathbb{R})$ such that $w + z = x + y$ and convex function $f : \mathbb{R} \to \mathbb{R}$, the following inequality is satisfied:
\begin{equation*}
    f(w) + f(z) \ge f(x) + f(y)
\end{equation*}
\end{prop}

\noindent
\textbf{Proof of Proposition 1}

\begin{proof}

\begin{equation*}
    \lambda := \frac{x-w}{z-w} \quad \mathit{satisfies} \quad \lambda \in [0,1] \quad \mathit{and} \quad x = (1-\lambda) w + \lambda z.
    % \lambda = \frac{b-a}{d-a} \in [0,1] \quad s.t. \quad b = \lambda a + (1-\lambda) d
\end{equation*}
From the condition $w+z=x+y$, we obtain 
$y = \lambda w + (1 - \lambda) z$.\\
Based on the definition of convex function, following two inequalities are satisfied,
\begin{eqnarray}
\lambda f(w) + (1-\lambda) f(z) \ge
f\left(\lambda w + (1-\lambda) z\right) = f(x) \label{f_b}\\
(1-\lambda) f(w) + \lambda f(z) \ge
f\left((1-\lambda)w + \lambda z\right) = f(y) \label{f_c} 
\end{eqnarray}
By summing up (~\ref{f_b}) and (~\ref{f_c}), we acquire
\begin{equation*}
    f(w) + f(z) \ge f(x) + f(y)
\end{equation*}
\qed
\end{proof}

The proposition indicates that when two pairs of candidates are delivered, the model selects the pair with the highest value of risk function.
When the value of risk functions of customer $C_w, C_x, C_y, C_z$ are $w,x,y,z$ ($w \le x\le y\le z$), respectively, and $w+z = x+y$ is satisfied, we support that the delivery to the customers $C_w$ and $C_z$ compared $C_x$ and $C_y$.

==> history/transportation_research_partC/DeliveryList/src/minBB.tex <==
\subsubsection{Minimize the Delivery Area using Bounding Box\label{sec:minBB}}

\paragraph{Motivation}

We obtain a rectangle that covers the delivery targets, i.e., both high- and moderate-risk customers.
We call this model the {\it minBB} model.


\begin{figure}[htbp]
\begin{center}
\includegraphics[width=10cm]{5:DeliveryList/figs/minBB.png}
\caption{Motivation of {\it minBB} model}
\end{center}
\label{fig:minBB}
\end{figure}

\paragraph{Formulation}

\begin{enumerate}
\item Variables
    \begin{itemize}
        \item $x_C^i =
        \left\{
            \begin{array}{ll}
                1 & \text{Customer} \ C \ \text{is selected in the delivery list with tripID} i \text{.} \\
                0 & \text{o.w.}
            \end{array}
        \right.$
        \item $v_{lb}^i , v_{ub}^i , w_{lb}^i , w_{ub}^i  \in \mathbb{R}$ : the variables to represent a square covering the delivery area. 
    \end{itemize}
% \item Constraints
\end{enumerate}

The formulation of the {\it minBB} model is shown in Problem~\ref{prob:minBB}.
Constraints 1 to 4 ensures that the square covers the customers to be delivered.
Constraint 5 enables us to deliver to high-risk customers consistently.
If it were not for constraint 6, the output rectangle always covers only high-risk customers.
Constraint 7 ensures us that every customer cannot select more than one trip.
Therefore, we have to prepare the lower bound of the number of deliveries $LB$.

\begin{problem}
\label{prob:minBB}
minBB: Obtaining the Smallest Rectangle which Covers the Target Customers
\[
\begin{aligned}
& \underset{x^i , v_{lb}^i , v_{ub}^i , w_{lb}^i , w_{ub}^i }{\rm minimize} && \sum_{i}(v_{ub}^i -v_{lb}^i ) + (w_{ub}^i -w_{lb}^i )
\\
& \text{subject to} && {\rm lat^{(C)}} x_C^i \le w_{ub}^i  (\forall C \in \mathcal{C}' \cup \mathcal{C}^*) && & \text{(1)}
\\
& && {\rm lat^{(C)}} x_C^i  + (1-x_C^i )M_w \ge w_{lb}^i  \ (\forall C \in \mathcal{C}' \cup \mathcal{C}^*) && & \text{(2)}
\\
& && {\rm lon^{(C)}} x_C^i  \le v_{ub}^i  \ (\forall C \in \mathcal{C}' \cup \mathcal{C}^*) && & \text{(3)}
\\
& && {\rm lon^{(C)}} x_C^i  + (1-x_C^i )M_v \ge v_{lb}^i  \ (\forall C \in \mathcal{C}' \cup \mathcal{C}^*) && & \text{(4)}
\\
& && \sum_{i} x_C^i  = 1 \ (\forall C \in \mathcal{C}^*, \forall i) && & \text{(5)}
\\
& && \sum_{C \in \mathcal{C}' \cup \mathcal{C}^*} x_C^i  \ge LB \ (LB \in \mathbb{N}) && & \text{(6)}
\\
& && \sum_{i} x_C^i \le 1 \ (\forall C, \forall i) && & \text{(7)}
\\
% & && w_{lb} \le w_h \le w_{ub} \ (\forall h \in H^*) && & \text{(7)}
% \\
% & && v_{lb} \le v_h \le v_{ub} \ (\forall h \in H^*) && & \text{(8)}
% \\
& && \text{(Truck Capacity constraint and weight constraint explained in Section~\ref{sec:truck_constraint})}
\\
& && M_w := \underset{C}{\rm max} \ {\rm lon^{(C)}}, M_v := \underset{C}{\rm max} \ {\rm lat^{(C)}}
\end{aligned}
\]
\end{problem}

==> history/transportation_research_partC/DeliveryList/src/multiBB.tex <==
\subsubsection{Minimize the Delivery Area for Multiple Dates\label{sec:multiBB}}

\paragraph{Motivation}

The {\it maxRisk} (Section~\ref{sec:maxRisk}) and {\it minBB} (Section~\ref{sec:minBB}) algorithms are not focused on multiple-days.
When we obtain the delivery route sequentially, it may be harmful to the future delivery area.
In other words, the delivery area becomes large, as shown in the bottom-left image in Figure~\ref{fig:multiBB}.
To prevent such occurrences, we would like to acquire a multi-day delivery list at the same time.
We call this model the {\it multiBB} model.
The basic concept of {\it multiBB} is the same as that of {\it minBB}, which acquires a rectangle covering the delivery targets.


\begin{figure}
    \centering
    \includegraphics[width=12cm]{5:DeliveryList/figs/multiBB.png}
    \caption{Motivation of {\it multiBB} model}
    \label{fig:multiBB}
\end{figure}

\paragraph{Formulation}

\begin{enumerate}
\item Variables
    \begin{itemize}
        \item $x_C^{D, i}=
        \left\{
            \begin{array}{ll}
                1 & \text{Customer} \ C \ \text{is selected in the delivery list with tripID ${i}$ in date $D$} \\
                0 & \text{o.w.}
            \end{array}
        \right.$
        \item $v_{lb}^{D,i}, v_{ub}^{D,i}, w_{lb}^{D,i}, w_{ub}^{D,i} \in \mathbb{R}$ : the variables to represent a square covering the delivery area for tripID $i$ in date $D$.
    \end{itemize}
\end{enumerate}

For the {\it minBB} formulation, we prepare the lower bound of the number of cylinders to be delivered for each {\it trip} in the constraint.
We prepare the number of rectangles as the same as the output of dividing the high-risk customer.
The formulation of the {\it multiBB} model is shown in Problem~\ref{prob:multiBB}.
We attempt to minimize the maximum value of the summation of the edges in a rectangle.
Constraints 1 – 4 ensure that the rectangle covers the customers to be delivered.
Constraint 5 enables us to deliver to high-risk customers consistently.
If it were not for constraint 5, the output rectangle would always cover only high-risk customers.
Therefore, we have to prepare the lower bound of the number of deliveries $LB$.
Constraint 6 ensures that a high-risk customer during the target days will be delivered at least once.
Every customer can belong to at most one trip each day, which is ensured by constraint 7.

When the problem is infeasible, the situation is derived from constraint 6 because the target customers are less than the lower bound.
Under this situation, we reduce the lower bound by 1 and solve the problem repeatedly.


\begin{problem}
\label{prob:multiBB}
{\it multiBB}: Obtaining Small Rectangle which Covers the Target Customers for Multiple Days' Delivery Plan
\[
\begin{aligned}
& \underset{x, v_{lb}, v_{ub}, w_{lb}, w_{ub}, L}{\rm minimize} && \underset{D \in \mathcal{D}, i}{\rm max}L^{D, i}
\\
& \rm{subject \ to} && {\rm lon^{(C)}} x_C^{D, i} \le w_{ub}^{D, i} \ (\forall C, i, D) && & \text{(1)}
\\
& && {\rm lon^{(C)}} x_C^{D, i} + \left(1-x_C^{D, i}\right)M_w \ge w_{lb}^{D, i} \ (\forall C \in \mathcal{C}' \cup \mathcal{C}^*) && & \text{(2)}
\\
& && {\rm lat^{(C)}} x_C^{D, i} \le v_{ub}^{D, i} \ (\forall C \in \mathcal{C}' \cup \mathcal{C}^*) && & \text{(3)}
\\
& && {\rm lat^{(C)}} x_C^{D, i} + \left(1-x_C^{D, i}\right)M_v \ge v_{lb}^{D, i} \ (\forall C \in \mathcal{C}' \cup \mathcal{C}^*) && & \text{(4)}
\\
& && \sum_{C \in \mathcal{C}' \cup \mathcal{C}^*} x_C^{D, i} \ge LB&& & \text{(5)}
\\
& && \sum_{i \in \mathcal{D}^{'}_C \cup \mathcal{D}^{*}_C}{x_C^{D, i}} \ge 1 \ \left(\forall C \in \mathcal{C} {\rm ~s.t.~} \mathcal{D}^{*}_C \neq \emptyset \right) && & \text{(6)}
\\
& && \sum_{i} x_C^{D, i} \le 1 \ (\forall C, D) && & \text{(7)}
\\
& && \text{(Truck Capacity constraint and weight constraint explained in Section~\ref{sec:truck_constraint})}
\\
& && M_w := \underset{C}{\rm max} \ {\rm lon^{(C)}}, M_v := \underset{C}{\rm max} \ {\rm lat^{(C)}}
\\
& && L^{D, i} = \left(v_{ub}^{D, i}-v_{lb}^{D, i}\right) + \left(w_{ub}^{D, i}-w_{lb}^{D, i}\right) 
\\
% & && \mathcal{D}^*_C = \underset{C \in \mathcal{C}^*({D})}{\rm argmin}\mathcal{D} 
& && \mathcal{D}^*_C = \rm{min}\{D \in \mathcal{D} | C \in \mathcal{C}^*(\mathcal{D}) \}  \ (\forall C)
\\
& && \mathcal{D}^{'}_C = \{D \in \mathcal{D} | C \in \mathcal{C}^{'}({D})\} \  (\forall C)
\end{aligned}
\]
\end{problem}


\paragraph{Post processing}

Constraint 6 ensures deliveries to customers who will become high-risk customers in a few days. 
There is no guarantee that deliveries will be made on these days to such customers.
Therefore, it is necessary to upgrade them to high-risk customers. 
The last day on the delivery list is selected for high-risk customers, even if deliveries are made on moderate-risk days. (see Figure~\ref{fig:upgrade})

\begin{figure}[htbp]
    \centering
    \includegraphics[width=15cm]{5:DeliveryList/figs/upgrade.png}
    \caption{Upgrade to the high-risk customer}
    \label{fig:upgrade}
\end{figure}

==> history/transportation_research_partC/DeliveryList/src/risk_func.tex <==
\subsection{Estimating the Risk for Gas Shortage\label{sec:risk_func}}
\begin{figure}
    \centering
    \includegraphics[width=15cm]{5:DeliveryList/figs/overall_risk_ver6.png}
    \caption{The process of obtaining the risk function}
    \label{fig:overall_risk}
\end{figure}

In Section~\ref{sec:demand_forecast}, we discuss the demand forecast method per meter.
Because some meters share the same customer's cylinders, we have to aggregate the forecast results per meter to obtain the forecast result per customer.
The risk function is proposed by considering the forecasting gas usage and forecasting accuracy to determine the emergency of a cylinders' replacement.
Based on the risk function, we extract high-risk customers and moderate-risk customers, which are candidates of the delivery, which is the goal of this section.

% Since some meters share the same customer's cylinders; we have to define the risk function per customer based on the prediction per meter.
We introduce the definition of the proposed risk function mathematically, and the procedure is illustrated in Figure~\ref{fig:overall_risk}.
We assume that the forecast error of each meter per day independently follows a normal distribution.
The daily gas consumption of one meter does not influence that of other meters.
% Moreover, most of the gas usages is used for daily life, and it is difficult to consume the gas usages the day before or tomorrow in advance.
First, we sum up the forecast gas usages and unbiased variances based on the forecast accuracy for the same customer's meters per day.
Then, we calculate the cumulative summation to obtain the cumulative gas usages and unbiased variances for a customer.
Based on this information, we define the risk function as the probability of falling below a specific gas rate. 
% The integrated value can be used to calculate the probability distribution function.
Subsequently, we determine whether the customer belongs to high-risk customers by being given the threshold for the risk function.

% We describe the risk function mathematically.
Let $D$ be today's date, and we pick up one customer $C$.
Let $x_i^{(M)} \sim \hat{p}_i^{(M)} = N\left(\widehat{\rm du}_{{\rm D}+i}^{(M)}, \widehat{\rm dv}_{{\rm D}+i}^{(M)} \right)$ be the probability distribution function of the forecasting the gas consumption in $i$-th day after $D$ for the meter $M$~($i \in [0,n_f-1] \cap \mathbb{Z}$). 
$\widehat{\rm du}_{{\rm D}+i}^{(M)}$ and $\widehat{\rm dv}_{{\rm D}+i}^{(M)}$ are the output of forecasting gas consumption and an unbiased variance based on the accuracy for forecasting gas consumption, respectively.
Based on the assumption that the error of gas usage of each meter that shares the same cylinder per day independently follows the normal distribution, we can apply the reproductive property of normal distribution for $\hat{p}_i^{(M)}$.
Therefore, we can define $X_i^{(C)} \sim p_i^{(C)}  = N\left(\mu_{{\rm mD}(D,i)}^{(C)}, \sigma_{{\rm mD}(D,i)}^{(C)}\right)$
$\left(\mu_{{\rm mD}(D,i)}^{(C)} := \sum_{M \in C}\widehat{\rm du}_{{\rm D}+i}^{(M)}, \sigma_{{\rm mD}(D,i)}^{(C)} := \sum_{M \in C}\widehat{\rm dv}_{{\rm D}+i}^{(M)} \right)$ be the probability distribution function of the forecasting the gas consumption in $i$-th day after $D$ for the apartment $C$.
% $\widehat{\rm du}_{{\rm D}+i}^{(C)}$ and $\widehat{\rm dv}_{{\rm D}+i}^{(C)}$ is also obtained by the output of forecasting gas consumption and an unbiased variance based on the accuracy for forecasting gas consumption, respectively.
Based on the assumption that the gas usage of each customer per day independently follows the normal distribution, we can also apply the reproductive property of normal distribution for $p_i^{(C)}$.
Then, the function that represents the amount of gas consumption $\bar p_{n_f}^{(C)}$ for $n_f$ days can be written as follows,
\begin{equation*}
    \bar p_{n_f}^{(C)} = N\left(\sum_{i=0}^{n_f - 1} \mu_{{\rm mD}(D,i)}^{(C)}, \sum_{i=0}^{n_f -1} \sigma_{{\rm mD}(D,i)}^{(C)}\right)
\end{equation*}

Let $z, z_\alpha$ be the current remain gas and the amount of gas when the remaining gas rate is equal to $\alpha$, respectively.
Then, we can describe the temporary risk function $\hat r_{\alpha, C} : \mathcal{D} \to [0,1]$ which returns the probability that the remaining gas level will be less than $\alpha$.
\begin{eqnarray*}
\hat r_{\alpha,C}(D) &:=& P\left(x \ge z^{(C)} - z_\alpha^{(C)}\right) \\
&=& 1 - P\left(x \le z^{(C)} - z_\alpha^{(C)}\right) \\
&=& 1 - \int_{-\infty}^{z^{(C)}-z_\alpha^{(C)}} \bar p_{D}^{(C)}(x)dx
\end{eqnarray*}

In reality, every customer cannot be replaced the gas cylinder due to the customer's absence or staff's vacations.
Then, we prepare $I^{(\rm avail)}_{C} :  \mathcal{D} \to \{0,1\}$ as the indicator function representing the availability of customer $C$.

By considering the $\hat r_{\alpha, C}$ and the availability of the customers and staff, we can finally define the risk function $r_{\alpha, C} :  \mathcal{D} \to [0,1]$  as follows,
\begin{equation}
    r_{\alpha, C}(D) := \hat r_{\alpha, C}(D^*) \ \left(D^* = {\rm min}\ \{ D' \in \mathcal{D} \mid D' \ge D, I^{(\rm avail)}_{C}({\rm mD} (D', 1))=1 \} \right)
\end{equation}

When we determine the threshold of the risk function, we can categorize the customers into high-risk customers, moderate-risk customers, and low-risk customers.
In this case, we prepare two risk functions with different parameters for the remaining gas rate: $\alpha$ and $\beta$.
When we prepare the thresholds $q^*, q'$, the high-risk customers and the moderate-risk customers on day $D$ can be written as follows:

\begin{itemize}
    \item High-risk customers $\mathcal{C}^*(D) := \{C \in \mathcal{C} \mid q^* < r_{\alpha, C}(D) \}$
    \item Moderate-risk customers $\mathcal{C}^{'}(D) := \{C \in \mathcal{C} \setminus \mathcal{C}^*(D) \mid q' < r_{\beta, C}(D) \}$
\end{itemize}

We simply write high-risk customers and moderate-risk customers as $\mathcal{C}^*$ and $\mathcal{C}^{'}$ when we do not have to take care of the $D$.
When we calculate the delivery plan using the above definition, the number of moderate-risk customers sometimes be relatively small.
To prepare more candidate delivery customers as moderate-risk customers, we set a parameter $D'$ and ensure that the customer belongs to a moderate-risk customer for $D'$ days before becoming a high-risk customer.
We call $D'$ as a {\it look back dates}.
When we set the hyperparameter $q^*$ to be 0.5, we only focus on whether the average value of the distribution is above the threshold of the gas rate when we determine the high-risk customer, which the following proposition can support.

\begin{prop}
Given usage distribution $\bar{p}_{n_f}^{(C)}$, if parameter $q^*$ is set to 0.5, then it holds that customer $C$ is satisfied to be a high-risk customer after $n_f$ days if and only if $\sum_{i=0}^{n_f-1} \mu_{{\rm mD}(D,i)}^{(C)} \color{black}\ge z^{(C)} - z_\alpha^{(C)}$. 
\end{prop}

\begin{proof}
\begin{eqnarray*}
&& \hat r_{\alpha,C}(D) \ge 0.5 \\
&\iff&  1 - \int_{-\infty}^{z^{(C)}-z_\alpha^{(C)}} \bar p_{n_f}^{(C)}(x)dx \ge 0.5 \\
&\iff& 0.5 \ge \int_{-\infty}^{z^{(C)}-z_\alpha^{(C)}} \bar p_{n_f}^{(C)}(x)dx \\
&\iff& \sum_{i=0}^{n_f-1} \mu_{{\rm mD}(D,i)}^{(C)}  \ge z^{(C)} - z_\alpha^{(C)} \quad (\because \bar{p}_{n_f}^{(C)} \text{is a symmetric probability distribution.})
\end{eqnarray*}
\qed
\end{proof}

==> history/transportation_research_partC/DeliveryList/src/updated_NF.tex <==
\begin{algorithm}                      
\caption{Updated Next-Fit Algorithm}         
\label{alg:updated_NF}                          
\begin{algorithmic}      
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE High-risk customers $\mathcal{C}^*$, distance function $d$
and truck feasible function $P$
\ENSURE The division of high-risk customers $\mathcal{C}_1^*, \ldots, \mathcal{C}_k^*$
\STATE $C_s, C_e \gets \underset{(C,C') \in \mathcal{C}^* \times \mathcal{C}^*}{\rm argmax}d(C,C')$
\STATE Sort $\mathcal{C}^*$ with $g(C) = d(C_s, C) - d(C_e, C)$.
\STATE $k \gets 1$
\STATE $\mathcal{C}_k^* \gets \emptyset$
\FOR{$i = 1$ to $n$}
\IF{$P(\mathcal{C}_k^* \cup \{C_i\})$ is False}
\STATE $k \gets k + 1$
\STATE $\mathcal{C}_k^* \gets \emptyset$
\ENDIF
\STATE $\mathcal{C}_k^* \gets \mathcal{C}_k^* \cup \{C_i\}$
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> history/transportation_research_partC/DeliveryRoute/src/dr_main.tex <==
\section{Delivery Route Optimization\label{sec:delivery_route}}

In this section, we would like to determine the following aspects.
\begin{itemize}
    \item The customers are to receive a delivery. We deliver moderate-risk customers as much as possible by delivering them to high-risk customers.
    \item The order is delivered to the customers. We utilize MapBox to acquire the optimal route between two customers.
\end{itemize}

To realize these conditions, we propose two frameworks for acquiring the final output, which is described in Section~\ref{sec:IP-based}.
Each framework contains multiple algorithms, most of which are formulated as integer optimization problems.
Because it is essential to construct an algorithm that can be used in the real world, the framework should output a reasonable delivery plan in all cases.
Therefore, we prepare a greedy but reasonable algorithm for a situation in which we cannot find a feasible solution to integer optimization problems.

\input{6:DeliveryRoute/src/graph_construction}

\subsection{Preliminaries for Demonstrating the Algorithm to Obtain a Delivery Route}
\input{6:DeliveryRoute/src/maxDeli}
\input{6:DeliveryRoute/src/minWork}
\input{6:DeliveryRoute/src/tsp}
% \input{6:DeliveryRoute/src/tsptw}
% \input{6:DeliveryRoute/src/tsptw_modify}
\input{6:DeliveryRoute/src/squeeze}


\input{6:DeliveryRoute/src/ip-based}
% \input{6:DeliveryRoute/src/tsp-based}

==> history/transportation_research_partC/DeliveryRoute/src/graph_construction.tex <==
\subsection{Topology Construction for Obtaining Multi-trip Delivery Order}


% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=13cm]{6:DeliveryRoute/figs/graph_construction.png}
% \caption{Topology construction to obtain multi-trip delivery route}
% \end{center}
% \label{fig:graphIP}
% \end{figure}

This section constructs a graph and acquires the path representing the delivery order to formulate integer optimization problems.
We prepare the vertex and edge as follows:
\begin{enumerate}
    \item $V := \cup_{i=1}^{m}\mathcal{C}^{(i)} \cup SN$ : Vertices
    \begin{itemize}
        \item $\mathcal{C}^{(i)}$ : Set of customers selected in trip $i$
        \item $SN$ : Set of supernodes representing the delivery center%$s_1,\ldots ,s_{m+1}$
    \end{itemize}
    \item  $E := E_{inter} \cup E_{intra}$ : Edges
    \begin{itemize}
        \item $E_{inter} (\forall (v_0, v_1) \in E_{inter}, v_0 \notin SN \land v_1 \notin SN)$ : Edge represents during the trip (customer to customer) 
        \item $E_{intra} (\forall (v_0, v_1) \in E_{intra}, v_0 \in SN \lor v_1 \in SN)$ :  Edge represents across the trip (supernode to customer)
    \end{itemize}
\end{enumerate}


==> history/transportation_research_partC/DeliveryRoute/src/ip-based.tex <==
\subsection{IP-based Algorithm \label{sec:IP-based}}

The first framework is mainly developed using an integer optimization problem.
As the basic concept, we add moderate-risk customers to the delivery route after obtaining only high-risk customers.
The flowchart of the algorithm is illustrated in Figure~\ref{fig:IP-based}.

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=13cm]{6:DeliveryRoute/figs/IP-based_alg_2.png}
\caption{IP-based algorithm \label{fig:IP-based}}
\end{center}
\end{figure}

\subsubsection{Demonstrating the Flowchart}
\paragraph{Traveling Salesman Problem only High-risk Customers}
\begin{enumerate}
    \item Algorithm\\
    2-opt algorithm to solve Traveling Salesman Problem (Section~\ref{sec:tsp})
    \item Motivation\\
    To determine which integer optimization problem should be solved.
    \item Next Step
    \begin{itemize}
        \item When the arrival time of the last trip is earlier than the end of the work hours, we solve the maxDeli model described in Section~\ref{sec:maxdeli}.
        \item When the arrival time of the last trip is earlier than the limits for overwork, we solve the minWork model described in Section~\ref{sec:minWork}.
        \item When the arrival time of the last trip is later than the limits for the overwork, we solve the maxDeli model described in Section~\ref{sec:maxdeli}.
    \end{itemize}
\end{enumerate}


\paragraph{Maximize the Number of Deliveries of Moderate-risk Customers}
\begin{enumerate}
    \item Algorithm\\
    Maximize the delivery model (Section~\ref{sec:maxdeli})
    We input the moderate- and high-risk customers as those for delivery and those that must be delivered to, respectively.
    \item Motivation\\
    We acquire a delivery route that maximizes the number of moderate-risk customers while ensuring deliveries to high-risk customers.
    \item Next Step
    \begin{itemize}
        \item When the incumbent solution is obtained, we obtain the delivery route with the minimum duration, including the moderate-risk customers.
        \item When the incumbent solution is not obtained, we solve the delivery route with the minimum duration.
    \end{itemize}
\end{enumerate}

\paragraph{Minimize Delivery Route Including Moderate-risk Customers}
\begin{enumerate}
    \item Algorithm\\
    Minimize the working time in Section~\ref{sec:minWork}.
    \item Motivation\\
    We acquire the minimum working time for visits to every high- and moderate-risk customer chosen in the maximum-delivery model.
    \item Next Step\\
    The result is the final output of the IP-based algorithm; the output of the last problem is one of the feasible solutions to the problem.
\end{enumerate}

\paragraph{Minimize Delivery Route only for High-risk Customers}
\begin{enumerate}
    \item Algorithm\\
    Minimize the working time in Section~\ref{sec:minWork}.
    \item Motivation\\
    We acquire the minimum working time for visiting every high-risk customer.
    \item Next Step
    \begin{itemize}
        \item When the incumbent is obtained, we output the result as the final output of the IP-based algorithm.
        \item When the incumbent is not obtained, we go to the traveling salesman problem only for high-risk customers.
    \end{itemize}
\end{enumerate}

\paragraph{Traveling Salesman Problem only High-risk Customers}
\begin{enumerate}
    \item Algorithm\\
    2-opt algorithm to solve traveling salesman problem (Section~\ref{sec:tsp})
    \item Motivation\\
    To obtain the shortest route in terms of duration to visit every high-risk customer.
    \item Next Step
    \begin{itemize}
        \item When the arrival time of the last trip is earlier than the end of the work hours, we output the result as the final output of the IP-based algorithm.
        \item When the arrival time of the last trip is not earlier than the end of the work hours, we solve the maxDeli model described in Section~\ref{sec:maxdeli} only for high-risk customers.
    \end{itemize}
\end{enumerate}

\paragraph{Maximize Delivery to High-risk Customers}
\begin{enumerate}
    \item Algorithm\\
    Maximize delivery model (Section~\ref{sec:maxdeli})
    \item Motivation\\
    When we give up on delivering all high-risk customers based on constraints such as staff time availability, we would like to maximize the delivery to high-risk customers.
    \item Next Step
    \begin{itemize}
        \item When we obtain the incumbent, we output the result as the final output of the IP-based algorithm.
        \item When we cannot obtain the incumbent, we move to the squeeze model.
    \end{itemize}
\end{enumerate}

\paragraph{Squeeze Delivery for High-risk Customers}
\begin{enumerate}
    \item Algorithm\\
    Squeeze model (Section~\ref{sec:squeeze})
    \item Motivation\\
    We construct a simple but reasonable algorithm for obtaining a delivery route that satisfies the schedule constraint of the driver.
    \item Next Step\\
    We output the final result of IP-based algorithm.
\end{enumerate}

% \subsubsection{Output}
% The output can be categorized three type, and each type can describe their output.
% \begin{enumerate}
%     \item Delivery for moderate-risk customer
%     \item Delivery only for all high-risk customer
%     \item Delivery only for partial high-risk customer
% \end{enumerate}


==> history/transportation_research_partC/DeliveryRoute/src/maxDeli.tex <==
\subsubsection{Maximize the Number of Delivery \label{sec:maxdeli}}

\paragraph{Motivation}
% We would like to deliver as much as the moderate-risk customer while ensuring delivery to the high-risk customer.
With this problem, we would like to acquire a delivery route that maximizes the number of deliveries to moderate-risk customers under ensuring the deliveries to high-risk customers.
When we try to maximize the number of visits, the routes become efficient.
Note that if the duration of a staff time window is much larger than the number of candidate customers, the routes tend to become redundant.


\paragraph{Formulation}

\begin{enumerate}
\item Variables
    \begin{itemize}
        \item $x_{C, C^{\prime}}=
        \left\{
            \begin{array}{ll}
                1 & \text{Staff visits customer} \ C^{\prime} \ \text{next to} \ C \\
                0 & \text{o.w.}
            \end{array}
        \right.$
        \item $u_C \in \mathbb{Z}$ : The order in which customer $C$ is visited in one day.
        \item $t_C \in \mathbb{Z}$ : The time when a worker visits customer $C$. Note that, the worker replaces cylinders after $t_C$ 
    \end{itemize}
\item Constants
    \begin{itemize}
        \item $d: V \times V \to \mathbb{R}$ : The duration of movement between two points
        \item $[T_{lb}^{\rm work}, T_{ub}^{\rm work}] \subset [0, 24\times60]$ Time window representing for staff availability (minutes)
        % \item $T_{\rm work} \in [0, 24\times60]$ : Duration of work by staff
        \item $[T_{lb}^{C}, T_{ub}^{C}] \subset [0,24\times60]$ : Time window representing availability of customer $C$ 
        \item $rep : \mathcal{C} \to \mathbb{R}$ The duration for replacing gas cylinder
        \item $m$ : Number of trips
        \item $\mathcal{C}_i^*$ : Customer must be visited during trip $i$
        \item $\mathcal{C}_i^{\prime}$ : Customer can be chosen to be delivered in trip $i$
        \item $N: V \rightarrow 2^{V}$: Neighbor customers from customer
        \item $n := |V|$
        % \item $n = \sum_{i = 1}^{m}|\mathcal{C}_i^* \cup \mathcal{C}_i^{'}|　+ |SN|$ : Number of customers  to be visited in trip from $1$ to $m$ 
    \end{itemize}
\end{enumerate}


The formulation of maxDeli model is shown in Problem~\ref{prob:maxDeli}.
Constraints 1 and 2 represent the flow conservation for the customers. 
Moreover, it ensures that high-risk customers must be delivered, and moderate-risk customers can be delivered.
Constraints 3 and 4 ensure that every supernode satisfies the flow conservation and must be visited immediately.
Constraint 5 is the sub-tour elimination constraint.
Constraint 6 is the relationship between variables $x$ and $u$.
Constraints 7 and 8 are set to satisfy the time demands of the customers and staff, respectively.
Constraint 9 ensures the relationship between $x$ and $t$.
Constraint 10 assures that the working time is included in the staff's availability.

% Constraint 1 to 4 ensures that the square covers the customers to be delivered.
% Constraint 5 enables us to always deliver to high-risk customers.
% Constraint 7 and 8 can be obtained from Constraints 1 to 5, but we set them explicitly to find a feasible solution quickly. 
% If it were not for the (6) constraint, the output rectangle always becomes only covering the high-risk customers.
% Therefore, we have to prepare the lower bound of the number of delivery $N_0$.

\begin{problem}
\label{prob:maxDeli}
maxDeli: Acquiring the Delivery Order for the High-risk and Moderate-risk Customers
\[
\begin{aligned}
& \underset{x,u,t}{\rm maximize} && \sum_{(C,C^{'})\in E} x_{C,C^{'}} 
\\
& \rm{subject \ to} && \sum_{C_{0} \in N(C)} x_{C_{0}, C}=\sum_{C_{1} \in N(C)} x_{C, C_{1}} \leq 1 \ (\forall C \in V \setminus SN) && & \text{(1)}
\\
& && \sum_{C_{0} \in N(C)} x_{C_{0}, C}=\sum_{C_{1} \in N(C)} x_{C, C_{1}} = 1 \ (\forall i, \forall C \in \mathcal{C}^{*}_{i}) && & \text{(2)}
\\
& && \sum_{C \in N(s_1)} x_{sn_1, C} = \cdots = \sum_{C \in N(sn_{m-1})} x_{sn_{m-1}, C} = 1 \ (sn_1 ,\ldots, sn_{m-1} \in SN)  && & \text{(3)}
\\
& && \sum_{C \in N(sn_2)} x_{C, sn_2} = \cdots = \sum_{C \in N(sn_{m})} x_{C, sn_{m}} = 1 \ (sn_2 ,\ldots, sn_{m} \in SN) && & \text{(4)}
\\
& && u_{C} - u_{C^{'}} + (n-1)x_{C,C^{'}} \le n - 2 \ (\forall C,C^{'} \in V) && & \text{(5)}
\\
& && T_{lb}^{C} \sum_{C^{\prime} \in V} x_{C^{\prime}, C} \leq t_{C} \leq \left(T_{ub}^{C}-rep({C})\right) \sum_{C^{\prime} \in V} x_{C^{\prime}, C} \quad(\forall C \in V \setminus SN) && & \text{(6)}
\\
& && t_{C} - t_{C^{'}} \le T_{max} - rep({C^{'}}) && & \text{(7)}
\\
& && t_{C^{\prime}}-t_{C} \geq\left(rep({C})+d({C, C^{\prime}})\right) x_{C, C^{\prime}}-T_{\max }\left(1-x_{C, C^{\prime}}\right)\left(\forall\left(C, C^{\prime}\right) \in E\right) && & \text{(8)}
\\
& &&T_{lb}^{\rm work} \le t_{C} \le T_{ub}^{\rm work} && & \text{(9)}
\end{aligned}
\]
\end{problem}

% \paragraph{Situation}
% \begin{enumerate}
%     \item a
%     \item b 
% \end{enumerate}

% \paragraph{Next step}
% \begin{enumerate}
%     \item (Feasible) The incumbent or optimal solution is obtained.\\
%     We solve the maxDeli model described in the \ref{sec:maxdeli}
%     \item The incumbent is not obtained.\\
%     We solve the minWork model described in the \ref{sec:minWork}
% \end{enumerate}


==> history/transportation_research_partC/DeliveryRoute/src/minWork.tex <==
\subsubsection{Minimize the Working Duration for Delivery \label{sec:minWork}}

\paragraph{Motivation}
We minimize the working time under delivery to all given customers.
Note that we consider a much more complicated problem than the traveling salesman problem due to other constraints such as time window constraints.

\paragraph{Formulation}
\begin{problem}
\label{prob:minWork}
minWork: Acquiring the Delivery Order for All High-risk Customers ( All notation is followed by~\ref{sec:maxdeli} )
\[
\begin{aligned}
& \underset{x,u,t}{\rm minimize} && \underset{C,C^{\prime}}{\max}(t_{C^{\prime}} + rep({C})) x_{C,C^{'}} 
\\
& \rm{subject \ to} && \sum_{C_{0} \in N(C)} x_{C_{0}, C}=\sum_{C_{1} \in N(C)} x_{C, C_{1}} = 1 \ (\forall C \in V \setminus S)  && & \text{(1)}
\\
& && \sum_{C \in N(s_1)} x_{s_1, C} = \cdots = \sum_{C \in N(s_{m-1})} x_{s_{m-1}, C} = 1 \ (sn_1 ,\ldots, sn_{m-1} \in SN) && & \text{(2)}
\\
& && \sum_{C \in N(s_2)} x_{C, s_2} = \cdots = \sum_{C \in N(s_{m})} x_{C, s_{m}} = 1 \ (sn_2 ,\ldots, sn_{m} \in SN)  && & \text{(3)}
\\
& && u_{C} - u_{C^{'}} + (n-1)x_{C,C^{'}} \le n - 2 \ (\forall C,C^{'} \in V) && & \text{(4)}
\\
% \\
% & && n \sum_{C^{\prime}} x_{C^{\prime}, C} \geq u_{C}(\forall C \in V) && & \text{(5)}
% \\
& && T_{lb}^{C} \sum_{C^{\prime} \in V} x_{C^{\prime}, C} \leq t_{C} \leq \left(T_{ub}^{C}-rep({C})\right) \sum_{C^{\prime}} x_{C^{\prime}, C} \quad(\forall C \in V \setminus S) && & \text{(5)}
% & && t_{C} - t_{C^{'}} \le T_{max} - d_{C^{'}} && & \text{(7)}
\\
& && t_{C^{\prime}}-t_{C} \geq\left(rep({C})+d({C, C^{\prime}})\right) x_{C, C^{\prime}}-T_{\max }\left(1-x_{C, C^{\prime}}\right)\left(\forall\left(C, C^{\prime}\right) \in E\right) && & \text{(6)}
\end{aligned}
\]
\end{problem}

The formulation of the {\it minWork} model is shown in Problem~\ref{prob:minWork}.
%Constraints 1 and 2 represent the flow conservation for customers. 
%Moreover, this ensures that high-risk customers must be delivered and that moderate-risk customers are excluded from delivery.
%Constraints 3 and 4 ensure that every supernode satisfies the flow conservation and must be visited immediately.
%Constraint 5 is the sub-tour elimination constraint.
%Constraint 6 is the relationship between variables $x$ and $u$.
%Constraints 7 and 8 are set to satisfy the time demands of the customers and staff, respectively.
%Constraint 9 ensures the relationship between $x$ and $t$.
Constraints 1 represent the flow conservation for customers. 
Constraints 2 and 3 ensure that every supernode satisfies the flow conservation and must be visited immediately.
Constraint 4 is the sub-tour elimination constraint.
% Constraint 5 is the relationship between variables $x$ and $u$.
Constraints 5 is the set to satisfy the time demands of the customers respectively.
Constraint 6 ensures the relationship between $x$ and $t$.


% \paragraph{Next step}
% \begin{enumerate}
%     \item (Feasible) The incumbent or optimal solution is obtained.\\
%     We solve the maxDeli model described in the \ref{sec:maxdeli}
%     \item The incumbent is not obtained.\\
%     We solve the minWork model described in the \ref{sec:minWork}
% \end{enumerate}

==> history/transportation_research_partC/DeliveryRoute/src/squeeze.tex <==
\subsubsection{Squeeze Customers by Focusing on the Risk of Gas Shortage\label{sec:squeeze}}

When the maxDeli model for high-risk customers cannot find a feasible solution, we apply the {\it squeeze} model for the greedy but reasonable method to determine the order for delivery.
The basic strategy of {\it squeeze} model is to remove the delivery list with the minimum value of risk function until the end time of delivery satisfies the staff's availability.
The details are summarized in Algorithm~\ref{alg:squeeze}.
The model has no guarantee in satisfying the customer's availability, as in the maxDeli model, for high-risk customers.

\begin{algorithm}                      
\caption{(Squeeze Model) Squeeze the Customers to Satisfy the Time Window of the Staff}         
% \label{alg:squeeze}                          
% \begin{algorithmic}   
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \REQUIRE Delivery route $\mathcal{C}^{(1)}, \ldots, \mathcal{C}^{(m)}$
% \ENSURE Delivery route $\mathcal{C}^{(1)}, \ldots, \mathcal{C}^{(m)}$
% \WHILE {$\underset{C}{\max} \  t_C > T_{\max}$}
% \STATE $C \gets \underset{C \in \mathcal{C}^*}{\rm argmax} \  r_{\alpha,C}(D) $ 
% \STATE pop customer $C$ from $C^*$
% \STATE update visiting time
% \ENDWHILE
% \end{algorithmic}
% \end{algorithm}

\label{alg:squeeze}                          
\begin{algorithmic}   
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE 
\begin{itemize}
    \item Ordered list of delivery positions $\{C_i \}_{i=1}^n \ (C_i \in \mathcal{C} \cup SN)$
    \item Ordered list of arrival times $\{t_i \}_{i=1}^n \ (t_i \le t_{i+1})$ (Staff visits $C_j$ at $t_j$)
    \item $r_{\alpha, C}(D)$ : value of risk function of customer $C$, where $\alpha$ and $D$ are hyperparameters
    \item $d:V \times V \to \mathbb{R}$ : The duration of movement between two points
    \item $rep : V \to \mathbb{R}$ : The duration for replacing gas cylinder when staff visits customers, and the duration for breaking time when staff visits base.
% \STATE \bar{\mathcal{C}}^* \gets {C_i \in \mathcal{C}^* | }
\end{itemize}
\ENSURE 
\begin{itemize}
 \item Ordered list of delivery positions $\{C_i \}_{i=1}^{n'} \ (C_i \in \mathcal{C} \cup SN)$
 \item Ordered list of arrival times $\{t_i \}_{i=1}^{n'} \ (t_i \le t_{i+1})$ (Staff visits $C_j$ at $t_j$)
\end{itemize}
\STATE $n' \gets n$
\WHILE {$t_{n'} > T_{\max}$}
\STATE $C_j \gets \underset{C \in \mathcal{C}}{\rm argmin} \  r_{\alpha,C}(D) $ 
% 削除対象のLC１つのみで構成されるトリップの場合
\IF{$C_{j-1} \in SN$ and $C_{j+1} \in SN$}
\STATE {\small {\it  // remove $C_j$ and $C_{j+1}$}}
\STATE $t_{{\rm diff}}$ $\gets d(C_{j-1},C_{j})+rep(C_j)+d(C_{j},C_{j+1})+rep(C_{j+1})+d(C_{j+1},C_{j+2})-d(C_{j-1}, C_{j+2})$
\STATE $i \gets 2$
\ELSE
\STATE {\small {\it // remove $C_j$} }
\STATE $t_{{\rm diff}}$ $\gets d(C_{j-1},C_{j})+rep(C_j)+d(C_{j},C_{j+1})-d(C_{j-1},C_{j+1})$
\STATE $i \gets 1$
\ENDIF
\STATE {\small {\it // update ordered lists $C$ and $t$}}
\FOR{$k = j$ to $n'-i$}
\STATE $C_{k} \gets C_{k+i}$
\STATE $t_{k} \gets t_{k_i} - t_{{\rm diff}}$
\ENDFOR
\STATE $n' \gets n' - i$
% \STATE Pop $C_j$ and $C_{j+1}$ from $\{C_i \}_{i=1}^{n'}$
% \STATE Pop $t_j$ and $t_{j+1}$ from $\{t_i \}_{i=1}^{n'}$
% \STATE $\mathcal{C}_n \gets \mathcal{C}_n \setminus \cup_{k=n-i}^{n}\{C_k\}$
% \STATE $\mathcal{T}_n \gets \mathcal{T}_n \setminus \cup_{k=n-i}^{n}\{t_k\}$
% \IF{$C_{j-1} \in SN$ and $C_{j+1} \in SN$}
% \STATE $diff$ $\gets d(C_{j-1},C_{j})+rep(C_j)+d(C_{j},C_{j+1})+rep(C_{j+1})+d(C_{j+1},C_{j+2})-d(C_{j-1}, C_{j+2})$
% \FOR{$k = j$ to $n-2$}
% \STATE $C_{k} \gets C_{k+2}$
% \STATE $t_{k} \gets t_{k+2} - diff$
% \ENDFOR
% \STATE $\mathcal{C}_j \gets \mathcal{C}_j \setminus \{C_{n-1}, C_n\}$
% \STATE $\mathcal{T}_j \gets \mathcal{T}_j \setminus \{C_{n-1}, T_n\}$
% \ELSE
% \STATE $diff$ $\gets d(C_{j-1},C_{j})+rep(C_j)+d(C_{j},C_{j+1})-d(C_{j-1}, C_{j+1})$
% \FOR{$k = j$ to $n-1$}
% \STATE $C_{k} \gets C_{k+1}$
% \STATE $t_{k} \gets t_{k+1} - diff$
% \ENDFOR
% \STATE $\mathcal{C}_j \gets \mathcal{C}_j \setminus \{C_n\}$
% \STATE $\mathcal{T}_j \gets \mathcal{T}_j \setminus \{T_n\}$
% \ENDIF
% \STATE $n \gets |\mathcal{C}_n|$
\ENDWHILE
% \STATE $n' \gets |\mathcal{C}|$
\RETURN $\{C_i \}_{i=1}^{n'}$ and $\{t_i \}_{i=1}^{n'}$
\end{algorithmic}
\end{algorithm}

==> history/transportation_research_partC/DeliveryRoute/src/tsp-based.tex <==
\subsection{TSP-based Algorithm \label{sec:tsp-based}}

The second framework is mainly developed with traveling salesman problems with time window.
The image is that we remove the moderate-risk customers to the delivery route after obtaining the delivery route for all high-risk and moderate-risk customers.
The flowchart is visualized in Figure~\ref{fig:TSP-based}.

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=13cm]{6:DeliveryRoute/figs/TSP-based_alg.png}
\caption{TSP-based algorithm\label{fig:TSP-based}}
\end{center}
\end{figure}

\subsubsection{Demonstrating the flowchart}
\paragraph{Traveling Salesman Problem with Time Window for both moderate-risk and high-risk customers}
\begin{enumerate}
    \item Algorithm\\
    Traveling Salesman Problem with Time Window (Section~\ref{sec:tsptw})
    \item Motivation\\
    To determine all moderate-risk customers can be delivered.
    \item Next Step
    \begin{itemize}
        \item When the arrival time of the last trip is earlier than the end of work hours, we solve the modified model described in Section~\ref{sec:modify}.
        \item When the arrival time of the last trip is earlier than the limits for the overwork, we solve the minWork model described in Section~\ref{sec:minWork}.
        \item When the arrival time of the last trip is later than the limits for the overwork, we solve the maxDeli model described in Section~\ref{sec:maxdeli}.
    \end{itemize}
\end{enumerate}


\paragraph{Extract the moderate-risk customers to be delivered}
\begin{enumerate}
    \item Algorithm\\
    Modify Model (Section~\ref{sec:modify})
    \item Motivation\\
    We extract some moderate-risk customers to satisfy the staff's shift constraint if needed.
    \item Next Step
    \begin{itemize}
        \item When we find the solution, we output as the final result of tsp-based algorithm.
        \item When the incumbent solution is not obtained, we solve the minimum duration's delivery route only for high-risk customers.
    \end{itemize}
\end{enumerate}

The latter part of the algorithm is as same as the IP-based algorithm from Section 6.3.1.4 to 6.3.1.7.
Therefore, we do not write down the same things again.

==> history/transportation_research_partC/DeliveryRoute/src/tsp.tex <==
\subsubsection{Traveling Salesman Problem \label{sec:tsp}}

Traveling Salesman Problem (TSP) is a well-known problem: to find a minimum cost route under visits every city once.
The output of simple TSP does not ensure the time window constraint for staff and customers. However, we utilize this problem for selecting which integer optimization problem to be solved.
We apply the 2-opt method to update better TSP solution after obtaining the nearest neighbor method to acquire an initial solution.

We input the high-risk customer to solve TSP for each trip.
When we solve TSP for after the second trip, we add the rest time after coming back to the center on the last trip. 

% \paragraph{Next step}
% \begin{enumerate}
%     \item (Feasible) When the arrival time of the last trip is earlier than the end of work hours.\\
%     We solve the maxDeli model described in Section~\ref{sec:maxdeli}.
%     \item When the arrival time of the last trip is earlier than the limits for the overwork.\\
%     We solve the minWork model described in Section~\ref{sec:minWork}.
%     \item When the arrival time of the last trip is later than the limits for the overwork.
% \end{enumerate}

==> history/transportation_research_partC/DeliveryRoute/src/tsptw.tex <==
\subsubsection{Traveling Salesman Problem with Time Window \label{sec:tsptw}}

Traveling Salesman Problem with Time Window is the problem of acquiring the minimum cost path for visiting every town once with satisfying the time window of the city.
We utilized the algorithm proposed in \cite{cheng2007modified}.

\paragraph{Motivation}
We obtain the delivery plan for all moderate-risk and high-risk customers with satisfying the time window for customers.
After that, we give up to delivery to some moderate-risk customers for satisfying the time window of staff if necessary, which is described in Section~\ref{sec:modify}.

==> history/transportation_research_partC/DeliveryRoute/src/tsptw_modify.tex <==
\subsubsection{Modify delivery route to satisfy all time window \label{sec:modify}}

\paragraph{Motivation}
The output of TSPTW (Section~\ref{sec:tsptw}) does not ensure to satisfy the duration for a staff time window.
Therefore, we would like to remove the visits for the moderate-risk customer to satisfy the staff time window.
The customer to be removed is selected the time difference between if it were visited and not visited.
We determine not to visit the customer while the staff time window does not satisfy.

\begin{algorithm}                      
\caption{(Modify delivery route to satisfy all time window)}         
\label{alg:modify}                          
\begin{algorithmic}   
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE Delivery route $\mathcal{C}^{(1)}, \ldots, \mathcal{C}^{(m)}$
\ENSURE Delivery route $\mathcal{C}^{(1)}, \ldots, \mathcal{C}^{(m)}$
\WHILE {$\underset{C}{\max} \  t_C > T_{\max}$}
\STATE $C_1, C_2 \Leftarrow$ the customers with the maximum save working duration if they were not visited
\STATE pop customer $C_1$ and $C_2$
\STATE update visiting time
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> history/transportation_research_partC/DemandPrediction/src/ML/GradientBoostingRegression.tex <==
\subsubsection{Gradient Boosting Regression Trees}
Gradient Boosting Regression Trees (GBRT) utilize a boosting approach to sequentially constructing regression trees with reweighted versions of the training data ~\cite{schapire1990strength,10.1214/aos/1016218223, friedman2001greedy}).
% On the forecasting day $D_0$, we forecast the daily gas usage for the next $n_{\rm n}$ days $\boldsymbol{\widehat{\rm du}}_{0}$, by using the actual observed daily gas usage for the past $(n_{\rm p}+n_{\rm s}-1)$ days $\boldsymbol{{\rm du}}_{i}'(\forall i \in [-n_{\rm s}-1,-1]\cap\mathbb{Z})$, 

We use a tree-structured regression set $\left\{\text{Tree}_{j}\left(\boldsymbol{\rm du} ; \boldsymbol{\beta}_{j}\right), r=1, \ldots, n_{\rm t}\right\}$, where $\boldsymbol{\beta}_{j}$ is a parameter for dividing each tree node, and a parameter $\rho_j$ which is the scaling factor that determines which subset regression is used and how strongly. 
% The number of trees $R$ is set to 100. 
We obtain $\boldsymbol{\beta}_{j}$ and $\rho_j$ by sequentially fitting a simple parameterized function, i.e., a base learner, to the current pseudo-residuals using the least-squares at each iteration. 
We then forecast $\widehat{\rm du}_{D_0+i}$ as 
$\dsp \sum_{j=1}^{n_{\rm t}}\rho_j \mathrm{~Tree}_{j}\left(\boldsymbol{{\rm du}}_{D_0+i} ; \boldsymbol{\beta}_{j}\right)$.\\

% Advantage 
% \begin{itemize}
% \item GBR is robust against long-tailed distributions and outliers because it is invariant under all monotone transformations of the individual input variables. (\cite{friedman2001greedy})
% \item GBR tends to be quite robust against the addition of irrelevant input variables. (\cite{friedman2001greedy})
% \item GBR can be interpreted using partial dependence plots in conjunction with the input variable relative importance measure. (\cite{friedman2001greedy})
% \item GBR increases the flexibility of stable weak learners by incorporating them in a jointly fitted additive expansion. (\cite{10.1214/aos/1016218223}
% \end{itemize}
    
% Disadvantage
% \begin{itemize} 
% \item Many boosting iterations may be required to obtain the optimal GBR approximations. (\cite{friedman2001greedy})
% \end{itemize}






==> history/transportation_research_partC/DemandPrediction/src/ML/LinearRegression.tex <==
\subsubsection{Linear Regression}
Multiple linear models are the most primitive and widely-used models. We use a linear least squares regression with $L^2$ regularization, which is ridge regression.  

Using the hyperparameter $\lambda$, which determines the strength of the regularization, we obtain $\boldsymbol{\beta}$ by calculating 
$\dsp \arg\min_{\boldsymbol{\beta}}  \left\{\sum_{ i =-n_{\rm s}}^{-1}{(\boldsymbol{\beta}^T\boldsymbol{{\rm du}}_{D_0+i}-{\rm du}_{D_0+i})}^{2}+\lambda \boldsymbol{\beta}^T\boldsymbol{\beta}\right\}$



==> history/transportation_research_partC/DemandPrediction/src/ML/RandomForestRegression.tex <==
\subsubsection{Random Forest Regression}
Random Forest Regression (RFR) utilizes the bagging approach to grow a decision regression tree for each of the bootstrap samples independently (~\cite{breiman1996bagging,breiman2001random}).
% On the forecasting day $D_0$, we forecast daily gas usage for the next $n_{\rm n}$ days $\boldsymbol{\widehat{\rm du}}_{0}$, by using the actual observed daily gas usage for the past $(n_{\rm p}+n_{\rm s}-1)$ days $\boldsymbol{{\rm du}}_{i}'(\forall i \in [-n_{\rm s}-1,-1]\cap \mathbb{Z})$, and 

We use a tree-structured regression set $\left\{\text{Tree}_{j}\left(\boldsymbol{\rm du} ; \boldsymbol{\beta}_{j}\right), j=1, \ldots, n_{\rm t}\right\}$, where $\boldsymbol{\beta}_{j}$ is a parameter for dividing each tree node. 
We obtain the parameter $\boldsymbol{\beta}_{j}$ by minimizing the prediction error, that is, the least-squares between the predicted and the observed values. 
Then, we forecast 
$\widehat{\rm du}_{D_0+i}$ as 
$\dsp \frac{1}{n_{\rm t}} \sum_{j=1}^{n_{\rm t}} \mathrm{~Tree}_{j}\left(\boldsymbol{{\rm du}}_{D_0+i} ; \boldsymbol{\beta}_{j}\right)$.


% Advantage (~\cite{breiman2001random}~)
% \begin{itemize}
% \item RFR is robust against overfitting because of the law of large numbers.
% \item RFR is usually not overly sensitive to values of the two main parameters: the number of variables in the random subset at each node and the number of trees in the forest.
% \item The accuracy of RFR is as good as that of Adaboost and sometimes better.
% \item RFR is relatively robust to outliers and noise because it does not concentrate weight on any subset of regressions. 
% \item RFR is faster than the other bagging models because it is easily parallelized.
% \item RFR can give variable importance by using internal out-of-bag estimates.
% \end{itemize}
    
% Disadvantage
% \begin{itemize}
% \item The structure of RFR is no longer as simple and easy to interpret as a single decision tree. (~\cite{breiman1996bagging}~)
% \end{itemize}




==> history/transportation_research_partC/DemandPrediction/src/ML/SupportVectorRegression.tex <==
\subsubsection{Support Vector Regression} 
Support Vector Regression (SVR) is one of the nonlinear regression models based on the Vapnik-Chervonenkis theory of support vectors(~\cite{ boser1992training, vapnik1995support, drucker1997support}).
% On the forecasting day $D_0$, the daily gas usage for the next $n_{\rm n}$ days  $\boldsymbol{\widehat{\rm du}}_{0}$ is forcasted by using the observed daily gas usage for the past $n_{\rm p}$ days $\boldsymbol{{\rm du}}_{i}'(\forall i \in [-n_{\rm s}-1,-1]\cap \mathbb{Z})$, parameters $\boldsymbol{\beta}$ and $\boldsymbol{\beta}'$, 

We use a hyperparameter $\varepsilon$ that determines the radius of the $\varepsilon$ tube.
In addition, we apply the radial basis function kernel $\dsp {\rm K}(\boldsymbol{\rm du}_{t}, \boldsymbol{\rm du}_{t'}):=\exp \left(-\frac{1}{2 \sigma^{2}}\left\|\boldsymbol{\rm du}_{t}-\boldsymbol{\rm du}_{t'}\right\|^{2}\right)$, where $\sigma^2$ is the variance.
We obtain the parameters $\boldsymbol{\beta}$ and $\boldsymbol{\beta}'$ by solving a quadratic programming problem, which is an optimization problem that attempts to find the narrowest $\varepsilon$-tube, while minimizing the prediction error, that is, the distance between the prediction and the observation.
And we forecast $\widehat{\rm du}_{D_0+i}$ as 
$\dsp \beta_0 + \sum_{j=i-n_{\rm p}}^{i-1}\left(\beta_{j}'-\beta_{j}\right) {\rm K}\left({\boldsymbol{\rm du}}_{D_0+i}, {\boldsymbol{\rm du}}_{D_0+j}\right)$.\\

% Advantage
% \begin{itemize}
% \item SVR overcomes the curse of dimensionality because SVR optimization does not depend on the dimensionality of the input space.(~\cite{drucker1997support}).
% \item SVR performs better than Bagging for certain nonlinear problems.(~\cite{drucker1997support}).
% \item SVR forecasts well even when the data set is small.(~\cite{attewell2015data}~)
% robust
% \end{itemize}

% Disadvantage
% \begin{itemize}
% \item The performance of SVR is highly dependent on the settings of the hyperparameters.(~\cite{cherkassky2004practical}~)
% \end{itemize}



==> history/transportation_research_partC/DemandPrediction/src/complement.tex <==
\subsection{Complement Algorithm for Smart Meters \label{sec:complement}}
% The cumulative usage data acquired by smart meters are sometimes not sent on time due to communication errors or dead batteries. As a result, the cumulative usage data is missing. 
% Also, some smart meters are broken and do not send the meter readings for a long time. In the case of meters without smart meters, the cumulative usage data is manually obtained. In the manual meter reading data, the cumulative usage of a  meter is not recorded every day.
% On the other hand, to plan daily gas cylinder delivery, it is necessary to calculate the amount of daily gas remaining and the daily cumulative usage is required. In this section, we describe an algorithm to complement the missing values.
Smart meters are installed in approximately one-third of the meter homes in our target area, allowing us to receive daily cumulative usage data from such meters.
However, the data can be missing owing to communication errors or battery failures. 
In most cases, the data are recovered within a day. However, the data of some meters might be lost for a long period owing to malfunction. 
By contrast, conventional meters can only obtain cumulative usage data manually, approximately once a month.
In this section, we describe algorithms used to complement these missing values. 
When the meters have multiple missing periods, we perform the following completion process iteratively. 
In the following, we assume that the cumulative gas usages $\left \{\widehat{\rm cu}_{D_{\rm start}+i}\right \}_{i \in[0, n_{\rm m}-1] \cap \mathbb{Z}}$ is missing for $n_{\rm m}$ days from date $D_{\rm start}$. 
In this case, we complete the daily usages by $
\left \{\widehat{\rm du}_{D_{\rm start}+i}\right \}_{i \in[-1, n_{\rm m}-1]\cap \mathbb{Z}}$. Note that we also complement the daily usage $\widehat{\rm du}_{D_{\rm start}-1}$ because the first term $\widehat{\rm cu}_{D_{\rm start}}$ in Equation~\ref{equ:du} is missing.

\subsubsection{Smart Meters with Long-Term Missing Cumulative Usage}
Some smart meters are broken and cannot record the cumulative usage for a long period. 
The daily usages of most smart meters used for forecasting are calculated from complemented values. 
Therefore, it is challenging to create forecasting models with high-level performance.
We consider smart meters whose cumulative usages are missing for more than the last 80 days like conventional meters and apply the complementary algorithms and forecasting algorithms to solve this problem.

\subsubsection{Complementary Algorithm for Smart Meters}
We introduce three algorithms for the daily cumulative usage complementary method for smart meters.

\paragraph{Linear Complement Algorithm}
% The linear complement algorithm is simple.
\label{Linear Complement}
\begin{itemize}
% 内挿
    \item Interpolation
% For the missing period $[{D_{\rm start}}, {D_{n_{\rm m}-1}}]$, we calculate the difference $\Delta {\rm cu}(D_{\rm start}, D_{n_{\rm m}-1})$ of the cumulative usage during the following missing period
% \begin{equation}
%     \Delta {\rm cu}(D_{\rm start}, D_{n_{\rm m}-1})={\rm cu}_{D_{\rm start}-{n_{\rm m}}} - {\rm cu}_{D_{\rm start}-1}
% \end{equation}

% By dividing the difference $\Delta{\rm cu}(D_{\rm start}, D_{n_{\rm m}-1})$ by the number of missing days $n_{\rm m}$, we calculate the average daily usage $\Delta{\rm du}(D_{\rm start},D_{n_{\rm m}-1})$ of the missing period.
% \begin{equation}
%     \Delta{\rm du}(D_{\rm start},D_{n_{\rm m}-1}) := \frac{\Delta {\rm cu}(D_{\rm start}, D_{n_{\rm m}-1})}{n_{\rm m}}
% \end{equation}

For the missing period $[{D_{\rm start}}, {\rm mD}(D_{\rm start},n_{\rm m}-1)]$, we calculate the difference of the cumulative usages during the missing period. By using the average daily usage of the missing period, we calculate the cumulative usage of the $i$-th missing for $i \in [0, n_{\rm m}-1]$. %欠損開始日からi日先の累積使用量
\begin{equation}
    \widehat{{\rm cu}}_{D_{\rm start}+i} := {\rm cu}_{D_{\rm start}-1} + (i+1)~\frac{{\rm cu}_{D_{\rm start}-{n_{\rm m}}} - {\rm cu}_{D_{\rm start}-1}}{n_{\rm m}}
\end{equation}

% 外挿
\item Extrapolation \\
    In the completion of the extrapolation, the missing cumulative usage data before the initial meter reading date or after the last meter reading date are completed using the third quartile of the daily usage denoted by ${\emph tq}$. 
\begin{equation}
    \widehat{{\rm cu}}_{D_{\rm start}+i} := {\rm cu}_{D_{\rm start}-1} + (i+1)~{\rm tq}
\end{equation}

\end{itemize}

%周期補完アルゴリズム
\paragraph{Periodic Complement Algorithm} 
Assuming that the daily usage has a periodicity of the week, this algorithm completes the missing day by applying the daily usage of the same day of the week. Unlike the interpolation process of~\ref{Linear Complement}, this algorithm has specific improvements to ensure the monotonicity of its cumulative usage.
For the $i$-th missing day $(i\in [-1, n_{\rm m}-1])$, let $\Lambda_i$ be the set of dates on the same day of the week. 
% for which the daily usage can be calculated.
In this case, the daily usage $\overline{{\rm du}}_{D_{\rm start}+i}$ of the $i$-th missing day from $D_{\rm start}$ is calculated using the following equation, where $\overline{{\rm du}}_{D_{\rm start}+i}$ is the average daily usage of the dates in the set $\Lambda_i$,
% \begin{equation}
%     \Lambda_i^{(M)} := \left\{D={\rm mD}(D_{\rm start},7z+i), \forall z \in \mathbb{Z}~|~ I^{(\rm miss)}(M,D) = 0   \right\}
% \end{equation}
\begin{equation}
    \overline{{\rm du}}_{D_{\rm start}+i} = \frac{1}{|\Lambda_i|}\sum_{\lambda\in \Lambda_i}{\rm du}_{\lambda}.
\end{equation}
        
\begin{itemize}
    \item Interpolation\\
         If we use $\overline{{\rm du}}_{D_{\rm start}+i}$ in the same way as the interpolation process of the linear completion algorithm, it may contradict the monotonicity of the cumulative usage. Therefore, the modified daily usage $\widehat{{\rm du}}_{D_{\rm start}+i}$, modified by applying the calculated daily usage $\overline{{\rm du}}_{D_{\rm start}+i}$, is calculated through the following equation:
        \begin{equation}
            \widehat{{\rm du}}_{D_{\rm start}+i} = \frac{\overline{{\rm du}}_{D_{\rm start}+i}}{\displaystyle \sum_{j=-1}^{n_{\rm m}-1}\overline{{\rm du}}_{D_{\rm start}+j}}\left({\rm cu}_{D_{\rm start}-{n_{\rm m}}}-{\rm cu}_{D_{\rm start}-1}\right)
        \end{equation}
        We complement the cumulative usage $ {\rm cu}_{D_{\rm start}+i}$ using the modified daily usage $\widehat{\rm du}_{D_{\rm start}+i} $.
        \begin{equation}
            \widehat{\rm cu}_{D_{\rm start}+i} = {\rm cu}_{D_{\rm start}-1} + \sum_{j=-1}^{i-1} \widehat{\rm du}_{D_{\rm start}+j}
        \end{equation}

    \item Extrapolation\\
        In the case of an extrapolation, because the modified daily usage $\widehat{\rm du}_{D_{\rm start}+i}$ cannot be calculated, which is applied in the case of the interpolation, the daily usage $\overline{\rm du}_{D_{\rm start}+i}$ is used to supplement the cumulative usage $\widehat{\rm cu}_{D_{\rm start}+i}$.
        \begin{equation}
            \widehat{\rm cu}_{D_{\rm start}+i} = {\rm cu}_{D_{\rm start}-1} + \sum_{j=-1}^{i-1} \overline{\rm du}_{D_{\rm start}+j}
        \end{equation}
        
\end{itemize}

\paragraph{Complementary Algorithm based on Similar Tendencies}
\label{similar complement}
This algorithm extracts meters with similar daily gas usage and completes the missing days. 
As with the periodic complimentary algorithm, there is an improvement to ensure the monotonicity of the cumulative usage.



We define a function ${\rm Sim}(M, k)$ to extract the top-$k$ similarity meters of the meter $M$. The daily usage vector of $M$ is defined as ${\bf du}^{(M)}$, and the inverse of the $L^2$ distance between ${\bf du}^{(M)}$ and ${\bf du}^{(M')}~(M'\in \mathcal{M}_s^*)$ is defined as the similarity $w^{(M,M')}$.
\begin{equation}
    w^{(M, M')} = 
    \frac{1}{||{\bf du}^{(M)} - {\bf du}^{(M')}||_2}
\end{equation}
Let ${\rm Sim}(M, k)$ denote the top-$k$ meters with a high similarity.
\begin{equation}
    {\rm Sim}(M,k):= \underset{S\subset \mathcal{M}_s^*, |S|=k}{\arg\max} \ \underset{M_0\in S}{\min }~w^{(M, M_0)}
\end{equation}
 We denote the meters extracted by ${\rm Sim}(M, k)$ as \emph{k-nearest neighbor meters}.
 Using the daily usages of the smart meters to be complemented during the period when their data are not missing, we calculate the $k$-nearest neighbor meters with similar usage tendencies using ${\rm Sim}(M, k)$. 
        
        Calculate the daily usages for the $i$-th missing day in $[-1, n_{\rm m}-1]\cap \mathbb{Z}$ by applying the daily usages of the meters in ${\rm Sim}(M, k)$.
        \begin{equation}
            \overline{\rm du}_{D_{\rm start}+i}^{(M)} = \frac{1}{k} \sum_{M_0\in {\rm Sim}(M,k)} {\rm du}_{D_{\rm start}+i}^{(M_0)}\\
        \end{equation}
\begin{itemize}
    \item Interpolation\\
        To ensure the monotonicity of the cumulative usage, we calculate the modified daily usage $\widehat{\rm du}_{D_{\rm start}+i}$.
        \begin{equation}
            \widehat{\rm du}_{D_{\rm start}+i} = \frac{\overline{\rm du}_{D_{\rm start}+i}}{\displaystyle \sum_{j=-1}^{n_{\rm m}-1}\overline{\rm du}_{D_{\rm start}+j}}\left({\rm cu}_{D_{\rm start}+n_{\rm m}}-{\rm cu}_{D_{\rm start}-1}\right)
        \end{equation}
        Using the calculated adjusted daily usage $\widehat{\rm cu}_{D_{\rm start}+i}$ for the missing period, we complement the cumulative usage $\widehat{\rm cu}_{D_{\rm start}+i}$ for the $i$-th missing day in $[0, n_{\rm m}-1] \cap \mathbb{Z}$.
        \begin{equation}
            \widehat{\rm cu}_{D_{\rm start}+i} = {\rm cu}_{D_{\rm start}-1} + \sum_{j=-1}^{i-1} \widehat{\rm du}_{D_{\rm start}+j}
        \end{equation}
    \item Extrapolation\\
        In the case of extrapolation, because the adjusted daily usage cannot be estimated, the daily usage is used to supplement the cumulative usage $\widehat{\rm cu}_{D_{\rm start}+i}$ for the missing period
        \begin{equation}
            \widehat{\rm cu}_{D_{\rm start}+i} = {\rm cu}_{D_{\rm start}-1} + \sum_{j=-1}^{i-1} \overline{\rm du}_{D_{\rm start}+j}
        \end{equation}
    
\end{itemize}

% NCU日設置需要家
\subsection{Complementary Algorithm for Conventional Meters}\label{sec:comp_NonNCU}
The frequency of meter reading for conventional meters is approximately once a month. 
It is necessary to complement the daily cumulative usage to conduct daily forecasting and calculation of the remaining gas amount.
Therefore, we introduce an algorithm that completes the cumulative usage by smart meters that do not have missing values. 
This algorithm is similar to that in Section~\ref{similar complement}.

% kNN
\subsubsection{kNN Complement}
\label{complement_kNN}
% ${\rm Sim}:{\mathcal M}\times {\mathcal D}\rightarrow {\mathcal B}({\mathcal S}^*)$ 
A similar meters extraction function ${\rm Sim}:{\mathcal M}\times {\mathbb Z}_{>0} \rightarrow 2^{\mathcal{M}_s^*}$ introduced in Section~\ref{similar complement} is used to extract $k$ neighboring meters. 
Whereas the similar meters complement algorithm calculates the daily usage of the completed target meter $M$ using the average of the daily usage of each of ${\rm Sim}(M, k)$, this algorithm calculates it using a weighted average based on the similarity. 

First, we calculate the weight coefficients $w^{(M,M')}$ for each neighboring meter $M'$. Here, the weight coefficients are normalized such that the sum of the similarities of the neighboring meters is $1$.
 \begin{equation}
    w_{{\rm norm}}^{(M,M')} = \frac{w^{(M,M')}}{\displaystyle \sum_{M_0 \in {\rm Sim}(M, k)} w^{(M,M_0)}}
\end{equation}
The daily consumption of the complementary target meter $M$ is calculated using the weighted average of the daily consumption of neighboring meters using the obtained weight coefficient.
\begin{align*}
    \overline{\rm du}_{D_{\rm start}+i} = \sum_{M_0\in {\rm Sim}(M,k)} w_{{\rm norm}}^{(M,M_0)} ~\overline{\rm du}_{D_{\rm start}+i}^{(M_0)}
\end{align*}
\begin{itemize}
    \item Interpolation\\
        To ensure the monotonicity of the cumulative usage, we calculate the modified daily usage $\widehat{\rm du}_{D_{\rm start}+i}$.
        \begin{equation}
            \widehat{\rm du}_{D_{\rm start}+i} = \frac{\overline{\rm du}_{D_{\rm start}+i}}{\displaystyle \sum_{j=-1}^{n_{\rm m}-1}\overline{\rm du}_{D_{\rm start}+j}}\left({\rm cu}_{D_{\rm start}+n_{\rm m}}-{\rm cu}_{D_{\rm start}-1}\right)
        \end{equation}
        Using the calculated adjusted daily usage $\widehat{\rm du}_{D_{\rm start}+i}$ for the missing period, we supplement the cumulative usage $\widehat{\rm cu}_{D_{\rm start}+i}$ for the $i$-st missing day $\in [0, n_{\rm m}-1]$.
        \begin{equation}
            \widehat{\rm cu}_{D_{\rm start}+i} = {\rm cu}_{D_{\rm start}-1} + \sum_{j=-1}^{i-1} \widehat{\rm du}_{D_{\rm start}+j}
        \end{equation}
        
    \item Extrapolation\\
        In the case of the extrapolation, because the adjusted daily usage cannot be estimated, the daily usage is used to supplement the cumulative usage for the missing period.
        \begin{equation}
            \widehat{\rm cu}_{D_{\rm start}+i} = {\rm cu}_{D_{\rm start}-1} + \sum_{j=-1}^{i-1} \overline{\rm du}_{D_{\rm start}+j}
        \end{equation}
\end{itemize}

% TQ外挿処理
\subsubsection{For Conventional Meters with High Usage}
\label{tq complement}
%One of the disadvantages of the completion algorithm introduced in \ref{complement_kNN} is that the accuracy of the completion value is significantly reduced when the set of meters in ${\rm Sim}(M, k)$ contains meters whose gas usage tendency of $M$ is not similar.
When the set of meters in ${\rm Sim}(M, k)$ contains meters whose gas usage tendency of $M$ is not similar, the accuracy of the complement value is significantly reduced.
In particular, restaurants and laundromats tend to use a large amount of gas, which is highly different from the usage trend of general households. Therefore, we extract those meters that could not be complemented through the kNN completion and apply the linear completion algorithm to those meters, which is expected to reduce the risk of their gas running out.


The $k$-nearest neighbor meters ${\rm Sim}(M, k)$ to conventional meters $M$ are a subset of the smart meters without missing cumulative gas usage data  $\mathcal{M}_s^*$. We extract $\mathcal{M}_c^{HU}$, which has more than the maximum value of the third quartile of the daily usages of each meter in $\mathcal{M}_s^*$, as high gas consumption. 
The extracted meters are likely to differ significantly from the meters in ${\rm Sim}(M, k)$ in terms of their tendency gas usage tendency. 
Letting $TQ_{M_0}$ be the third quartile of the daily usage of meter $M_0$, the maximum value of the third quartile value of the  Smart Meter (TQ\_SM) is defined as follows.
\begin{equation}
    {\rm TQ\_SM} := \max \{ TQ_{M_0}| {M_0} \in \mathcal{M}_s^*\} 
\end{equation}
Using TQ\_SM, conventional meters with high usage $\mathcal{M}_{c}^{HU}$ is represented by the following set.
\begin{equation}
   \mathcal{M}_{c}^{HU} := \{M_0 \in \mathcal{M}_c | TQ_{M_0} > {\rm TQ\_SM}\}
\end{equation}
The missing cumulative usage data of meters in $\mathcal{M}_{c}^{HU}$ are complemented by the~\ref{Linear Complement} algorithm.

==> history/transportation_research_partC/DemandPrediction/src/dp_main.tex <==
\section{Demand Forecast\label{sec:demand_forecast}}
% 3章の説明 残量予測part


The conventional meters keep the cumulative gas usages from the installation of the meter.
The smart meters send the meter value to the core system at 00:00 every day. 
The conventional meters without smart meters are read by gas providers visiting occasionally, such as once a month.
Using these meter values, we forecast the meter values in the future to determine the delivery list.
We propose complementary algorithms and demand forecasting models for conditions, such as the data acquisition interval and the gas usage tendency. 
In order to improve the forecast accuracy, we construct the model selection flow, as shown in the figure.


% We describe algorithms that complete the missing data of past gas usage data and then predict the daily gas usage for each meter for $N$ days.
% First, we describe the completion process for the missing values in the cumulative usage data acquired by smart meters. 
% Next, we describe the completion process for missing values in the cumulative usage data acquired manually. 

% For all meters, we can obtain the daily usage after the complement process. 
% We construct forecasting models using the obtained daily usage.
% We construct four regression models for meters with a smart meter.
% It is difficult for meters without a smart meter to forecast daily usage because the cumulative usage data obtained is only available for one month on average.
% Therefore, we extract meters with smart meters with similar gas usage tendencies and construct a forecasting algorithm using their forecast gas usage. 

% We describe the flow used to obtain the remaining gas values as illustrated in Figure~\ref{fig:overall_dp}.

We describe the flow for forecasting the daily usages as shown in Figure~\ref{fig:overall_dp}.
Let $D_0$ be today’s date. 
We receive the cumulative usages $\left\{{\rm cu}^{(M)}_{D_0}\right\}_{M\in \mathcal{M}_s}$ at 0:00AM from the smart meters. 
If the meter reading is missing, we complement the cumulative usages by $\widehat{\rm cu}^{(M)}_{D_t}$ for each missing date $D_t$. 
We also calculate $\widehat{\rm cu}^{(M)}_{D_t}$ to complement the meter readings of conventional meters that only read cumulative usage once a month.
Then, we obtain the daily usages $\left\{{\rm du}_{mD(D_0,-1)}^{(M)}\right\}_{M\in \mathcal{M}}$ by calculating the difference of the cumulative usage as follows.

\begin{align}
    {\rm du}_{{\rm mD}(D_0,-1)}^{(M)} := {\rm cu}^{(M)}_{D_0} - {\rm cu}^{(M)}_{{\rm mD}(D_0,-1)}    
     \label{equ:du}
\end{align}

For simplicity, we refer to ${\rm cu}_{{\rm mD}(D_0,i)}^{(M)}$ as ${\rm cu}_{D_0+i}$ and refer ${\rm du}_{{\rm mD}(D_0,i)}^{(M)}$ as ${\rm du}_{D_0+i}$ ($i \in \mathbb{Z}$).
%  These are omitted as well in the complement sections, although $D_0$ becomes $D_t$.
Now that we have the daily usages until yesterday ${\boldsymbol{\rm du}}^{(M)}:=[{\rm du}_{D_0-1}, {\rm du}_{D_0-2},\dots]^T$, we can use them to forecast the daily usages for the next $n_{\rm f}$ days including today ${\boldsymbol{\widehat{\rm du}}}_{D_0}^{(M)}:=[\widehat{\rm du}_{D_0}, \widehat{\rm du}_{D_0+1},\dots,\widehat{\rm du}_{D_0+n_{\rm f}-1}]^T$.
This chapter is organized into four sections as follows.


\begin{enumerate}
    \item \textbf{Complementary Algorithm}
    \begin{enumerate}
        \item Section~\ref{sec:complement} describes the complementary algorithm for smart meters.
        \item Section~\ref{sec:comp_NonNCU}  describes the complementary algorithm for conventional meters.
    \end{enumerate}

    \item \textbf{Demand Forecast}
    \begin{enumerate}
        \item Section~\ref{sec:NCU_forecast}  describes the four models used for smart meters.
        \item Section~\ref{sec:NonNCU_forecast} describes the forecasting model for conventional meters.
    \end{enumerate}
    \item \textbf{Error Variance}
    \begin{enumerate}
        \item Section~\ref{sec:forecast_variance} describes the unbiased variance used in the delivery plan.
    \end{enumerate}
\end{enumerate}


% In addition, ${\bf x}$ represents the vector, and ${\bf{x}^T}$ denotes the transpose of $\bf x$.


\begin{figure}
    \centering
    \includegraphics[width=16cm]{4:DemandPrediction/figs/overall_dp_ver4.png}
    \caption{The overall flow of demand forecast *1 TQ: The third quartile of daily gas usages for a given meter.
*2 TQ\_SM: The maximum value of the third quartile of the daily usages of all customers using smart meters.
 }
    \label{fig:overall_dp}
\end{figure}


\input{4:DemandPrediction/src/complement}
\input{4:DemandPrediction/src/ncu}
\input{4:DemandPrediction/src/nonncu}
\input{4:DemandPrediction/src/variance}

==> history/transportation_research_partC/DemandPrediction/src/ncu.tex <==
\subsection{Demand Forecast for Smart Meters\label{sec:NCU_forecast}}
Let $D_0$ be today date.
We forecast daily gas usages for the next $n_{\rm f}$ days including today $\boldsymbol{\widehat{\rm du}}_{D_0}$.
% $\forall i \in [-n_n-n_s, -n_n]$We use the daily gas usages for the past $(n_{\rm p}+n_{\rm s}-1)$ days $\boldsymbol{{{\rm du}}}_{D_0+i}:= [1, {\rm du}_{D_0+i-1},{\rm du}_{D_0+i-2},\cdots, {\rm du}_{D_0+i-n_{\rm p}}]^T (\forall i \in [-n_{\rm s},-1] \cap \mathbb{Z})$. We also use parameters $\boldsymbol{\beta}:=[\beta_0, \beta_1, \cdots, \beta_{n_{\rm p}}]^T$, and the hyperparameter $\lambda$, which determines the strength of the regularization. 
We prepare $n_{\rm s}$ samples of $\boldsymbol{{{\rm du}}}$, which is a vector of the usage of the past $n_{\rm p}$ days and 1, as
\begin{align*}
    \boldsymbol{\widehat{\rm du}}_{D_0}:&= [\widehat{\rm du}_{D_0}, \widehat{\rm du}_{D_0+1},\cdots \widehat{\rm du}_{D_0+n_{\rm f}-1}]^T\\
    \boldsymbol{{{\rm du}}}_{D_0+i}:&= [1, {\rm du}_{D_0+i-1},{\rm du}_{D_0+i-2},\cdots, {\rm du}_{D_0+i-n_{\rm p}}]^T, \forall i \in [-n_{\rm s},-1] \cap \mathbb{Z}
\end{align*}

The goal of learning demand forecast is to estimate the parameters $\boldsymbol{\beta}:=[\beta_0, \beta_1, \cdots, \beta_{n_{\rm p}}]^T$ so that the usage $\widehat{\rm du}_{D_0}$ forecast from $\boldsymbol{{{\rm du}}}_{D_0+i}$ is close to the actual usages ${\rm du}_{D_0}$ for $\forall i \in [-n_{\rm s},-1] \cap \mathbb{Z}$.
As a result, we can forecast $\boldsymbol{\widehat{\rm du}}_{D_0}$ as
\begin{equation*}
    \begin{aligned}
    \widehat{\rm du}_{{D_0}} &=\beta_0 + \beta_{1}{\rm du}_{D_0-1}+\beta_{2} {\rm du}_{D_0-2}+\cdots+\beta_{n_{\rm p}} {\rm du}_{D_0{-n_{\rm p}}}\\
    \widehat{\rm du}_{D_0+1} &=\beta_0 + \beta_{1} \widehat{\rm du}_{{D_0}}+\beta_{2} {\rm du}_{D_0-1}+\cdots+\beta_{n_{\rm p}} {\rm du}_{D_0-n_{\rm p}+1}\\
& \vdots \\
    \widehat{\rm du}_{D_0+n_{\rm f}-1} &=\beta_0 + \beta_{1} \widehat{\rm du}_{D_0+n_{\rm f}-2}+\beta_{2} \widehat{\rm du}_{D_0+n_{\rm f}-3}+\cdots+\beta_{n_{\rm p}} {\rm du}_{D_0{-n_{\rm p}+(n_{\rm f}-1)}}
    \end{aligned}
\end{equation*}
Note that $\widehat{\rm du}_{D_0+i}(i>0)$ uses the forecast values $\widehat{\rm du}_{D_0+{j}}(0\leq j<i)$.


% We describe the parameter estimation applied to the forecasting. Since smart meters have not been installed for a long period, there are currently not many meter readings available. 
We use statistical and machine learning models to forecast the demand.%, which can be achieved even with little data.
First, statistical models are models that apply statistical analysis to the demand forecast. 
We introduce two popular statistical methods: Linear regression and Support Vector Regression. 
Second, decision-tree-based models such as CART(~\cite{breiman1984classification}) are among the most popular forecasting methods in machine learning. We introduce two models for ensemble learning of decision trees: Random Forest Regression and Gradient Boosting Regression Trees.



\input{4:DemandPrediction/src/ML/LinearRegression}
\input{4:DemandPrediction/src/ML/SupportVectorRegression}
\input{4:DemandPrediction/src/ML/RandomForestRegression}
\input{4:DemandPrediction/src/ML/GradientBoostingRegression}



==> history/transportation_research_partC/DemandPrediction/src/nonncu.tex <==
\subsection{Demand Forecasting for Conventional Meters}\label{sec:NonNCU_forecast}

% kNN予測モデル
\subsubsection{kNN Model}
We propose the demand forecast method for conventional meters based on the prediction results of smart meters.
\label{kNN forecast}
% Let $M^*$ be a conventional meter. 
For the $k-$nearest neighbor meters ${\rm Sim}(\mathcal{M}_s^*, k)$, the weights are $w^{(M_0)}_{\rm norm}$ obtained by normalizing the similarity $w^{(M_0)}$ of $M_0\in {\rm Sim}(\mathcal{M}_s^*, k)$.

\begin{equation}
    w^{(M_0)}_{\rm norm} = \frac{w^{(M_0)}}{\displaystyle \sum_{M'\in {\rm Sim}(M^*, k)}w^{(M')}}
\end{equation}
Let $\{\boldsymbol{\widehat{\rm du}}_{0}^{(M_0)}\}_{M_0\in {\rm Sim}(M^*, k)}$ be the predicted value of the date $D_0$ for each of the meters in ${\rm Sim}(M^*,k)$. 
In this case, the forecast gas usage at $D_0$ for $M^*$ is as follows.
\begin{equation}
    \boldsymbol{\widehat{\rm du}}_{0}^{(M^*)} = \sum_{M_0\in {\rm Sim}(M^*,k)}w^{(M_0)}_{\rm norm} \  \boldsymbol{\widehat{\rm du}}_{0}^{(M_0)}
\end{equation}
This is a weighted average of the forecast gas usage of ${\rm Sim}(M^*, k)$.

% TQ予測モデル
\subsubsection{Forecast for Conventional Meters with High Usages (TQ Model)}
\label{TQ forecast}
The~\ref{kNN forecast} method does not work well for forecasting meters with high gas usage because the gas usage tendency of the $k$-nearest neighbor meters is different from that of $\mathcal{M}_s^*$. In addition, it is not easy to construct an accurate prediction model for a machine learning model that takes complementary values as input because most of the input vectors are complemented values. Therefore, we construct another forecast model that uses the third quartile of its own past daily usage as the forecast gas usage. 
Conventional meters with high gas usage $\mathcal{M}_{c}^{HU}$ are extracted using the method described in Section ~\ref{tq complement}.
For completion, its own third quartile is calculated and used as the forecast gas usage.


\subsubsection{When any Model Fails to Train (AllMean model)}
During actual operation, the training of the above models may not work for some reason. To deal with this, we prepare a simple model, \emph{AllMean model} that outputs the average usage of all meters as the forecast value. AllMean model allows us to output the forecast usage under any situation.

==> history/transportation_research_partC/DemandPrediction/src/variance.tex <==
\subsection{Variance of Forecast Error}\label{sec:forecast_variance}
% By the previous sections, we have forecast the daily usage for all meters in $\mathcal{M}$; however, the forecast accuracy varies from meter to meter. 
% For example, if a meter $M_{\rm high}$ with high accuracy and a meter $M_{\rm low}$ with low accuracy have the same forecast usage $\boldsymbol{\widehat{\rm du}}_0$ on a forecasting day $D_0$, the actual usage $\boldsymbol{{\rm du}}_0$ will be $\left|\boldsymbol{\widehat{\rm du}}_0-\boldsymbol{{\rm du}}_0^{(M_{\rm high})}\right|\leq\left|\boldsymbol{\widehat{\rm du}}_0-\boldsymbol{{\rm du}}_0^{(M_{\rm low})}\right|$.
We estimate the error variance for each meter to make an effective delivery plan that takes forecast errors into account.
We prepare the pair of the forecast usage $\boldsymbol{\widehat{\rm du}}_{D_0-i}$ and the actual usage $\boldsymbol{{\rm du}}_{D_0-i}$ for each date ${\rm mD}(D_0,-i)~(\forall i \in [n_{\rm f},n_{\rm f}+n_{\rm s}]\cap \mathbb{Z})$ during parameter estimation.
\begin{align}
    \boldsymbol{\widehat{\rm du}}_{D_0-i} :&= [\widehat{\rm du}_{D_0-i}, \widehat{\rm du}_{D_0-(i-1)},\cdots \widehat{\rm du}_{D_0-(i-n_{\rm f}+1)}]^T\\
    \boldsymbol{{\rm du}}_{D_0-i}:&= [{\rm du}_{D_0-i}, {\rm du}_{D_0-(i-1)},\cdots, {\rm du}_{D_0-(i-n_{\rm f}+1)}]^T
\end{align}
Let $\boldsymbol{e}_{D_0-i}:=\boldsymbol{{\rm du}}_{D_0-i}-\boldsymbol{\widehat{\rm du}}_{D_0-i}$ be the forecast error. 
Assuming that each $\left \{\boldsymbol{e}_{D_0-i}\right \}_{i}$ independently follows a normal distribution with mean $0$, we estimate the unbiased variance vector $ \boldsymbol{\widehat{\rm dv}}$ as follows
\begin{align}
      \boldsymbol{\widehat{\rm dv}}^{(M)}:= \frac{1}{n_{\rm s}}\sum_{i=n_{\rm f}}^{n_{\rm f}+n_{\rm s}}{(\boldsymbol{e}_{D_0-i}-\bar{\boldsymbol{e}})\odot (\boldsymbol{e}_{D_0-i}-\bar{\boldsymbol{e}})}
      \qquad(\forall M \in \mathcal{M}),
\end{align}
where $n_{\rm f}$ is the number of forecast days, $n_{\rm s}$ is the number of sample, $\bar{\boldsymbol{e}}=\frac{1}{n_{\rm s}}\sum_{i=n_{\rm f}}^{n_{\rm f}+n_{\rm s}}{\boldsymbol{e}_{D_0-i}}$ and $\odot$ means the element-wise product.

% 予測使用量と正解使用量のペア

==> history/transportation_research_partC/Experiment_DLDR/src/exp_ISG.tex <==
\subsection{Verification Experiment}
% プロと比較して提案モデルの有用性を確認した(需要予測/配送計画)
We confirm the effectiveness of our proposed model by comparing it with the conventional model.
In the conventional model, the demand forecast model used in Exp A and Exp C is similar to MaxModel, which has the following features.
\begin{itemize}
    \item The daily gas usage is assumed to be constant.
    \item They pick up the value that the maximum value of average daily usage among five different periods. 
    \item The forecast value is calculated by the above value and the constant value to consider the next period's usage tendency.
\end{itemize}
Moreover, the delivery plan with Exp A and Exp B is manually formulated by the worker's hands based on their experience.

\subsubsection{Settings}
% Table13の説明
We conduct numerical experiments under four different settings, as summarized in Table~\ref{tab:exp_ISG_result_edited}.
The settings of Exp D in this section are the same as those in Exp 3 in Table~\ref{tab:exp_result_edited}.

\begin{table}[htbp]
    \begin{tabular}{c|c|c}
    \centering
        Name  & Demand forecast & Delivery plan \\ \hline
        Exp A & Gas provider    & Gas provider \\
        Exp B & Proposed model  & Gas provider \\
        Exp C & Gas provider    & Proposed model \\
        Exp D (Exp 3 in Section~\ref{sec:exp_dldr}) & Proposed model  & Proposed model 
    \end{tabular}
    \caption{Experimental setting. The result of Exp D in this section is the same as Exp 3 in Table~\ref{tab:exp_result_edited}}
    \label{tab:exp_ISG}
\end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=15cm]{8:Experiment_DLDR/figs/last_modify_2.jpg}
%     \caption{Whether or not received smart meter data, whether or not calculated delivery plan, and whether or not driver's availability. Output date is the date when calculated delivery plan.}
%     \label{fig:last_modify_2}
% \end{figure}

\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
        \begin{tabular}{c}Date\\(2021 March)\end{tabular} & 15th & 16th & 17th & 18th & 19th & 20th & 21st & 22nd & 23rd & 24th     \\ \hline \hline
        \begin{tabular}{c}Received\\smart meter data\end{tabular} & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ &  \\ \hline
        \begin{tabular}{c}Calculate\\delivery plan\end{tabular} & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ &  &  & $\checkmark$ & $\checkmark$ &  \\ \hline
        \begin{tabular}{c}Driver's\\availability\end{tabular}  & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ &  &  & $\checkmark$ & $\checkmark$ &  $\checkmark$ \\ \hline
        \begin{tabular}{c}Output date\\(2021 March)\end{tabular} & & 15th & 16th & 17th & 18th &  &  & 19th & 22nd & 23rd
    \end{tabular}
    \caption{Whether smart meter data are received, whether the delivery plan is calculated, and whether a driver is available are indicated. The output date is when the delivery plan is calculated.}
    \label{tab:last_date}
\end{table}

%実験期間
The target dates are from 16/3/2021 to 24/3/2021.
%計算した結果は翌日の配送に組み込まれる
% The output delivery plan is delivered on the driver's next working day. In other words, the delivery plan output on each execution day is for one day (See Table~\ref{tab:last_date}).
On the target date, we calculate the delivery plan for the next working date.
%ドライバーの働き方
The driver works from Monday to Friday.
The driver loads the cylinders on the truck after the delivery work the previous day but loads the cylinders delivered on Monday after the delivery on Friday. (see Table~\ref{tab:last_date})
%データエラーの件
%However, an error occurred in the data acquisition of the smart meter on 24/3/2021, and the meter reading data of all the smart meters except one could not be received. Therefore, we did not calculate delivery plans after 25/3/2021, and delivery plans for three days of 25/3/2021, 26/3/2021, and 29/3/2021 were output on 24/3/2021.
% Please see Figure \ref{tab:last_date}.
%未交換訪問はなし
During the experiment, it is assumed that non-replacement visits are made.


\subsubsection{Results and Discussion}
We summarize the results of the evaluation metrics in Table~\ref{tab:exp_ISG_result_edited} and use the same evaluation metrics in Section~\ref{sec:dldr_metric}.
We consider the following things based on the results.
%\begin{table}[htbp]
%    \centering
%    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
%        Name & Rate & Success & Fail-out & Fail-over & Fail-time & Visit & Time/customer & Distance/trip & Visit/day \\ \hline
        % 有効数字4桁, 複数ある場合は10%,15%
%        Exp A   &  10.3   \% & 36.3\% & 30.5\% & 33.2\% & 3 & 289 & 12m55s & 41.5km & 41.3 \\
%        Exp B   & 8.83e-05\% & 56.6\% & 38.3\% & 4.68\% & 2 & 235 & 13m30s & 69.6km & 33.6 \\
%        Exp C   & 8.73    \% & 31.3\% & 35.4\% & 33.3\% & 0 & 339 & 13m19s & 64.7km & 48.4 \\
%        Exp D-1 & 2.08    \% & 53.3\% & 36.6\% & 10.9\% & 0 & 347 & 13m06s & 44.7km & 49.6 \\
%    \end{tabular}
%    \caption{The result of evaluation metrics. We omit evaluation metrics as Rate, Success, Fail-out, Fail-over, Fail-time, Visit, Time/customer, Distance/trip and Visit/day.}
%    \label{tab:exp_ISG_result}
%\end{table}

\renewcommand{\arraystretch}{1.5}
\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c|c|c|c}
        Name            & Exp A           & Exp B           & Exp C          & 
        \begin{tabular}{c}
             Exp D  \\
             (Exp 3 in Section~\ref{sec:exp_dldr})
        \end{tabular}
        \\ \hline
        Demand forecast & Gas provider    & Proposed model  & Gas provider   & Proposed model  \\
        Delivery plan   & Gas provider    & Gas provider    & Proposed model & Proposed model  \\ \hline \hline
        Rate-average    & 10.3 \%          & 8.83e-05 \%    & 8.73 \%         & -1.36 \% \\
        Rate-median     & 7.56 \%          & 1.82 \%          &  7.07 \%        & 0.09 \%  \\
        Success      & 36.3 \%          & 56.6 \% & 31.3 \%         & 47.1 \%          \\
        Fail-out        & 30.5 \%          & 38.3 \%          & 35.4 \%         & 45.1 \%          \\
        \textbf{Fail-over(↓)} & 33.2 \%    & \textbf{4.7 \%} & 33.3 \%         & 7.8 \%          \\
        Fail-time(↓)    & 3               & 2               & \textbf{0}     & \textbf{0}      \\
        Visit(↑)        & 289             & 235             & 339            & \textbf{357}    \\
        Time/customer(↓)& 12 m 55 s          & 13 m 30 s          & 13 m 19 s         & \textbf{12 m 05 s}          \\
        Distance/trip(↓)& 41.5 km & 69.6 km          & 64.7 km         & \textbf{37.0 km}          \\
        Visit/day(↑)    & 41.3            & 33.6            & 48.4           & \textbf{51.0}   \\
        \textbf{Run out(↓)}  & 34.4            & 21.7   & 49.7           & \textbf{21.6}
    \end{tabular}
    \caption{Experimental setting and evaluation metrics of the experiment. Rate-average, Rate-median, Success, Fail-out, Fail-over, Fail-time, Visit, Time/customer, Distance/trip, Visit/day and Run out are abbreviations for the evaluation metrics introduced in Section~\ref{sec:dldr_metric}, respectively. 
    As the criterion for Fail-over is that the remaining gas rate at replacement is over 15\%. 
    The results of Exp D in this section are the same as those in Exp 3 in Table~\ref{tab:exp_result_edited}.}
    \label{tab:exp_ISG_result_edited}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=15cm]{8:Experiment_DLDR/figs/outLCs_new.png}
    \caption{The number of customers whose gas has run out during the target period. Note that the lines overlap if the numbers are the same for two consecutive days.}
    \label{fig:outLCs}
\end{figure}

% \subsubsection{Discussion}
\begin{enumerate}
    \item (\textbf{Demand Forecast}) Comparison of our proposed model with a conventional method for demand forecasting. 
    In both Exp A and Exp B, the delivery plan is made by the gas provider. 
    In Exp A, the gas provider executes the demand forecast, whereas our proposed model in Exp B conducts it.
    \begin{itemize}
        \item Rate-median in Exp B is lower than Exp A. 
        With our proposed model for demand forecasting, the gas provider can deliver to customers with a low remaining gas rate. 
        % It can be said that the proposed model is better in demand forecast.
        The results show the superiority of our proposed model in a demand forecast task.
    \end{itemize}
    \item  (\textbf{Delivery Plan}) Comparison of our proposed model and the conventional method for delivery planning. Based on the demand forecast result of the gas provider, the delivery plan is made by the gas provider and our proposed model in Exp A and Exp C, respectively.
    \begin{itemize}
        \item Distance of Exp C is longer than that of Exp A.
        Because our model focuses on the visit to high-risk customers with the highest priority, the delivery route occasionally becomes longer than the delivery plan of the gas provider.
        Exp C records the most Run out events owing to the accuracy of the demand forecast. 
        \item In Exp C, as shown in the Figure~\ref{fig:outLCs}, the number of customers with Run out events increases. 
        Many high-risk customers are owing to the imprecise demand forecast.
        It causes many high-risk customers and some non-high-risk customers, but they are determined as high-risk customers.
        When the number of trips is too large, we extract some trips to calculate the delivery route.
        The result indicates that non-high-risk customers are extracted, whereas an actual high-risk customer included in the delivery list is not extracted.
        Thus, the number of high-risk customers increases over time.
        It implies that the quality of the delivery plan can be improved by modifying the selection among many high-risk customers, which is one of our future work.
        % This suggests that the quality of the demand forecast is sensitive to the quality of the delivery plan.
        % because they have large high-risk customers.
        % However, there is no method to distinguish between real high-risk customers and non-high-risk customers with plenty of gas in reality.
        % It is because the gas provider tends to avoid long-distance customers while the proposed model focuses on visiting high-risk customers with the highest priority.
        % There are many Run out, which is derived from the demand forecast accuracy.
        % However, it can be said that the proposed model is better in that it has a lower Rate and more Visit.
    \end{itemize}
    \item (\textbf{Demand Forecast and Delivery Plan}) In Exp D, the delivery plan is created using our proposed model based on its demand forecast.
    \begin{itemize}
        \item Exp D is more successful than Exp A in terms of all evaluation metrics.
        % Rate decreases because customers with a high remaining gas rate in Exp A are not targeted for delivery.  
        % Since our model focuses on the visit to high-risk customers with the highest priority, Exp D achieves a lower Rate compared to Exp A.
        % On the contrary, by focusing the delivery to high-risk customers, Exp D is unavoidable the longer trip than Exp A, which can be understood by Time/customer and Distance/trip.
        % It is because the gas provider tends to avoid long-distance customers while the proposed model focuses on visiting high-risk customers with the most priority.
        Exp A records the least Fail-out visits; however, this is mainly because they leave out the existence of the customers with a gas shortage (see Figure~\ref{fig:outLCs}).
        % While Fail-out is the best result in Exp A, and they leave the existence of the customer with a gas shortage as shown in Figure \ref{fig:outLCs}. 
        % It indicates that Fail-out is not perfect evaluation metrics, and we evaluate the delivery plan by combining some evaluation metrics.
        By contrast, Exp D visits the high-risk customers, as shown in Figure~\ref{fig:outLCs}. 
        These tendencies can be observed by comparing the Run out events between Exp A and Exp D.
        \item Exp D achieved a smaller number of customers with Run out events and competitive results in terms of Fail over events compared to Exp B.
        It indicates that our proposed model can realize a better delivery plan similar to that of a gas provider.
        Moreover, the Time/customer and Distance/trip in Exp D achieve a much better performance than Exp B.
        We prepare for a future increase in high-risk customers by delivering to moderate-risk customers, which can be understood as the slope occurring near March 22nd in Figure~\ref{fig:outLCs}.
        Figure~\ref{fig:outLCs} shows that Exp D achieves the least increase in the number of customers experiencing a gas shortage.
        In other words, a larger number of Fail-out events indicates that delivery is assured to the customer after running out of gas.
        Because the Rate-median of Exp D is lower than Exp A and Exp C, Exp D tends to deliver to customers who are about to run out of gas.
        \item Through our proposed model, more efficient delivery is realized than Exp C for every evaluation metric. 
        The number of Run out events can be dramatically reduced in Exp D based on the better demand forecast.
        \item In Exp D, more Fail-out visits are observed. 
        By contrast, Exp D succeeds in reducing the number of Run out events compared to Exp A.
        Exp D focuses more on delivery to high-risk customers, which causes the accumulation of Run out events deceased.
        The least Rate-median is reported in Exp D, indicating that its focus is on delivery to high-risk customers in Exp D.
    \end{itemize}
    In conclusion, when our proposed model is utilized for both a demand forecast and delivery plan (Exp D), the quality of the delivery can be understood as the highest.
    It is because Exp D achieves the best result of Run out and the second-best result in Fail-over.
    Moreover, it succeeds in making an efficient delivery plan which can be understood by Time/customer or Distance/trip.
\end{enumerate}

==> history/transportation_research_partC/Experiment_DLDR/src/exp_dldr.tex <==
\subsection{Comparing Proposed Model with Different Parameters \label{sec:exp_dldr}}
\subsubsection{Evaluation Settings}
We compare the vehicle routing plan when changing the parameters.
We change only one parameter while fixing the other parameters.
The basic information of the customers is summarized as follows:
\begin{enumerate}
    \item The number of Customers: $|\mathcal{C}|=1,366$
    \item The number of Customers with smart meters: $|\{C \in \mathcal{C}| C \in \mathcal{M}_s\}|=861$
\end{enumerate}


%The experimental settings are summarize in Table \ref{tab:exp_settings}.
The experimental settings are summarized in Table~\ref{tab:exp_result_edited}.
%\begin{table}[htbp]
%    \centering
%    \begin{tabular}{c|c|c|c|c|c|c}
%        Name & $\alpha, q^*$ & $\beta, q'$ & look back dates & Trip division & Delivery List \\ \hline %& Delivery Route\\ \hline
%        Exp1 & 5\%, 0.3 & 7\%, 0.3 & 2 & FAVA & multiBB \\%& IP-based \\
%        Exp2 & 5\%, 0.5 & 7\%, 0.5 & 2 & FAVA & multiBB \\%& IP-based \\
%        Exp3 & 0\%, 0.3 & 7\%, 0.3 & 2 & FAVA & multiBB \\%& IP-based \\
%        Exp4 & 5\%, 0.3 & 7\%, 0.3 & 0 & FAVA & multiBB \\%& IP-based \\
%        Exp5 & 5\%, 0.3 & 7\%, 0.3 & 2 & updated binpacking & multiBB \\%& IP-based \\
%        Exp6 & 5\%, 0.3 & 7\%, 0.3 & 2 & FAVA & DLGreedy \\%& IP-based \\
%        Exp7 & 5\%, 0.3 & 7\%, 0.3 & 2 & FAVA & maxRisk \\%& IP-based \\
%        Exp8 & 5\%, 0.3 & 7\%, 0.3 & 2 & FAVA & minBB & \\%IP-based \\
%        %Exp9 & 5\%, 0.3 & 7\%, 0.3 & 2 & FAVA & multiBB & TSP-based \\
%    \end{tabular}
%    \caption{Hyperparameter settings for each experimental settings. ($\alpha, q^*$) and ($\beta, q'$) are the threshold to extract high-risk and moderate-risk customer, respectively.}
%    \label{tab:exp_settings}
%\end{table}

\subsubsection{Evaluation Metrics \label{sec:dldr_metric}}
We calculate the following evaluation metrics to investigate the quality of the delivery plan.
Delivery time includes replacing cylinders at customers' places because we do not know the time required for replacement during the experiment.
The abbreviations in the parentheses are used to summarize results in Table~\ref{tab:exp_result_edited}.
\begin{itemize}
    %交換時残ガス率(平均)
    \item The average remaining gas rate at replacement (Rate-average)
    %交換時残ガス率の中央値
    \item The median of remaining gas rate at replacement (Rate-median)
    %配送成功LC数の割合：全体-失敗
    \item Total success rate, excluding failures (Success)
    %配送失敗LC数割合(0%以下)
    \item The rate of failure in replacement owing to a cylinder being out of gas (Fail-out)
    %配送失敗LC数割合(15%以上)
    \item The rate of failure in replacement due to an overabundance of gas (Fail-over)
    %配送失敗LC数(時間指定), 少ないので割合ではなく数にしています
    \item The number of failures in replacement owing to the time window of the customer (Fail-time)
    %配送LC数合計
    \item The number of visiting customers (Visit) 
    \begin{itemize}
        \item During the experiment, we assume that there are no non-replacement visits. 
        We can determine that some non-replacement visits must occur when Rate is larger than 8\% following the gas provider's rule.
        \item Because many customers whose remaining gas is below 0\% at the beginning of the experiment, a more Visit is beneficial.
    \end{itemize}
    %1LCあたりの配送時間(分秒)
    \item Delivery time per customer (Time/customer)
    %1トリップあたりの配送距離(km)：実験ABにおいて配送回数が1回の日があるのでday→tripに変更
    \item Travel distance per trip (Distance/trip)
    %1日あたりの配送LC数
    \item The number of visiting customers per day (Visit/day)
    %残ガス率が0%を下回っている需要家数の平均
    \item The average number of customers whose gas has run out (Run out)
\end{itemize}

\subsubsection{Results and Discussion}
% 実験Dの結果
We summarize the results of the evaluation metrics of the experiments in Table~\ref{tab:exp_result_edited}, which enables us to consider the following things,
%\begin{table}[htbp]
    %\centering
%    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
%        Name & Rate & Success & Fail-out & Fail-over & Fail-time & Visit & Time/customer & Distance/trip & Visit/day \\ \hline
    % 有効数字4桁
%        Exp1 &  2.08\% & 53.3\% & 36.6\% & 10.1\% & 0 & 347 & 13m06s & 44.7km & 49.6 \\
%        Exp2 & -0.88\% & 50.1\% & 41.1\% & 8.70\% & 1 & 345 & 13m00s & 43.8km & 49.3 \\
%        Exp3 & -1.36\% & 47.1\% & 45.1\% & 7.84\% & 0 & 357 & 12m05s & 37.0km & 51.0 \\
%        Exp4 &  1.16\% & 52.5\% & 36.9\% & 10.6\% & 1 & 320 & 13m38s & 46.1km & 45.7 \\
%        Exp5 &  1.03\% & 51.7\% & 38.6\% & 9.71\% & 0 & 350 & 13m01s & 43.3km & 50.0 \\
%        Exp6 &  0.28\% & 48.3\% & 38.9\% & 12.9\% & 0 & 373 & 11m09s & 30.6km & 53.3 \\
%        Exp7 &  0.35\% & 50.3\% & 39.2\% & 10.5\% & 0 & 344 & 11m38s & 33.0km & 49.1 \\
%        Exp8 &  0.49\% & 47.7\% & 38.9\% & 13.4\% & 0 & 350 & 11m24s & 31.1km & 50.0 \\
%        Exp9 &  0.83\% & 53.0\% & 36.6\% & 10.4\% & 0 & 336 & 13m01s & 43.2km & 48.0 \\
%    \end{tabular}
%    \caption{Evaluation metrics of the experiment. We omit evaluation metrics as Rate, Success, Fail-out, Fail-over, Fail-time, Visit, Time/customer, Distance/trip and Visit/day. The criterion for Fail-over is that the remaining gas rate at replacement is 15\%.}
%    \label{tab:exp_results}
%\end{table}

%秦追記 要修正（はみだす)
%片岡追記 閾値の()を除去, binpacking, ルートのBasedを消すことで対応
\renewcommand{\arraystretch}{1.5}
\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c|c|c|c|wc{15mm}|c|c|c}
        Name & Exp 1 & Exp 2 & Exp 3 & Exp 4 & Exp 5 & Exp 6 & Exp 7 & Exp 8     \\ \hline %&Exp9
        $\alpha, q^*$ & 5 \%, 0.3 & 5 \%, \framebox[1.1\width]{0.5} & \framebox[1.1\width]{0 \%}, 0.3 & 5 \%, 0.3 & 5 \%, 0.3 & 5 \%, 0.3 & 5 \%, 0.3 & 5 \%, 0.3 \\%& 5\%, 0.3  \\
        $\beta, q'$ & 7 \%, 0.3 & 7 \%, \framebox[1.1\width]{0.5} & 7 \%, 0.3 & 7 \%, 0.3 & 7 \%, 0.3 & 7 \%, 0.3 & 7 \%, 0.3 & 7 \%, 0.3  \\%& 7\%, 0.3  \\
        {\it look back} dates  & 2 & 2 & 2 & \framebox[1.1\width]{0} & 2 & 2 & 2 & 2  \\%& 2  \\
        Trip division & FAVA & FAVA & FAVA & FAVA &
        \renewcommand{\arraystretch}{1.0}
        \framebox[0.8\width]{\begin{tabular}{c}updated\\binpacking\end{tabular}}
        \renewcommand{\arraystretch}{1.5} & FAVA & FAVA & FAVA  \\%& FAVA  \\
        Delivery list & multiBB & multiBB & multiBB & multiBB & multiBB & \framebox[1.1\width]{DLGreedy} & \framebox[1.1\width]{maxRisk} & \framebox[1.1\width]{minBB} \\[5pt] \hline \hline
        %Delivery Route & IP       & IP & IP & IP & IP & IP & IP & IP & TSP \\ \hline \hline
        Rate-average & 2.08 \% & -0.88 \% & -1.36 \% & 1.16 \% & 1.03 \% & 0.28 \% & 0.35 \% & 0.49 \%  \\%&  0.83\%  \\
        Rate-median & 4.10 \% & 2.57 \% & 0.09 \% & 3.87 \% & 3.32 \% & 2.81 \% & 2.41 \% & 2.42 \% \\
        Success & 53.3 \% & 50.1 \% & 47.1 \% & 52.5 \% & 51.7 \% & 48.3 \% & 50.3 \% & 47.7 \%  \\%& 53.0\%  \\
        Fail-out & 36.6 \% & 41.1 \% & 45.1 \% & 36.9 \% & 38.6 \% & 38.9 \% & 39.2 \% & 38.9 \%  \\%& 36.6\%  \\
        \textbf{Fail-over(↓)} & 10.1 \% & 8.7 \% & \textbf{7.8 \%} & 10.6 \% & 9.7 \% & 12.9 \% & 10.5 \% & 13.4 \%  \\%& 10.4\%  \\
        Fail-time(↓) & \textbf{0} & 1 & \textbf{0} & 1 & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0}  \\%& 0  \\
        Visit(↑) & 347 & 345 & 357 & 320 & 350 & \textbf{373} & 344 & 350  \\%& 336  \\
        Time/customer(↓) & 13m06s & 13m00s & 12m05s & 13m38s & 13m01s & \textbf{11m09s} & 11m38s & 11m24s  \\%& 13m01s  \\
        Distance/trip(↓)& 44.7 km & 43.8 km & 37.0 km & 46.1 km & 43.3 km & \textbf{30.6 km} & 33.0 km & 31.1 km  \\%& 43.2km  \\
        Visit/day(↑) & 49.6 & 49.3 & 51.0 & 45.7 & 50.0 & \textbf{53.3} & 49.1 & 50.0 \\%& 48.0 \\
        \textbf{Run out(↓)} & 28.1 & 31.6 & \textbf{21.6} & 26.6 & 28.6 & 35.3 & 29.2 & 29.6 \\
    \end{tabular}
    \caption{Hyperparameter settings for each experimental settings and evaluation metrics of the experiment. Pairs of $\alpha, q^*$, and $\beta, q'$ are the thresholds for extracting high- and moderate-risk customers, respectively. Rate-average, Rate-median, Success, Fail-out, Fail-over, Fail-time, Visit, Time/customer, Distance/trip, Visit/day, and Run out are abbreviations for the evaluation metrics introduced in Section~\ref{sec:dldr_metric}.  As the criterion for failure, the remaining gas rate at replacement was over 15\%. The differences in the settings between Exp 1 and the others are highlighted by the surrounding rectangles. The best results are presented in bold.}
    \label{tab:exp_result_edited}
\end{table}
\renewcommand{\arraystretch}{1.0}

% \paragraph{Discussion}
\begin{enumerate}
    \item ($\boldsymbol{q^*, q^{'}}$) The difference between Exp 1 and Exp 2 is the threshold of determining the high-risk and moderate-risk customers.
    The experiments aim to observe the effect of considering the risk function defined in Section~\ref{sec:risk_func}.
    \begin{itemize}
        \item Exp 1 succeeds in increasing on the Success and decreasing the Fail-out but fails to increase a Fail-over.
        Because $q^*$ and $q'$ are smaller in Exp 1, customers are more likely to be included in the delivery list than Exp 2.
        We can observe a smaller Fail-out by decreasing the parameter $q^*$ and $q^{'}$, which shows the effectiveness of considering the risk function described in Section~\ref{sec:risk_func}.
    \end{itemize}
    \item ($\boldsymbol{\alpha}$) Exp 3 especially sets the remaining gas rate to 0\%, whereas Exp 1 sets it as the 5\%.
    \begin{itemize}
        \item There are fewer Run out and Fail-over events in Exp 3 compared to Exp 1.
        Because $\alpha$ is less in Exp 3, we can focus on delivering to the customer who is about to experience Run out event than in Exp 1.
        In other words, Exp 1 is more likely to be delivered to customers whose remaining gas is not about to below 0\% even they are high-risk customers.
        The result indicates that we can focus on delivering to the customers with a specific gas rate by changing $\alpha$.
        % \item Run out is decreased by set $\alpha$ is 0\%.
        % This is because Exp 3 can focus on delivering to customers with out of gas while Exp 1 can deliver the customer where it does not happen gas shortage.
        %is later to become a high-risk customer, Fail-out increased.
        % These Fail-out are derived from the forecast and complement error or situation that the impossible to deliver the all high-risk customer.
        % In the current proposed model, the result tells us that it is not appropriate that the threshold $\alpha$ is set to zero for reducing gas shortage.
        % In Exp 3, $\alpha$ is 0\%. Therefore, the timing of becoming a high-risk consumer is later than that in Exp. 1. Therefore, the failure rate increases.
    \end{itemize}
    \item (\textbf{\it look back} dates) Exp 4 does not force to add more moderate-risk customers without considering {\it look back} dates, aiming to reveal the effectiveness of {\it look back} dates.
    \begin{itemize}
        \item Based on the definition of {\it look back} dates, the number of moderate-risk customers is increasing.
        Significantly, some customers are in the moderate-risk customer in Exp 1. 
        However, they are not moderate-risk customers in Exp 4.
        These customers enable us to obtain a smaller delivery area than in Exp 4.
        Such customers even have a low risk of experiencing a gas shortage.
        Therefore, more Run-out events in Exp 1 are reported, with a larger number of Visit and shorter Distance/trip.
        However, when there are few high- and moderate-risk customers, we can obtain more candidates for delivery by considering the {\it look back} dates.
        It is one of the promising techniques for realizing workload leveling.
        % Considering look back dates, it is possible to deliver to moderate-risk customers.
        % The closer these moderate-risk customers are to high-risk customers, the easier it will be to deliver.
        %Therefore, Visit is larger and Distance/trip is shorter than not considering. 
        %This customer difference can be the cause that Fail-out decreased and Fail-over increased. 
        %The influence of considering look back dates is slight compared to other parameters.
    \end{itemize}
    \item (\textbf{Algorithm for trip division}) Exp 5 utilizes the updated bin packing problem, whereas Exp 1 applies the FAVA model for the trip division.
    \begin{itemize}
        % \item Contrary to our expectation, Exp1 has a larger Distance/Trip than Exp5.
        % Trip division is given as the initial solution of multiBB.
        % However, it is thought that Exp 5 can search for a better solution than Exp1.
        \item The two models are competitive owing to all evaluation metrics.
        It indicates that the influence of changing the trip division is slight when compared to the other parameters.
    \end{itemize}
    \item (\textbf{Algorithms to get delivery list}) The difference among Exp 1 and Exp 6–8 is used in the delivery list model. Exp 1, Exp 6, Exp 7, and Exp 8 utilize multiBB, DLGreedy, maxRisk, and minBB, respectively.
    \begin{itemize}
        % \item Compared Exp 6, 7 and 8, Distance/trip are longer in Exp 1. However, it achieves the least Run out because Exp 1 utilizes the multiBB. 
        \item Distance/trip of Exp 1 is longer than Exp 6, 7, and 8, which suggests that considering the long-term optimal delivery plan is ineffective in terms of Distance/trip.
        However, Exp 1 achieved the best result regarding Fail-over and Run out events, which is the most important aspect for evaluating the quality of the delivery plan.
        % \item Exp 1 also achieves the least number of Fail-over events through workload leveling using multiBB.
        \item Exp 6 records the most number of Visit events compared to Exp 1, 7, and 8.
        It is derived from the candidate moderate-risk customers, which are larger in number than Exp 1, 7, and 8.
        In Exp 7, the moderate-risk customer can be visited only when included in ellipses focusing on any two high-risk customers.  
        Exp 1 and 8 set the lower bounds of the number of cylinders in which the moderate-risk customer must be visited.
        In other words, multiBB (Exp 1) and minBB (Exp 8) acquire the delivery list only for high-risk customers without setting the lower bounds.
        In these experiments, there are more spaces to be loaded in the results of Exp 1 or Exp 8, even though Exp 6 tries to load as much as possible.
        Although Exp 6 has the most Visit events, the number of Run out events is worse than the others.
        It happens if there are many trips, and the final output of the trip contains many moderate-risk customers compared to high-risk customers. 
        % \item Visit of Exp 7 is smaller than Exp 6, which is derived from the fact that not all moderate-risk customers can be visited in Exp 7.
        % Exp 7 delivers moderate-risk customers within an ellipse that focuses on any two high-risk customers.  
        % There are some moderate-risk customers delivered in Exp 6 are not included in the ellipse in Exp 7. 
        % Therefore, Exp6 has more Visit than Exp 7. 
        % Distance/trip is also shorter in Exp 7 because it is closer to the high-risk customers than Exp 6 by targeting the moderate-risk customers in the ellipse.
        % When the number of trip is too large, we extract few trips due to the limited work availability.
        % This is because when the number of trips are too large, we extract the trips. 
        % This situation in Exp 8 happens that the extracted trips contain many moderate-risk customers while non-extracted trips do less moderate-risk customers.
        % MultiBB is a more complex problem than minBB. 
        % It may not be possible to find a suitable solution with multiBB because the time limit is the same.
        \item In Exp 8, Distance/trip is shorter than in Exp 1 because minimizing the delivery area for multiple days is not implemented when formulating the delivery list. As a result, when both delivery list problems in Exp 1 and Exp 8 obtain optimal solutions, the delivery list of the first day in Exp 8 is equal to or smaller than that in Exp 1. Therefore, Exp 1 recorded worse results than Exp 8 in terms of Time/customer and Distance/trip.
    \end{itemize}
    In conclusion, Exp 3 achieves the best results in Fail-over and Run out events and has the best hyperparameter settings between Exp 1 and Exp 8.
%    \item The effect of delivery route algorithm (Exp1 v.s. Exp9)
%    \begin{itemize}
%        \item There are not any significant changes in terms of Success or Fail. In addition, there is almost no difference in the algorithm for formulating the output of the delivery route. One day, the only difference is with Exp1 being the solution in Section \ref{sec:tsp} and Exp9 being the solution in Section \ref{sec:squeeze}. However, customers delivered are different, which is expected to be the cause of the differences between Rate and Visit.
%    \end{itemize}
\end{enumerate}

% 実験E
% \subsubsection{Additional experiment}
% In the experiment, there are many high-risk customers on the first day of the experiment.
% Therefore, we think that the goal of delivering as much as possible to moderate-risk customers would be challenging for a limited period.
% As shown in Figure \ref{fig:outLC_D}, the number of customers whose gas is running out during the target period is a lot.
% It means that Fail-out is high due to these customers.
% We conducted the additional experiment only in Exp 1 after deleting 69 customers with less than 10\% gas remaining as the first day of the experiment.
% We summarize the result of evaluation metrics of the additional experiments in Table \ref{tab:expE_result_edited}.
% As shown in Figure \ref{fig:outLC_DvsE}, customers whose remaining gas rate falls below 0 \% during the target period decreased.
% Moreover, it reduces Fail-out and makes it easier to deliver to moderate-risk customers, thus increasing Rates and Fail-over.
% \begin{figure}
%     \centering
%     \includegraphics[width=15cm]{8:Experiment_DLDR/figs/outLC_D.png}
%     \caption{The number of customers whose gas rate is running out during the target period in Exp D. Note that the lines overlap if the numbers are the same for two consecutive days.}
%     \label{fig:outLC_D}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=15cm]{8:Experiment_DLDR/figs/outLC_DvsE.png}
%     \caption{The number of customers whose gas is running out during the target period in the additional experiment.}
%     \label{fig:outLC_DvsE}
% \end{figure}
% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c|c|c}
%         Name             & Exp 1            & Exp 3 additional \\ \hline
%         $\alpha, q^*$    & 5\%, 0.3        & 0\%, 0.3        \\
%         $\beta, q'$      & 7\%, 0.3        & 7\%, 0.3        \\
%         look back dates   & 2               & 2               \\
%         Trip division    & FAVA            & FAVA            \\
%         Delivery List    & multiBB         & multiBB         \\
%         Delete customers &  -              & $\checkmark$         \\ \hline \hline
%         Rate             &  2.08\%         & \textbf{3.85\%} \\
%         Success (↑)       & 53.3\%          & \textbf{55.9\%} \\
%         Fail-out (↓)      & 36.6\%          & \textbf{27.2\%} \\
%         \textbf{Fail-over (↓)}     & \textbf{10.1\%} & 16.9\%          \\
%         Fail-time (↓)     & \textbf{0}      & \textbf{0}      \\
%         Visit (↑)         & \textbf{347}    & 331             \\
%         Time/customer (↓) & 13m06s          & \textbf{12m512s} \\
%         Distance/trip (↓) & 44.7km          & \textbf{35.8km} \\
%         Visit/day (↑)     & \textbf{49.6}   & 47.3            \\
%         \textbf{Running out(↓)}      & 28.1            & \textbf{9.2}  \\
%     \end{tabular}
%     \caption{Experimental setting and evaluation metrics of the additional experiment. Rate, Success, Fail-out, Fail-over, Fail-time, Visit, Time/customer, Distance/trip and Visit/day are abbreviations for the evaluation metrics introduced in Section \ref{sec:dldr_metric}, respectively. Rate should be close to $\alpha$. The criterion for Fail-over is that the remaining gas rate at replacement is over 15\%.}
%     \label{tab:expE_result_edited}
% \end{table}


% 実験Eの結果
%\begin{table}[htbp]
%    \centering
%    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
%        Name & Rate & Success & Fail-out & Fail-over & Fail-time & Visit & Time/customer & Distance/trip & Visit/day \\ \hline
    % 有効数字4桁
%        Exp1 & 4.67\% & 59.8\% & 22.4\% & 17.8\% & 0 & 321 & 12m51s & 39.3km & 45.9 \\
%        Exp2 & 3.83\% & 65.1\% & 23.8\% & 11.1\% & 0 & 324 & 13m20s & 43.6km & 46.3 \\
%        Exp3 & 3.85\% & 55.9\% & 27.2\% & 16.9\% & 0 & 331 & 12m12s & 35.8km & 47.3 \\
%        Exp4 & 4.52\% & 63.2\% & 21.7\% & 15.1\% & 0 & 318 & 13m04s & 40.7km & 45.4 \\
%        Exp5 & 4.67\% & 59.8\% & 22.4\% & 17.8\% & 0 & 321 & 12m51s & 39.3km & 45.9 \\
%        Exp6 & 3.29\% & 61.9\% & 26.2\% & 11.9\% & 0 & 328 & 12m00s & 33.9km & 46.9 \\ 
%        Exp7 & 2.74\% & 60.4\% & 27.2\% & 12.3\% & 0 & 316 & 11m57s & 32.1km & 45.1 \\
%        Exp8 & 3.85\% & 60.8\% & 26.6\% & 12.6\% & 0 & 342 & 11m48s & 33.2km & 48.9 \\
%        Exp9 & 3.57\% & 60.9\% & 25.8\% & 13.4\% & 0 & 322 & 12m59s & 40.6km & 46.0 \\
%    \end{tabular}
%    \caption{Evaluation metrics of the additional experiment. We omit evaluation metrics as Rate, Success, Fail-out, Fail-over, Fail-time, Visit, Time/customer, Distance/trip and Visit/day. The criterion for Fail-over is that the remaining gas rate at the replacement is 15\%.}
%    \label{tab:expE_results}
%\end{table}


==> history/transportation_research_partC/Experiment_DLDR/src/exp_dldr_main.tex <==
% \clearpage
\section{Numerical Experiment of Delivery Plan \label{sec:exp_dldr}}

\input{8:Experiment_DLDR/src/exp_dldr}
\input{8:Experiment_DLDR/src/exp_ISG}

==> history/transportation_research_partC/Experiment_DP/src/complement.tex <==
\subsection{Evaluation of Complementary Accuracy \label{sec:exp_polation}}
We evaluate the accuracy of $interpolation$ and $extrapolation$ of the complementary algorithm introduced in Sections~\ref{sec:complement} and ~\ref{sec:comp_NonNCU}. 
The experimental data are generated by intentionally missing the data of the target meters. 
In the {\it interpolation} experiments, we first pick up the target date, and we remove the data for $n_{\rm m}$ successive days before the target date, not including the target date. 
In the {\it extrapolation}, we remove the cumulative usages of the previous $n_{\rm m}$ successive days, including the target date.
 The two missing periods $n_{\rm m}$ are one day and 30 days and are label {\it Short} and {\it Long}, respectively. {\it Short} and {\it Long} are set because the most frequent missing interval for smart meters is one day. 
The most frequent missing interval for houses without a smart meter is 29 days.
% In addition, we added $Moderate$ as an intermediate value between $Short$ and $Long$.
In the above $4$ patterns ($2$ patterns of $interpolation$ or $extrapolation$ $\times$ $2$ patterns of $Short$ and $Long$), we experimented with four completion algorithms: Linear, Periodic, Similar, and kNN.
\subsubsection{Evaluation Settings}
% １日ごとの使用量のヒストグラム
% We show the histogram of daily gas usage in Figure xxx.
Data used for experiments are summarized as follows,
\begin{enumerate}
    \item Data : Cumulative daily meter readings (regular meter readings sent from smart meters) 
    % \begin{itemize}
    %     \item Cumulative daily meter readings (regular meter readings sent from smart meters) 
    %     \item Gas cylinder replacement data (irregular meter readings, including conventional meters)
    % \end{itemize}
    \item the Target dates $\mathcal{D}^*$ : $\{1/2/2021, 2/2/2021, \cdots, 14/3/2021\}$ ($|\mathcal{D}^*|=42$)
    \item the Target meters $\mathcal{M}^*_s$ :
    619 smart meters that have never been missing data in the target dates
    \item the Number of Missing Cumulative Usages $n_{\rm m}$ : $1$~({\it Short}) or $30$~({\it Long})
\end{enumerate}

\subsubsection{Evaluation Metrics}
For each meter $M\in \mathcal{M}_s^*$ , the evaluation metric is calculated as,
\begin{align}
\dsp \mathrm{RMSE}\,(M)= \sqrt{\frac{1}{|\mathcal{D}^*|\times (n_{\rm m}+\delta)}\sum_{D\in\mathcal{D}^*}\sum_{i=1}^{n_{\rm m}+\delta}\left(\widehat{\rm du}_{D-i}^{(M)}-{\rm du}_{D-i}^{(M)}\right)^2}
\quad
\delta =
\left\{
\begin{array}{l}
1 \quad Interpolation \\
0 \quad Extrapolation
\end{array}
\right.
\end{align}
 where the complemented daily usage is $\widehat{\rm du}_{D+i}^{(M)}$ and the actual measured daily usage is ${\rm du}_{D+i}^{(M)}$ for $M \in 
\mathcal{M}_s^*$.
% ($\delta=1$ if {\it Interpolation}, and $\delta=0$ if {\it Extrapolation})
We obtain the mean, median and maximum values after calculating the RMSE of every customer.
% \begin{enumerate}
%     \item $\dsp \mathrm{MAE}\,(M)=\frac{1}{|\mathcal{D}^*|\times N} \sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t-N-\delta}^{t-\delta}\left|\widehat{\rm du}_{D+i}^{(M)}-\mu_{D+i}^{(M)}\right|$
%     \item $\dsp  \mathrm{R^2}\,(M)= 1-\frac{\dsp  \sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t-N-\delta}^{t-\delta}(\widehat{\rm du}_{D+i}^{(M)}-\mu_{D+i}^{(M)})^2}{\dsp  \sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t-N-\delta}^{t-\delta}(\bar{\mu}^{(M)}-\mu_{D+i}^{(M)})^2} ~  \left(\bar{\mu}^{(M)}=\frac{1}{|\mathcal{D}^*|\times N}\sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t-N-\delta}^{t-\delta}{\mu_{D+i}^{(M)}}\right)$
%     \item $\dsp \mathrm{RMSE}\,(M)= \sqrt{\frac{1}{|\mathcal{D}^*|\times N}\sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t-N-\delta}^{t-\delta}\left|\widehat{\rm du}_{D+i}^{(M)}-\mu_{D+i}^{(M)}\right|}$
%     \item $\dsp \mathrm{MAPE}\,(M)=\frac{100}{|\mathcal{D}^*| \times N} \sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t-N-\delta}^{t-\delta}\left|\frac{\widehat{\rm du}_{D+i}^{(M)}-\mu_{D+i}^{(M)}}{\bar{\mu}}\right| ~ \left(\bar{\mu}=\frac{1}{|\mathcal{M}^*| \times |\mathcal{D}^*| \times N}\sum_{M\in\mathcal{M}^*}\sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t-N-\delta}^{t-\delta}{\mu_{D+i}^{(M)}}\right)$
% \end{enumerate}
% A lower $\mathrm{MAE}$, $\mathrm{RMSE}$ and $\mathrm{MAPE}$ values are better, whereas a higher $\mathrm{R^2}$ value is better.

 
\subsubsection{Results and Discussion}
% The results of the experiments on completion are shown in Figure ~\ref{fig:exp1-1_in,fig:exp1-1_ex,fig:exp1-2_in,fig:exp1-2_ex,fig:exp1-3_in,fig:exp1-3_ex} and Table \ref{table:exp1-1_in},\ref{table:exp1-1_ex},fig:exp1-2_in,fig:exp1-2_ex,fig:exp1-3_in,fig:exp1-3_ex. %TODO
We show the experiment results of {\it Interpolation} in Figure~\ref{fig:exp1-1_in} and Table~\ref{table:exp1-1_in}.
These results enable us to consider the following things,

\begin{enumerate}
    
    
\item The RMSE values of Linear and Periodic are smaller than those of Similar and kNN. 
It indicates that it is more effective to use the meter's own previous data.
\item The RMSE value of Linear is equal to or lower than Periodic value because the maximum error between the measured value and the predicted value by Linear is smaller than Periodic. 
A detailed explanation is provided in Figure~\ref{fig:discussion_dp}.
%  because Linear interpolation connects the meter readings before and after the missing data with a straight line.
\end{enumerate}

Next, we show the experimental results of {\it Extrapolation} in Figure~\ref{fig:exp1-1_ex} and Table~\ref{table:exp1-1_ex}.
We also consider the following things,
\begin{enumerate}
    \item Similar and kNN shows better results than Linear and Periodic. We can see that it is more effective to use other meters' data.
    \item The RMSE value of kNN is smaller than that of Similar. It shows the effectiveness of weighting according to similarity.
    \item Although Linear has a higher RMSE value, it is expected that the risk of running out of gas is smaller because Linear uses the TQ value as the complementary value. 
    Therefore, Linear can be chosen when safety is judged to be more critical, as Section~\ref{tq complement}.
\end{enumerate}
In summary, Linear and kNN have the best accuracy in terms of Interpolation and Extrapolation complement, respectively.

% 1. 実験shortの内挿

\begin{figure}
    \centering
    \includegraphics[width=15cm]{7:Experiment_DP/figs/interpolation.png}
    \caption{Violin plot of RMSE values in the {\it interpolation}. The left table shows the results for the {\it Short} term, and the right table shows the results for the {\it Long} term.}
    \label{fig:exp1-1_in}
\end{figure}

\begin{table}[]
\begin{tabular}{crrrlcrrr}

\multicolumn{1}{c|}{Short}     & \multicolumn{1}{c|}{Mean}   & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Maximum} &  & \multicolumn{1}{c|}{Long}     & \multicolumn{1}{c|}{Mean}       & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Maximum} \\ \cline{1-4} \cline{6-9} 
\multicolumn{1}{c|}{Linear}   & \multicolumn{1}{r|}{\textbf{0.1271}} & \multicolumn{1}{r|}{\textbf{0.1142}} & 0.4716                      &  & \multicolumn{1}{c|}{Linear}   & \multicolumn{1}{r|}{\textbf{0.4028}} & \multicolumn{1}{r|}{\textbf{0.3110}} & \textbf{2.8635}                      \\
\multicolumn{1}{c|}{Periodic}   & \multicolumn{1}{r|}{0.1315} & \multicolumn{1}{r|}{0.1166} & \textbf{0.4600}                      &  & \multicolumn{1}{c|}{Periodic}   & \multicolumn{1}{r|}{0.4109} & \multicolumn{1}{r|}{0.3227} & 2.9171                      \\
\multicolumn{1}{c|}{Similar}   & \multicolumn{1}{r|}{0.1878} & \multicolumn{1}{r|}{0.1673} & 0.8658                      &  & 
\multicolumn{1}{c|}{Similar}   & \multicolumn{1}{r|}{1.4926} & \multicolumn{1}{r|}{0.9735} & 19.5941                       \\
\multicolumn{1}{c|}{kNN}   & \multicolumn{1}{r|}{0.1870} & \multicolumn{1}{r|}{0.1672} & 0.8492                      &  & 
\multicolumn{1}{c|}{kNN}   & \multicolumn{1}{r|}{1.4696} & \multicolumn{1}{r|}{0.9751} & 19.5145                      \\
\end{tabular}
\caption{The RMSE values for each complementary method during the {\it Interpolation}. The left table shows the results for the {\it Short} term, and the right table shows the results for the {\it Long} term.} 
\label{table:exp1-1_in}
\end{table}







% 2. 実験shortの外挿

\begin{figure}
    \centering
    \includegraphics[width=15cm]{7:Experiment_DP/figs/extrapolation.png}
    \caption{Violin plot of RMSE values during the {\it Extrapolation}. The left figure shows the results for the {\it Short} term, and the right figure shows the results for the {\it Long} term.}
    \label{fig:exp1-1_ex}
\end{figure}

\begin{table}[]
\begin{tabular}{crrrlcrrr}
\multicolumn{1}{c|}{Short}     & \multicolumn{1}{c|}{Mean}   & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Maximum} &  & \multicolumn{1}{c|}{Long}     & \multicolumn{1}{c|}{Mean}       & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Maximum} \\ \cline{1-4} \cline{6-9} 
\multicolumn{1}{c|}{Linear}   & \multicolumn{1}{r|}{0.2063} & \multicolumn{1}{r|}{0.1826} & 1.3320                      &  & 
\multicolumn{1}{c|}{Linear}   & \multicolumn{1}{r|}{2.5965} & \multicolumn{1}{r|}{1.7372} & 24.6073                            \\
\multicolumn{1}{c|}{Periodic}   & \multicolumn{1}{r|}{0.2588} & \multicolumn{1}{r|}{0.2280} & 1.2304                      &  & 
\multicolumn{1}{c|}{Periodic}   & \multicolumn{1}{r|}{3.9113} & \multicolumn{1}{r|}{2.9453} & 28.6447                      \\
\multicolumn{1}{c|}{Similar}   & \multicolumn{1}{r|}{0.1867} & \multicolumn{1}{r|}{\textbf{0.1671}} & 0.8757                      &  & 
\multicolumn{1}{c|}{Similar}   & \multicolumn{1}{r|}{1.4755} & \multicolumn{1}{r|}{0.9629} & 19.2096                          \\
\multicolumn{1}{c|}{kNN}   & \multicolumn{1}{r|}{\textbf{0.1860}} & \multicolumn{1}{r|}{0.1672} & \textbf{0.8579}                      &  & 
\multicolumn{1}{c|}{kNN}   & \multicolumn{1}{r|}{\textbf {1.4528}} & \multicolumn{1}{r|}{\textbf {0.9520}} & \textbf {19.1322}                                   \\
\end{tabular}
\caption{The RMSE values for each complement method during the {\it Extrapolation}. The left table shows the results for the {\it Short} term, and the right table shows the results for the {\it Long} term.}
\label{table:exp1-1_ex}
\end{table}



==> history/transportation_research_partC/Experiment_DP/src/exp_dp.tex <==
% \subsection{Evaluation for prediction accuracy}
% We evaluate the accuracy of $interpolation$ and $extrapolatio$n of the completion algorithm introduced in Section~\ref{sec:complement} and Section~\ref{sec:comp_NonNCU}. The experimental data is generated by intentionally missing the data of the target customer. In the case of interpolation, the data from the day before the forecasting date to $N$ days before the forecasting date is missing, and in the case of extrapolation, the data from the day of the forecasting date to $N-1$ days before the forecasting date is missing. The three missing periods $N$ is 1 day, 15 days, and 30 days, and are named $Short$, $Moderate$, and $Long$, respectively. $Short$ and $Long$ are set because the most frequent missing interval for customers with smart meters is 1 day, and the most frequent missing interval for customers without smart meters is 29 days. In addition, we added $Moderate$ as an intermediate value between $Short$ and $Long$. In the above $6$ patterns ($2$ patterns of $interpolation$ or $extrapolation$ $\times$ $3$ patterns of $Short$, $Moderate$, and $Long$), we experimented with four completion algorithms: Linear, Periodic, Similar, and kNN.
% \subsubsection{Evaluation Settings}
% \begin{enumerate}
%     \item Data
%     \begin{itemize}
%         \item Cumulative daily meter readings (regular meter readings sent from smart meters) 
%         \item Gas cylinder exchange data (irregular meter readings, including those of customers without smart meters) 
%     \end{itemize}
%     \item the Forecasting Days $\mathcal{D}$ : $\{1/2/2021, \cdots, 14/3/2021\}$ ($|\mathcal{D}|=42$)
%     \item Set of Target Meters $\mathcal{M}$ :
%     619 customers with smart meters that have never been missing data in the forecasting days
% \end{enumerate}

% \subsubsection{Evaluation Metrics}
% For the complemented day $i$, the accuracy was calculated using the following four evaluation indices, where the complemented daily usage is $\hat{\mu}_i^h$ and the actual measured daily usage is $\mu_i^h$ for $h \in \mathcal{M}$. ($\sigma=1$ if $interpolation$, and $\sigma=0$ if $extrapolation$)

% \begin{enumerate}
%     \item $\mathrm{MAE}\,(h)=\frac{1}{|\mathcal{D}|\times N} \sum_{t=\min{\mathcal{D}}}^{\max{\mathcal{D}}}\sum_{i=t-N-\delta}^{t-\delta}\left|\hat{\mu}_i^h-\mu_i^h\right|$
%     \item $\mathrm{R^2}\,(h)= 1-\frac{\sum_{t=\min{\mathcal{D}}}^{\max{\mathcal{D}}}\sum_{i=t-N-\delta}^{t-\delta}(\hat{\mu}_i^h-\mu_i^h)^2}{\sum_{t=\min{\mathcal{D}}}^{\max{\mathcal{D}}}\sum_{i=t-N-\delta}^{t-\delta}(\bar{\mu}^h-\mu_i^h)^2}\,\,(\bar{\mu}^h=\frac{1}{|\mathcal{D}|\times N}\sum_{t=\min{\mathcal{D}}}^{\max{\mathcal{D}}}\sum_{i=t-N-\delta}^{t-\delta}{\mu_i^h})$
%     \item $\mathrm{RMSE}\,(h)= \sqrt{\frac{1}{|\mathcal{D}|\times N}\sum_{t=\min{\mathcal{D}}}^{\max{\mathcal{D}}}\sum_{i=t-N-\delta}^{t-\delta}\left|\hat{\mu}_i^h-\mu_i^h\right|}$
%     \item $\mathrm{MAPE}\,(h)=\frac{100}{|\mathcal{D}| \times N} \sum_{t=\min{\mathcal{D}}}^{\max{\mathcal{D}}}\sum_{i=t-N-\delta}^{t-\delta}\left|\frac{\hat{\mu}_i^h-\mu_i^h}{\bar{\mu}}\right| \,\, (\bar{\mu}=\frac{1}{|\mathcal{M}| \times |\mathcal{D}| \times N}\sum_{h\in\mathcal{M}}\sum_{t=\min{\mathcal{D}}}^{\max{\mathcal{D}}}\sum_{i=t-N-\delta}^{t-\delta}{\mu_i^h})$
% \end{enumerate}
% A lower $\mathrm{MAE}$, $\mathrm{RMSE}$ and $\mathrm{MAPE}$ values are better, whereas a higher $\mathrm{R^2}$ value is better.
 
% \subsubsection{Discussion}

==> history/transportation_research_partC/Experiment_DP/src/exp_dp_main.tex <==
\section{Numerical Experiment in Demand Forecast \label{sec:exp_dp}}


\input{7:Experiment_DP/src/exp_dp}
% \clearpage
\input{7:Experiment_DP/src/complement}
% \clearpage
\input{7:Experiment_DP/src/forecast}

% \clearpage
\input{7:Experiment_DP/src/predict_hard_date}


==> history/transportation_research_partC/Experiment_DP/src/forecast.tex <==
\begin{figure}
    \centering
    \includegraphics[width=15cm]{7:Experiment_DP/figs/discussion_dp.png}
    \caption{Case in which the sum of the errors is maximum in the interpolation of Linear and Periodic. In Linear, the maximum is the gray triangle shown on the left because a straight line connects the meter readings before and after the missing data. In Periodic, the worst-case is the gray rectangle, as shown on the right. Therefore, the Periodic's maximum of the sum of errors is greater than that of Linear.}
    \label{fig:discussion_dp}
\end{figure}

\subsection{Evaluation for Forecasting Accuracy \label{sec:exp_forecast}}
The accuracy of the demand forecast presented in Sections ~\ref{sec:NCU_forecast} and~\ref{sec:NonNCU_forecast} is evaluated for meters with and without smart meters, respectively. 
As a baseline, we prepare MaxModel, which takes the maximum value of the most recent daily usage as the predicted value. Then, experiments for smart meters are compared with MaxModel, LR, SVR, RFR, and GBRT.
The coefficient of the regularization term of LR as 0.5, max depth of RFR as 4, and the other hyperparameters of each model apply the default values of sklearn \cite{scikit-learn}. 
For the experiment of conventional meters, data generation is conducted by intentionally missing the data of the target meters every 29 days. 
Thus, this is the maximum frequency of the missing data of meters without a smart meter. 
Using these data, we compare the results with MaxModel, kNN, TQ, and AllMean. 


\subsubsection{Evaluation Settings}
\begin{enumerate}
    \item Data : Cumulative daily meter readings (regular meter readings sent from smart meters) 
    % \begin{itemize}
        % \item 
    %     \item Gas cylinder exchange data (irregular meter readings, including those of conventional meters) 
    % \end{itemize}
    \item the Target Dates $\mathcal{D}^*$ : $\{1/2/2021, \cdots, 14/3/2021\}$ ($|\mathcal{D}^*|=42$)
    \item the Target Meters $\mathcal{M}^*_s$ :
    619 smart meters that have never been missing data in the target dates
    \item the Number of Input Days $n_{\rm p}$: 7
    \item the Number of Samples $n_{\rm s}$ : 14
    \item the Number of Output Days $n_{\rm f}$: 9
\end{enumerate}

\subsubsection{Evaluation Metrics}
For the target date $i$, the evaluation metric is calculated as,
\begin{align*}
\dsp \mathrm{RMSE}\,(M)= \sqrt{\frac{1}{|\mathcal{D}^*|\times n_{\rm f}}\sum_{D\in\mathcal{D}^*}\sum_{i=0}^{n_{\rm f}-1}\left(\widehat{{\rm du}}_{D+i}^{(M)}-{\rm du}_{D+i}^{(M)}\right)^2}
\end{align*}
where the forecast daily usage is $\widehat{{\rm du}}_{D+i}^{(M)}$ and the actual usage is ${\rm du}_{D+i}^{(M)}$ for $M \in \mathcal{M}_s^*$.
We obtain the mean, median and maximum values after calculating the RMSE of each meter.

% \begin{enumerate}
    % \item $\dsp \mathrm{MAE}\,(M)=\frac{1}{|\mathcal{D}^*|\times L} \sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t}^{t+L-1}\left|\widehat{{\rm du}}_{D+i}^{(M)}-{\rm du}_{D+i}^{(M)}\right|$
    % \item $\dsp \mathrm{R^2}\,(M)= 1-\frac{\dsp \sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t}^{t+L-1}(\widehat{{\rm du}}_{D+i}^{(M)}-{\rm du}_{D+i}^{(M)})^2}{\dsp \sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t}^{t+L-1}(\bar{\mu}^{(M)}-{\rm du}_{D+i}^{(M)})^2} ~ \left(\bar{\mu}^{(M)}=\frac{1}{|\mathcal{D}^*|\times L}\sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t}^{t+L-1}{{\rm du}_{D+i}^{(M)}}\right)$
    % \item $\dsp \mathrm{RMSE}\,(M)= \sqrt{\frac{1}{|\mathcal{D}^*|\times L}\sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t}^{t+n_{\rm f}-1}\left|\widehat{{\rm du}}_{D+i}^{(M)}-{\rm du}_{D+i}^{(M)}\right|}$
    % \item $\dsp \mathrm{MAPE}\,(M)=\frac{100}{|\mathcal{D}^*| \times L} \sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t}^{t+L-1}\left|\frac{\widehat{{\rm du}}_{D+i}^{(M)}-{\rm du}_{D+i}^{(M)}}{\bar{\mu}}\right| ~  \left(\bar{\mu}=\frac{1}{|\mathcal{M}^*| \times |\mathcal{D}^*| \times L}\sum_{h\in\mathcal{M}^*}\sum_{t=\min{\mathcal{D}^*}}^{\max{\mathcal{D}^*}}\sum_{i=t}^{t+L-1}{{\rm du}_{D+i}^{(M)}}\right)$
% \end{enumerate}
% A lower $\mathrm{MAE}$, $\mathrm{RMSE}$ and $\mathrm{MAPE}$ values are better, whereas a higher $\mathrm{R^2}$ value is better.

\subsubsection{Results and Discussion}

First, we show the experimental results for smart meters on the left side of Figure~\ref{fig:NCU_forecasting} and in Table~\ref{table:NCU_forecasting}.
We consider the following things based on the results.
\begin{enumerate}
    \item The RMSE values of the four introduced models are smaller than those of the baseline MaxModel.
    \item Although the SVR and RFR are both highly accurate, the maximum value of the RMSE is the smallest for the SVR. 
    It shows that the SVR is more robust to outliers.
\end{enumerate}


Next, we show the experimental results for conventional meters on the right side of Figure~\ref{fig:NCU_forecasting} and in Table~\ref{table:NCU_forecasting}.
\begin{enumerate}
    \item The RMSE values of the proposed models are smaller than those of the baseline MaxModel.
    \item The RMSE values of the kNN are the smallest.
    It indicates that when we extract similar meters, the forecast period is also similar to that of the meters.
    \item Although TQ has a higher RMSE value, it is expected that the risk of running out of gas is smaller because TQ uses the meters' own historical third quartile as the forecast values. 
    Therefore, TQ can be chosen when safety is judged to be critical, as indicated in Section~\ref{tq complement}
\end{enumerate}

In summary, SVR/kNN achieves the highest accuracy in demand forecasts for meters with and without smart meters.



% \subsection{Result}
\begin{figure}
    \centering
    \includegraphics[width=15cm]{7:Experiment_DP/figs/forecasting.png}
    \caption{Violin plot of RMSE values in the demand forecasting. Because MaxModel records much worse results than the others, we exclude it in the figure. The left table shows the results of the demand forecast methods for smart meters, and the table on the right shows the results of the demand forecast methods for conventional meters.
    Both experiments are conducted with the smart meters because the evaluation data is quite small when we experiment with the demand forecast methods for conventional meters with the data of conventional meters.}
    \label{fig:NCU_forecasting}
\end{figure}
\begin{table}[]
\begin{tabular}{crrrlcrrr}

\multicolumn{1}{c|}{SM}     & \multicolumn{1}{c|}{Mean}   & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Maximum} &  & \multicolumn{1}{c|}{nonSM}     & \multicolumn{1}{c|}{Mean}       & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Maximum} \\ \cline{1-4} \cline{6-9} 
\multicolumn{1}{c|}{MaxModel}   & \multicolumn{1}{r|}{1.3628} & \multicolumn{1}{r|}{0.4227} & 2.165e+02                      &  & 
\multicolumn{1}{c|}{MaxModel}   & \multicolumn{1}{r|}{1.3628} & \multicolumn{1}{r|}{0.4227} & 2.165e+02                          \\
\multicolumn{1}{c|}{LR}   & \multicolumn{1}{r|}{0.5863} & \multicolumn{1}{r|}{0.4598} & 10.3792                      &  & 
\multicolumn{1}{c|}{kNN}   & \multicolumn{1}{r|}{\textbf {0.3795}} & \multicolumn{1}{r|}{\textbf {0.3478}} & \textbf {1.3350}                      \\
\multicolumn{1}{c|}{SVR}   & \multicolumn{1}{r|}{\textbf {0.3867}} & \multicolumn{1}{r|}{0.3590} & \textbf {1.4437}                      &  & 
\multicolumn{1}{c|}{TQ}   & \multicolumn{1}{r|}{0.4243} & \multicolumn{1}{r|}{0.3632} & 2.5515                      \\
\multicolumn{1}{c|}{RFR}   & \multicolumn{1}{r|}{0.3885} & \multicolumn{1}{r|}{\textbf {0.3570}} & 1.6324                      &  & 
\multicolumn{1}{c|}{AllMean}   & \multicolumn{1}{r|}{0.7722} & \multicolumn{1}{r|}{0.6084} & 4.0473                      \\
\multicolumn{1}{c|}{GBRT}   & \multicolumn{1}{r|}{0.4495} & \multicolumn{1}{r|}{0.4087} & 1.7484                      &  & 
   &      &  &                    \\
\end{tabular}
\caption{The RMSE values for each forecast model. The left table shows the results of the demand forecast methods for smart meters, and the table on the right shows the results of the demand forecast methods for conventional meters. Both experiments are conducted with the smart meters because the evaluation data is quite little when we experiment with the demand forecast methods for conventional meters with the data of conventional meters.
}
\label{table:NCU_forecasting}

\end{table}






==> history/transportation_research_partC/Experiment_DP/src/predict_hard_date.tex <==
\subsection{Evaluation of Predicting the Date of Becoming High-risk Customers}

In Sections~\ref{sec:exp_polation} and~\ref{sec:exp_forecast}, the proposed models are evaluated along with RMSE.
However, when we evaluate the result of the demand forecast when considering that it is utilized for making the delivery plan, we must prepare the other evaluation metric.
Therefore, we observe how many days are different between the number of dates from becoming the high-risk houses in reality and those forecast through machine learning.

\subsubsection{Evaluation Settings}
We extract houses that do not have missing values from 1/4/2020 to 23/3/2021.
We acquire the date from when the remaining gas rate falls below the threshold of remaining gas rate in the date units. 
Then, starting from the date seven days before the date, the demand forecast and the risk function are used to calculate the date when the house becomes a high-risk house.
During the experiment, the threshold of the gas rate is set to 5\%.
In some settings, we intentionally erase the meter data by utilizing the real missing data.
We prepare the following three settings to investigate the performance of demand forecasting models, the interpolation models, and the extrapolation models.
\begin{itemize}
    \item Exp1: We utilize the complete data without intentionally making missing data. 
    Because the setting is assumed for houses with smart meters, we utilize the five demand forecast models: MaxModel(baseline), LR, SVR, RFR, and GBRT.
    \item Exp2: The data are intentionally removed based on an actual missing probability of houses with smart meters, 0.181\%. This experiment aims at determining the influence of interpolation and extrapolation. Every house is determined to become a high-risk house after interpolating the missing data. 
    Because the setting is also assumed for houses with smart meters, we utilize the same demand forecast models as Exp1.
    \item Exp3: The data are intentionally removed every 29 days. This experiment aims at determining the influence of long-term interpolation and extrapolation. 
    Because the setting is assumed for houses without smart meters, we utilize the two demand forecast models: TQ and kNN. In addition, we execute NoEx: based on the Exp3 experimental setting; we do not utilize complementing missing values but actual measurements.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=13cm]{7:Experiment_DP/figs/predhard/CM_7_cumulativeFalse_danger0.05_thres0.5.png}
    \caption{The result in predicting the date for becoming a high-risk house with the threshold of the integral value $\beta$ of 0.5.}
    \label{fig:predhard_0.5}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=13cm]{7:Experiment_DP/figs/predhard/CM_7_cumulativeFalse_danger0.05_thres0.3.png}
    \caption{The result in predicting the date of becoming a high-risk customer with the threshold for an integral value $\beta$ of 0.3}
    \label{fig:predhard_0.3}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=13cm]{7:Experiment_DP/figs/predhard/CM_7_cumulativeFalse_danger0.05_thres0.01.png}
    \caption{The result in predicting the date of becoming a high-risk customer with the threshold for an integral value $\beta$ of 0.01}
    \label{fig:predhard_0.01}
\end{figure}

\subsubsection{Results and Discussion}
The experimental results for each model are shown in Figures ~\ref{fig:predhard_0.5},~\ref{fig:predhard_0.3}, and~\ref{fig:predhard_0.01}.
Our observations are summarized as follows,
\begin{itemize}
    \item Exp1: SVR and RFR have the fewest errors in predicting the date to becoming a high-risk house, and SVR is the best when comparing the model. When the threshold for the integral value is 0.5, the distribution of the predicted days is near symmetrical.
    Therefore, some customers are predicted to be high-risk customers lately by one day compared to the correct day to be high-risk customers.
    To mitigate this situation, we can make the customer a high-risk customer earlier by decreasing the threshold $q$.
    We experimentally observe that the distribution of the days predicted to be a high-risk house is shifted earlier by one day with a threshold $q$ of 0.01. 
    Under this situation, the rate of customer prediction to be late for the actual date (particularly after seven days) decreases from 28\% to 10 \% when $q$ changes from 0.5 to 0.01.
    \item Exp2: Most of the results are the same as in Exp1, which suggests no significant influences on the prediction performance per day due to the short-term missing data.
    \item Exp3: The accuracy in predicting the date of becoming a high-risk house is not as high as Exp 1 or Exp 2 due to the fewer data acquired.
    We observe the difference by focusing on the existence of extrapolation.
    Although the actual day is most frequently observed when extrapolation is applied, a more tailed distribution of the predicted days is observed.
    The prediction result of the kNN in Exp 3 is better than LR in Exp 1 without an extrapolation, and the distribution becomes skewed.
    Therefore, an extrapolation can significantly affect the accuracy, and a demand forecast model with non-smart meters can predict the dates.
\end{itemize}


In addition, the results of the experiment on a change in threshold show that the most accurate model in each experiment is the SVR in Exp 1, SVR in Exp 2, and kNN in Exp 3, and kNN w.o. extrapolation in Exp 3, as shown in Figures~\ref{fig:predhard_exp1_svr},~\ref{fig:predhard_exp2_svr},~\ref{fig:predhard_exp3_kNN}, and~\ref{fig:predhard_exp3_kNN_NoEx}, respectively.
We can observe that customers become high-risk customers earlier as the threshold decreases.
Users can freely choose the threshold value based on these figures.

\begin{figure}
    \centering
    \includegraphics[width=13cm]{7:Experiment_DP/figs/predhard/CM_7_cumulativeFalse_danger0.05_exp1_SVR.png}
    \caption{The prediction result using SVR when changing the threshold value in Exp1}
    \label{fig:predhard_exp1_svr}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=13cm]{7:Experiment_DP/figs/predhard/CM_7_cumulativeFalse_danger0.05_exp2_SVR.png}
    \caption{The prediction result using SVR when changing the threshold value in Exp2}
    \label{fig:predhard_exp2_svr}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=13cm]{7:Experiment_DP/figs/predhard/CM_7_cumulativeFalse_danger0.05_exp3_kNN.png}
    \caption{The prediction result using kNN when changing the threshold value in Exp3}
    \label{fig:predhard_exp3_kNN}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=13cm]{7:Experiment_DP/figs/predhard/CM_7_cumulativeFalse_danger0.05_exp3_kNN_NoEx.png}
    \caption{The prediction result using kNN when changing the threshold value in Exp3}
    \label{fig:predhard_exp3_kNN_NoEx}
\end{figure}



==> history/transportation_research_partC/Field_Test/src/field_test.tex <==
We execute the verification experiment in the Chiba prefecture in Japan.
The delivery plan of our proposed model is applied and compared with the records of the delivery plan.

\subsection{Evaluation Settings}
The experimental settings are summarized in Table~\ref{tab:FT_result_edited}.
The numbers of experimental period's days are the same.
Because the gas usage depends heavily on the temperature, the comparison periods are extracted based on the average temperature.
% The comparison periods are different because the average temperature of each target period used when calculating the gas density is close.
Temperature data is obtained from the Japan Meteorological Agency website\footnote{\url{http://www.data.jma.go.jp/obd/stats/etrn/index.php}}.
The match rate is the rate at which the gas provider delivered in reality according to the output of our proposed model.
The gas provider occasionally change our proposed model outputs of its customers. %, such as laundromats, supermarkets, and hotels.
\begin{table}[hbp]
    \centering
    \begin{tabular}{c|c|c|c|c}
        $\alpha, q^*$ & $\beta, q'$ & {\it look back} dates & Trip division & Delivery list  \\ \hline
        $5 \%, 0.3$ & $7 \%, 0.3$ & $2$ & FAVA & multiBB
    \end{tabular}
    \caption{Hyperparameter settings in the field test. The settings are same as the Exp-1 in the Section~\ref{sec:exp_dldr}, because it is assumed to be the basic setting of proposed model. However, the results of experiments in Section~\ref{sec:exp_dldr} suggests that there is better parameter settings, Exp-3. 
    Because experiments in Section~\ref{sec:exp_dldr} are conducted after the field test, we pick up the basic settings of hyperparameters in the field test. With parameters in Exp-3, it is promising to obtain better results in the field test.}
    \label{tab:FTsetting}
\end{table}
Hyperparameter settings in the field test are summarized in Table~\ref{tab:FTsetting}.

%\begin{table}[htbp]
%    \centering
%    \begin{tabular}{c|c|c|c}
%        Name           & Period              & Average temperature & Match rate\\ \hline
%        Gas provider   & 13/3/2020-27/3/2020 & 9.7$^\circ$C        & - \\
%        Proposed model &  1/3/2021-15/3/2021 & 9.8$^\circ$C        & 83.9\% 
%    \end{tabular}
%    \caption{}
%    \label{tab:FT_setting}
%\end{table}

\subsection{Evaluation Metrics \label{sec:FT_metric}}
We investigate the quality of the delivery plan with the following evaluation metrics.
These metrics are different from those in Section~\ref{sec:dldr_metric}.
"Travel time per day" and "Travel time per customer" do not include the time required to replace the cylinders at the visiting customers and visit non-replacement customers, that is, the driving time of the truck.
In addition, we calculate  "Total weight of delivered cylinders" and "Total weight of delivered cylinders per delivery".% as reference values. 
% This is because the weight and number of the cylinders of the customers do not always match.
The abbreviations in the parentheses indicate the evaluation metrics for a summary in a table.
The average number of customers whose gas has run out cannot be compared owing to missing data.
\begin{itemize}
    %1日あたり配送員総移動時間
    \item Travel time per day (Travel-time/day)
    %1配送あたり移動時間
    \item Travel time per customer (Travel-time/customer)
    %配送回数
    \item Total number of visited locations with a replacement (Visit)
    %未交換訪問回数
    \item Total number of visited non-replacement locations (Non-replacement)
    %配送可能数量(kg)
    \item Total weight of delivered cylinders (Weight)
    %1配送あたりの配送可能数量(kg)
    \item Total weight of delivered cylinders per customer (Weight/customer)
\end{itemize}

\subsection{Results and Discussion}
The abbreviations in the parentheses indicate the evaluation metrics for summary in Table~\ref{tab:FT_result_edited}.
Based on the results, our observations are follows,


%\begin{table}[htbp]
%    \centering
%    \begin{tabular}{c|c|c|c|c|c|c}
%        Name       & Travel-time/day(↓)  & Travel-time/customer(↓) & Visit & Non-replacement(↓) & Quantity & Quantity/customer \\ \hline
%        Past       & 2h52m32s & 3m46s & 431 & 78 & 2.75e+04kg & 54.0kg\\
%        Field Test & 2h06m44s & 2m34s & 512 & 0* & 2.85e+04kg & 55.7kg
%     \end{tabular}
%    \caption{The result of evaluation metrics. We omit evaluation metrics as Travel-time/day, Travel-time/customer, Replaced, Non-replacement, Quantity and Quantity/customer.}
%    \label{tab:FT_result}
%\end{table}

\renewcommand{\arraystretch}{1.5}
\begin{table}[hbp]
    \centering
    \begin{tabular}{c|c|c}
        Name                    & Gas provider        & Proposed model      \\ \hline
        Period                  & 13/3/2020-27/3/2020 & 1/3/2021-15/3/2021  \\
        Average temperature     & 9.7 $^\circ$C        & 9.8 $^\circ$C        \\
        Match rate              & -                   & 83.9 \%              \\ \hline \hline
        Travel-time/day(↓)      & 2 h 52 m 32 s            & \textbf{2 h 06 m 44 s}   \\
        Travel-time/customer(↓) & 3 m 46 s               & \textbf{2 m 34 s}      \\
        Visit(↑)                & 431                 & \textbf{512}        \\
        Non-replacement(↓)      & 78                  & $\textbf{0}^{*1}$ \\
        Weight(↑)             & 2.75e+04 kg          & \textbf{2.85e+04 kg} \\
        Weight/customer(↑)    & 54.0 kg              & \textbf{55.7 kg}     \\
    \end{tabular}
    \caption{Experimental setting and evaluation metrics of the field test. Travel-time/day, Travel-time/customer, Visit, Non-replacement, Weight and Weight/customer are abbreviations for the evaluation metrics introduced in Section~\ref{sec:FT_metric}, respectively. Because the average number of customers whose gas has run out cannot be compared owing to missing data, Run out is not evaluated.}
    \label{tab:FT_result_edited}
\end{table}

% \subsubsection{Discussion}
\begin{itemize}
    \item Our proposed model performs better than the gas provider for all evaluation metrics. 
    Our proposed model increases the Visit and reduces the Travel-Time and Non-replacement events.
    \item The gas provider's staff is penalized by the gas provider when the average remaining gas rate at the replacement exceeds 8\% per month. 
    In the field test, we ask the gas provider to avoid not replacing the gas cylinder by understanding better how many cylinders do not require non-replacement. 
    After finishing the field test, the average remaining gas rate is below 8\%.
    Therefore, we determine that there are no Non-replacement visits. (See *1 in Table~\ref{tab:FT_result_edited})
    % the number of customers thinned out until the average remaining gas rate at the replacement reaches 8\% will be calculated as equivalent to Non-replacement.  However, the average remaining gas rate at the replacement was below 8\%, and there were no customers equivalent to Non-replacement. (*1 in Table~\ref{tab:FT_result_edited})
\end{itemize}
Our proposed model reduces the delivery costs compared to the gas provider, as shown in Table~\ref{tab:FT_result_edited}.


==> history/transportation_research_partC/Field_Test/src/field_test_main.tex <==
% \clearpage
\section{Field Test \label{sec:field_test}}

\input{9:Field_Test/src/field_test.tex}


==> history/transportation_research_partC/Introduction.tex <==
\section{Introduction}

% 一般的な配送計画問題
Route optimization discovers the optimal routing design (distribution process from depots to customers) without violating any problem-specific constraints, such as time-related, safety-related, and environmental restrictions. 
In recent years, researchers have actively studied this area because of its theoretical interest, economic, and environmental importance (~\cite{raeesi2019multi,bektacs2011pollution, transmodal2012dg}), as well as the emergence of diverse real-life applications (~\cite{sacramento2019adaptive, liang2020automated}).
Enterprises have also raised serious concerns about this issue because they can rarely obtain economic and human resources owing to the rapid increase in travel costs.
Fortunately, recent advances in information and communications technologies (ICT), such as the growing use of GPS technologies, demand monitoring systems, and Internet computing technologies, facilitate more realistic and sometimes multi-objective optimization.
For example, a smart meter has emerged, which is set to the house, and it sends the cumulative gas consumption to the gas provider once a day.

%LPガス配送における課題
This study addresses the problem of liquefied petroleum gas (LP gas) replacement planning. 
Gas is a resource that is necessary for people to live. 
The gas is filled in cylinders, which are depleted as the gas is used. 
The gas company visits each customer approximately once a month to check the meter and replace the gas cylinder when the gas is about to run out. 
% There are two significant problems that can occur with a gas cylinder replacement service, i.e., the gas can run out, which means that it is too late to visit the customer, 
% and a large number of visits without a replacement can occur. 
Two significant problems can occur with a gas cylinder replacement service. 
The first problem is that the gas can run out, which means that it is too late to visit the customer. 
By contrast, it is also a problem a large number of visits without a replacement.
A customer is visited without a replacement when there is too much gas left. 
Although the customer does not run out of gas, the delivery services incur additional costs. 
Therefore, we need an algorithm to make an efficient delivery plan without causing out-of-gas and non-replacement visits.


%提案モデルについて
We propose an algorithm for developing an efficient LP gas delivery plan in which smart meters are installed at the homes of specific customers. 
The basic strategy of the proposed model is to classify customers into high-, moderate-, and low-risk customers according to their risk of running out of gas based on the forecasting of the remaining cylinder capacity.
Then, we always deliver to the high-risk customers and deliver to the moderate-risk customers as much as possible to achieve an efficient delivery in the long term.

%スマートメーター設置について
There are three main challenges in optimal delivery planning for replacing LP gas cylinders.
The first challenge is derived from an imbalance in the frequency of the data acquisition. 
It is necessary to forecast the daily usage for determining the date for gas cylinder replacement. 
However, for conventional meters, only monthly meter reading data have been available until now, making it extremely difficult to forecast daily usage. 
% The gas company saw this situation as a problem and have started to install smart meters. 
Recently, the gas company has started installing smart meters.
By transmitting daily meter readings through smart meters, it is possible to obtain daily usage data, which is expected to reduce out-of-gas and non-replacement visits. 
However, because smart meters are not completely widespread, two-thirds of customers have only conventional meters in our target area. 
The cumulative gas usage of these customers can be acquired approximately once a month.
We have to construct demand forecast models for these meters with an imbalance in the data acquisition frequency. 
We propose a demand forecast model conventional meters based on the demand forecast result for smart meters by utilizing the concept of the kNN algorithm.
% In addition, some customers cannot obtain the daily usage due to missing meter readings caused by communication errors.
% Therefore, the complement method must be utilized before executing the demand forecast.
%, so even customers with smart meters may obtain the data as frequently as customers with conventional meters.

% 危険度関数について
The second challenge is determining the customers to visit by considering the errors in the demand forecast.
While errors in usage forecast always occur, they must prevent an out-of-gas event from occurring.
It happens when forecast usage is much smaller than the actual usage.
We propose a new method for judging the customer based on the inference result and the demand forecast accuracy when considering a normal distribution.
Even if the forecast remaining gas level is the same, we can visit a customer with more insufficient demand forecast accuracy earlier than a customer with better accuracy.


% 長期的な工数平準化について
The third challenge is to realize the long-term optimal delivery plan.
Because the one-day delivery plan influences the delivery plan of the other day, optimal long-term planning is needed.
% When we greedily obtain the optimal delivery plan every time, it can negatively affect our future delivery plans. There is a significant workload that cannot be handled.
In other words, when we only focus on the customer who is expected to run out of gas that day, the workload occasionally becomes too heavy to finish the delivery.
We propose two methods to tackle this problem, which can be combined into one execution. 
% Former one is that we formulate the integer optimization problem to obtain delivery plans to visit for more than one day.
The former is the formulation of the integer optimization problem to obtain multiple-day delivery target customers.
The second method is to allow deliveries to customers who are not experiencing an emergency but are sufficiently low on gas, i.e., moderate-risk customers, as illustrated in Figure~\ref{fig:aim}.
\begin{figure}
    \centering
    \includegraphics[width=15cm]{other_fig/benefit.png}
    \caption{The benefit of the delivery for high-risk and moderate-risk customers compared to the delivery only for high-risk customer}
    \label{fig:aim}
\end{figure}
In Figure~\ref{fig:aim}, the number of high-risk customers that will occur in a few days can be decreased by visiting moderate-risk customers.
% Figure~\ref{fig:aim} illustrates the benefits that it allows us to delivery to the moderate-risk customer.
%新規性について
% In this paper, we propose an algorithm to develop an efficient LP gas delivery plan in the situation which smart meters are installed in some households. 
% Although delivery planning has been extensively studied as mentioned in the beginning, it differs significantly from existing delivery planning in the following two aspects.
% The first point is that we perform delivery list formulation. 
% In delivery planning for mail delivery or waste collection, a set of delivery destinations is given, and an efficient delivery route is sought under time constraints. 
% In this research, it is necessary to start from the formulation of a list of where gas cylinder deliveries are to be made.
% Second, in order to formulate the list, it is necessary to forecast the remaining quantity of gas cylinders. 
% In order to forecast the amount of gas remaining on a daily basis, we need to build a model to forecast the daily usage of each customer. 
% In particular, there are few examples of demand forecasting in a situation where customers with and with conventional meters are mixed.
% %提案モデルについて
% In this paper, we propose an algorithm to develop an efficient LP gas delivery plan in the situation which smart meters are installed in some households. 
% The basic strategy of the proposed model is to classify customers into essential customers, semi-essential customers, and non-essential customers according to their risk of running out of gas based on the forecasting of remaining cylinder capacity.
% Then, we always deliver to the essential customers and deliver to the semi-essential customers as much as possible to achieve efficient delivery in the long term.
The flow of the proposed model is shown in Figure~\ref{fig:overview} and is composed of three steps.
\\
\begin{enumerate}
\item \textbf{Demand Forecast} (Section~\ref{sec:demand_forecast})\\
The first step is to forecast the daily usage of each customer.
It is initially necessary to obtain daily usages by complementing the missing usage data.
% Only then the daily usage of gas cylinders for each customer can be forecast. 
Machine learning methods, such as support vector regression and random forest regression, are utilized for smart meters.
We propose a forecasting method for conventional meters based on similar usage trends for smart meters based on the k-nearest neighbor method.
% (including customers with smart meters who have to miss for over the last 80 days)
There are some conventional meters whose usage is exceptionally high compared to other consumers.
We use the third quartile to forecast their gas consumption to prevent out-of-gas events.
% For customers with outliers, we use the third quartile to forecast in order to prevent out-of-gas.
\item \textbf{Delivery List Optimization} (Section~\ref{sec:delivery_list})\\
The second step is to determine the target customer to visit.
Based on the inference results and the accuracy of the demand forecast, the risk of a gas shortage for each customer is calculated using the proposed method. 
The customers are classified into high-risk customers, moderate-risk customers, and those not eligible for delivery. 
The number of trucks required to load all high-risk customers and the division of high-risk customers is obtained by an algorithm that improves on the algorithm of the bin packing problem. 
We then propose three methods of list formulation with different motivations, most of which are formulated as integer optimization problems.
\item \textbf{Delivery Route Optimization} (Section~\ref{sec:delivery_route})\\
We solve the vehicle routing problems to obtain the visiting order of the customers to be visited and the estimated arrival time of each customer. 
It is assumed that the shortest distance between customers and the travel time is provided in advance by Mapbox\footnote{\url{https://www.mapbox.com}}. 
In the delivery route optimization, we solve several optimization problems, such as the traveling salesman problem and the maximization of the number of delivery cylinders problem formulated as an integer programming problem. 
In addition, for actual operation, a reasonable but straightforward algorithm is prepared as a post-processing step when no solution is found in the integer programming problem. 
Therefore, a delivery route can be output under any situation, essential for being incorporated in the real worlds scenario.
\end{enumerate}


There are many types of constraints in acquiring the delivery plan, and we divide the problem into several sub-problems, where each constraint is considered at least once, as summarized in Table~\ref{tab:constraint}.

\begin{table}[htbp]
\begin{tabular}{c || c |c|c|c}
&
\multicolumn{3}{c|}{Delivery List Optimization (Section~\ref{sec:delivery_list})}
&
% \begin{tabular}{c}
% \multirow{2}{c}{Delivery Route Optimization}
\multirow{2}{*}{
    \begin{tabular}{c}
        Delivery Route\\ Optimization \\ (Section~\ref{sec:delivery_route})
    \end{tabular}
}
% \end{tabular}  
\\ \cline{1-4}
& \begin{tabular}{c}
Extraction of high-risk / \\ moderate-risk customers \\ (Section~\ref{sec:risk_func})
\end{tabular} & 
\begin{tabular}{c}
Trip division \\ (Section~\ref{sec:divideTrip})
\end{tabular} 
& 
\begin{tabular}{c}
Acquisition of \\ delivery list \\ (Section~\ref{sec:DLmodel})
\end{tabular} 
& 
% \begin{tabular}{c}
% Determine the\\ delivery route
% \end{tabular}  
\\ \hline \hline
\begin{tabular}{c}
The remain gas \\threshold of cylinder
\end{tabular}
& \checkmark    &    &      &    \\ \hline
\begin{tabular}{c}
Truck availability\\ (Weight and Space)
\end{tabular} 
&       & \checkmark     & \checkmark      &      \\ \hline
\begin{tabular}{c}
Staff availability\\ (date information)
\end{tabular}     & \checkmark        &     &       &   \\ \hline
\begin{tabular}{c}
Staff availability\\ (hourly information) 
\end{tabular}    &     &        &       & \checkmark  \\ \hline
\begin{tabular}{c}
Customer availability\\ (date information)
\end{tabular}  & \checkmark    &         &     &     \\ \hline
\begin{tabular}{c}
Customer availability\\ (hourly information) 
\end{tabular} &          &                &    & \checkmark                         
\end{tabular}
\caption{Main constraints of the overall problem and which part is considered in each constraint \label{tab:constraint}}
\end{table}


% Although delivery planning has been extensively studied, it differs significantly from them the necessity of demand forecast and that of acquiring delivery lists.
% In delivery planning for mail delivery or waste collection, a set of delivery destinations is provided. 
% % An efficient delivery route is sought under time constraints. 
% Compared to most vehicle routing research, our algorithm differs from forecasting customers' demand and solving delivery list problems.

% frameworkの汎用性
% The proposed model is a new generic framework to realize an optimal vehicle routing plan to realize long-term optimal delivery plan by setting priority. 
% It is consisted of complement algorithm, demand forecast, delivery list optimization, and delivery route optimization to realize long-term optimal delivery plan by setting priority. 
% Compared to most vehicle routing research, our framework differs significantly from them the necessity of demand forecast and that of acquiring delivery lists.
% Since other industries have similar problems, such as optimizing grocery delivery or oil delivery, our model has a significant potential to solve real-world delivery problems.
Our proposed model is a new generic framework for realizing an optimal vehicle routing plan to realize a long-term optimal delivery plan by setting the priority. 
It consists of a complementary algorithm, demand forecast, delivery list optimization, and delivery route optimization to realize a long-term optimal delivery plan by setting the priority. 
Our framework differs significantly from them the necessity of demand forecast and acquiring delivery lists compared to most vehicle routing studies.
Because other industries have similar problems, such as optimized grocery delivery or oil delivery, our model has a significant potential to solve real-world delivery problems.

%数値実験
% In the numerical experiment, the delivery list and route are optimized for Chiba Prefecture in Japan and evaluated using several indicators. 
% For demand forecast, proposed model achieves better forecast accuracy compared to the conventional models.
% For delivery planning, proposed model succeeds in creating efficient delivery plan as gas provider's does by hand, which records less gas shortage and visits without replacement gas cylinder.
In the numerical experiment, the delivery list and route are optimized for Chiba Prefecture in Japan and evaluated using several indicators. 
For demand forecasting, our proposed model achieves a better forecast accuracy compared to the conventional models.
Our proposed model successfully creates an efficient delivery plan for delivery planning as gas providers plan by hand, recording fewer gas shortages and visits without gas cylinder replacement.
% A decrease in the number of out-of-gas deliveries was confirmed, as well as a decrease in working hours.

%Contribution
We summarize our contribution as follows,
\begin{itemize}
    \item We propose a generic framework to sustain a comfortable mobility service composed of the complementary algorithm, demand forecast, delivery list optimization, and delivery route optimization, which realizes a long-term optimal delivery plan by setting the priority. (Sections~\ref{sec:demand_forecast}-\ref{sec:delivery_route})
    The proposed approach has significant potential for application to other mobility services such as kerosene delivery planning or bike-sharing systems.
    \item We propose a method for formulating a delivery list that considers the delivery area after multiple days (based on daily usage forecasts). 
    It also achieves a more uniform workload distribution. (Sections~\ref{sec:delivery_list},~\ref{sec:delivery_route})
    \item We have developed an algorithm to forecast the daily usage of all customers after complementing various types of missing real data under the situation of different frequencies of data acquisition. (Section~\ref{sec:risk_func})
    \item We propose a new method for extracting customers for delivery when considering the forecast error. A customer with a poorer forecast accuracy can be visited earlier than a customer with better forecast accuracy, despite having almost the same amount of forecast remaining gas. (Section~\ref{sec:demand_forecast})
    \item Numerical experiments are conducted with real gas usage data. (Sections~\ref{sec:exp_dp},~\ref{sec:exp_dldr}) Moreover, we execute the verification experiment for comparison with a delivery plan made by the gas provider by hand. (Section~\ref{sec:field_test})
\end{itemize}

%構成
The remainder of this paper is organized as follows: Section~\ref{sec:related} describes previous related studies.
Section~\ref{sec:problem} demonstrates the daily operations and notations; Sections~\ref{sec:demand_forecast},~\ref{sec:delivery_list}, and~\ref{sec:delivery_route} deal with demand forecasting, delivery list optimization, and delivery route development, respectively.
The numerical experiments of the demand forecast and delivery plan are discussed in Sections~\ref{sec:exp_dp} and~\ref{sec:exp_dldr}, respectively.
Section~\ref{sec:field_test} presents the results of the field test, and Section~\ref{sec:conclusion} provides some concluding remarks regarding this research.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=15cm]{other_fig/overview.png}
    \caption{Overview of proposed framework}
    \label{fig:overview}
\end{figure}



==> history/transportation_research_partC/Problem_Setting/src/1_problem_setting.tex <==
\subsection{Daily Operation}

% 需要家の設定など
This section describes the problem focusing on in this study.
% The number of customers is about 2,800, of which about 900 have smart meters installed.
% The meter reading of a customer with an installed smart meter is sent to the core system at 00:00 each day.
% Customers with a conventional meter have their gas meter read approximately once a month by a gas provider's visit.
Smart meters sent the meter value to the core system at 00:00 every day. 
On the contrary, the meter values of conventional meters are acquired by a gas provider's visit approximately once a month.

% NCUでデータが取れてからの1日の流れ
We describe the flow of the day as being from the time the smart meter is read to the delivery of the gas cylinders.
%We assume that when the meter reading value is obtained by the smart meter, the output route is 5 hours.
Five hours are allowed to make a delivery plan.
Smart meters send us the cumulative meter value at approximately 00:00. 
%We are allowed to make a delivery plan for 5 hours.
% We make a delivery plan in about 5 hours.
%After that, we can get yesterday's gas usages by calculating the difference of two cumulative gas usages.
We can then obtain the gas usage of the day before by calculating the difference between the cumulative gas usage of the day before and that of today.
% We convert it to daily usage and forecast daily usage and all customers' remaining gas for the next week.
Firstly, the complement algorithms are applied to interpolate or extrapolate the gas usage, if needed.
Then, we execute the demand forecast to obtain gas demand in a few days.
% Customers can use a complementary algorithm to simulate daily usage based on gas remaining amount prediction if needed.
Next, the risk level, which is the probability of falling below the remaining gas amount threshold value by the delivery date, is calculated.
Customers are classified into three categories: high-risk customers, moderate-risk customers, and low-risk customers.
Based on the risk level, we formulate the optimization problem to acquire the customer list to deliver the next working day.
The delivery lists are divided into multiple trips owing to the load capacity constraint when there are plenty of customers to be visited.
% In that case, the delivery list will be formulated considering this division.
Finally, we solve the route optimization problem to obtain the order of the visit to customers.
Based on the route optimization results of the current day, the truck drivers load the customer's gas cylinder on tomorrow's first trip before the day is over.
%after the end of today's delivery.
% After delivery on the first trip, the driver loads the gas cylinder on the second trip and delivers the second trip. 
% In this way, today's calculation results will be reflected in tomorrow's delivery.


==> history/transportation_research_partC/Problem_Setting/src/2_notation.tex <==
\subsection{Notation}

This section summarizes the notations used to describe the delivery routing problem to replace a gas cylinder.

First, we define the set of customer and meter as follows,
\begin{itemize}
    \item Set of Meters : $\mathcal{M}$
    \item Set of Customers : $\mathcal{C} \subset 2^{\mathcal{M}}$
    \begin{itemize}
        \item $C \in \mathcal{C}$ is an isolated house $\iff$ $|C| = 1$
        \item $C \in \mathcal{C}$ is an apartment $\iff$ $|C| > 1$
    \end{itemize}

    % \item Set of Apartments : $\mathcal{C}$
    % \item Customer : $C$
    % \item Meter : $M \in C\quad$ ( $|C| = 1 $ if $C$ is an isolated house, $|C| > 1$ if $C$ is an apartment )
    % \item Set of Meters : $\mathcal{M} := \bigcup_{C \in \mathcal{C}}\bigcup_{M \in C}\{M\}$
    \item Location for Customer $C$: $(\rm{lon}^{(C)}, lat^{(C)}) \in \mathbb{R}^2$
    \item Number of Cylinders for Customer $C$ : $\rm{cn^{(C)}}$
    \item Weight of Cylinders for Customer $C$ : $\rm{cw^{(C)}}$
    % \item Travel time : $T^{\rm move} : \mathcal{C} \times \mathcal{C} \to \mathbb{R}$
    % \item repalce time for the gas cylinder :  $T^{\rm ex} : \mathcal{C} \to \mathbb{R} $
    \item Set of dates : $\mathcal{D}$
    \item Obtaining the date moved an integer number of days from the specific date.  $\rm mD : \mathcal{D} \times \mathbb{Z} \to \mathcal{D}$
    \begin{itemize}
        \item Ex1) $\rm mD(30/6/2020,  2) = 2/7/2020$
        \item Ex2) $\rm mD(30/6/2020, -1) = 29/6/2020$
        \item Ex3) $\rm mD(30/6/2020, 0) = 30/6/2020$
    \end{itemize}
    \item Obtaining the difference between two dates $\Delta : \mathcal{D} \times \mathcal{D} \to \mathbb{Z}$
    \begin{itemize}
        \item Ex1) $\Delta(2/7/2020, 30/6/2020) = 2$
        \item Ex2) $\Delta(29/6/2020, 30/6/2020) = -1$
    \end{itemize}
\end{itemize}

By preparing the identity function to indicate whether the smart meter is set, set of smart meters and set of conventional meters can be described as follows,
\begin{itemize}
    \item Set of smart meters : $\mathcal{M}_s  = \{M \in \mathcal{M} | I^{(\rm smart meter)}(M) = 1 \}$
    \item Set of conventional meters : $\mathcal{M}_c  = \{M \in \mathcal{M} | I^{(\rm smart meter)}(M) = 0 \}$
\end{itemize}

\begin{itemize}
    \item Set of Smart Meter which do not have missing data :\\ $\mathcal{M}_s^*  = \{M \in \mathcal{M}_s | I^{(\rm miss)}(M,D) = 0 \ (\forall D \in \mathcal{D}) \}$
\end{itemize}

More definitions are mentioned in each section when needed.

==> history/transportation_research_partC/Problem_Setting/src/3_model_overview.tex <==
% \subsection{Constraints}
% The part for being dealt with is described for each constraint with table~\ref{tab:constraint}.

% \begin{table}[htbp]
% \begin{tabular}{c || c |c|c|c}
% &
% \multicolumn{3}{c|}{Delivery list optimization}
% &
% \begin{tabular}{c}
% Delivery route Optimization
% \end{tabular}  \\ \hline 
% & \begin{tabular}{c}
% Extract high-risk/ \\ moderate-risk customers
% \end{tabular} & 
% \begin{tabular}{c}
% Dividing \\ trips
% \end{tabular} 
% & 
% \begin{tabular}{c}
% Obtain\\ delivery List 
% \end{tabular} 
% & 
% \begin{tabular}{c}
% Determine the\\ delivery route
% \end{tabular}  \\ \hline \hline
% The gas threshold of cylinder   & \checkmark    &    &      &    \\ \hline
% \begin{tabular}{c}
% Truck availability\\ (Weight and Space)
% \end{tabular} 
% &       & \checkmark     & \checkmark      &      \\ \hline
% \begin{tabular}{c}
% Staff availability\\ (date information)
% \end{tabular}     & \checkmark        &     &       &   \\ \hline
% \begin{tabular}{c}
% Staff availability\\ (hourly information) 
% \end{tabular}    &     &        &       & \checkmark  \\ \hline
% \begin{tabular}{c}
% Customer availability\\ (date information)
% \end{tabular}  & \checkmark    &         &     &     \\ \hline
% \begin{tabular}{c}
% Customer availability\\ (hourly information) 
% \end{tabular} &          &                &    & \checkmark                         
% \end{tabular}
% \caption{Constraints \label{tab:constraint}}
% \end{table}

==> history/transportation_research_partC/Problem_Setting/src/ps_main.tex <==
\section{Problem Setting\label{sec:problem}}

\input{3:Problem_Setting/src/1:problem_setting}
\input{3:Problem_Setting/src/2:notation}
\input{3:Problem_Setting/src/3:model_overview}

==> history/transportation_research_partC/Related_work/src/1_demand_forecast.tex <==
\subsection{Gas Consumption Forecasting}
% Forecasting Gas Consumption
Combining the Bernoulli equation and the non-homogeneous Grey model, ~\cite{wu2020novel} studied the natural gas consumption in the United States, Germany, the United Kingdom, China, and Japan, and demonstrated that natural gas consumption will further increase in the future.
In addition,~\cite{farrokhifar2020energy} estimated that global natural gas consumption will increase by approximately 40.% between 2018 and 2050, reaching approximately 58 trillion kWh by 2050.
Therefore, gas consumption forecasting is becoming increasingly important.

Research on gas consumption forecasting has increased in recent years. 
Most studies in this area can be categorized into country-level, city-level, and house-level forecasts by focusing on the data granularity.
Gas consumption forecasting at the country-level began with the Hubbert curve (~\cite{hubbert1949energy, hubbert1956nuclear}),
which forecast the future production rate of fossil fuels based on the annual global consumption.
Herbert (~\cite{herbert1987statistical,herbert1987analysis}) used a regression analysis to forecast monthly and annual natural gas consumption in the US from monthly usage data. 
In addition,~\cite{zhang1998forecasting} compared a forecast from artificial neural networks with statistical methods.
City-level forecasting has also been ongoing.
Moreover,~\cite{karimi2014artificial} published daily gas consumption forecasts in Iranian cities by optimizing the topology of a neural network and its parameters using genetic algorithms. 
In addition,~\cite{liu1991forecasting} used the ARIMA model to forecast monthly and quarterly gas usage in Taiwanese homes from monthly temperature and unit price data.
~\cite{tacspinar2013forecasting} forecast natural gas consumption in Sakarya province in Turkey using the multilayer perceptron of ANNs with a time-series approach from the last 1500 days of usage data to forecast 300 days of usage.
Moreover,~\cite{lu2019short} used a hybrid model that integrates a fruit fly optimization algorithm, simulated annealing algorithm, cross factor, and supports vector machine. The authors forecast the short-term gas load of urban gas in Kunming, China.
House-level forecasting has also recently focused on the spread of smart meters, and
~\cite{parhizkar2021evaluation} forecast hourly energy consumption of buildings in four different climate zones in Iran from monthly electricity and gas data by comparing among five forecast models (linear regression, support vector regression, regression tree, random forest, and K-nearest neighbors).
% \cite{parhizkar2021evaluation} forecast hourly energy consumption of buildings in four different climate zones (cold, mild, warm-dry, and hot-humid) in Iran from monthly electricity and gas data by comparing among five forecast models (linear regression, support vector regression, regression tree, random forest, and K-nearest neighbors).
The best forecast methods are random forest and regression tree approaches, depending on the weather data applied.
Finally,~\cite{de2019forecasting} forecast the natural gas usage of 52 homes in the Netherlands using six methods applying hourly data.
The most accurate hourly forecast was the deep neural network, and multivariate linear regression was applied daily.  
The smart meter enables us to not only forecast gas consumption but also to construct other applications.
For example,~\cite{hurst2019age} proposed a health management system that uses electricity and gas consumption from smart meters to detect people over the age of 65. 
They created a two-class decision tree for remotely monitoring patients with dementia.


==> history/transportation_research_partC/Related_work/src/2_delivery_route.tex <==
\subsection{Optimizing the Delivery Plan}
% TSP
The traveling salesman problem (TSP) aims to find the shortest possible route required to visit each city exactly once and return to the city of origin given a list of cities and the distances between each pair of cities. 
Although the TSP is a fundamental and straightforward problem used in many practical applications~\cite{lenstra1975some}, it is a well-known NP-hard problem~\cite{karp1972reducibility}; hence, various heuristics for the TSP have been proposed~\cite{rego2011traveling}.
Several variants of the TSP for managing real-world application constraints have also been proposed~\cite{feillet2005traveling}. 
In the TSP with a time window (TSPTW)~\cite{dumas1995optimal, solomon1986worst, savelsbergh1985local}, each city must be visited and serviced within a specific time frame. 
If the vehicle arrives at a city too early, it will wait there. 
~\cite{dumas1995optimal} developed an elimination test to significantly reduce the state space and number of state transitions, greatly enhancing the dynamic programming performance used to solve the TSPTW. 
In addition to the time window,~\cite{azi2010exact} considered multiple single-vehicle routes for delivering perishable goods. 
Although the vehicle has the capacity to deliver perishable items, each vehicle route has a deadline for serving a specific customer to preserve the freshness of the goods. 

The authors propose an exact algorithm based on an elementary shortest path algorithm with resource constraints. 
The method first generates feasible routes, and some routes are selected and sequenced to form the entire vehicle route. 
Although the time window for each customer is considered, the start and end time constraints for each route are not.

% VRP
One of the generalizations of the TSP is the vehicle routing problem (VRP) ~\cite{dantzig1959truck}, which considers the following: “What is the optimal set of routes for a fleet of vehicles to traverse in order to deliver to a given set of customers?” 
A VRP with multiple vehicles uses has been addressed in ~\cite{taillard1996vehicle}.
In addition,~\cite{taillard1996vehicle} generates various routes for the classical VRP using a tabu search heuristic. 
The routes obtained are then combined to produce routes with multiple vehicle uses by solving a bin-packing problem. 
Various managerial or legal constraints may impose limited trip duration and customer time window. For example, the customer-requested delivery time, the shippable date of the products, the nature of any perishable goods, the maximum allowed driving hours, and regular disinfection requirements of ambulances in the healthcare field~\cite{cattaruzza2016multi, hernandez2014new, liu2018branch}.
For a multi-trip multi-repairman problem with time windows, ~\cite{liu2018branch} developed a branch-and-price algorithm (B\&P), in which two route-generating approaches were devised to handle the pricing subproblem. 
A traditional study implicitly assumes the constant travel time between two nodes. 
However, this assumption deviates from the actual situation in which travel speeds vary substantially during peak and off-peak hours. Consequently, the routes generated using a traditional time-invariant VRP approach are suboptimal or even infeasible under time-dependent settings. 
~\cite{pan2021multi, truong2021condition, ichoua2003vehicle, gendreau2015time} conducted further research considering the time-dependent travel times to address these issues. 

%Long-term
To realize an optimal long-term delivery plan (~\cite{hernandez2017heuristics, lagana2021dynamic, archetti2015multi, ulmer2018value}), we must determine the delivery target for each day before acquiring the delivery order.
The optimal delivery plan for a single day has the potential to make future delivery plans inefficient.
~\cite{hernandez2017heuristics} studied the tactical delivery plan for large retailers selling and delivering large and heavy items to customers. 
~\cite{hernandez2017heuristics} does not offer customer delivery routes but instead aims to identify discretized time slots and geographical zones where vehicles visit. 
Each zone may be visited multiple times over the planning horizon (e.g., a week), and the possible combination of visit timings is predefined. 
Each ordered pair of zones associates a travel cost and a travel time. 
In this study, the total travel cost is minimized.
~\cite{lagana2021dynamic} modeled a general dynamic multi-period routing problem for postal and courier companies. 
New items arrive at the depots, which are the central hubs where vehicles are based each day. Each item has one of three priority classes:(1) urgent, (2) prominent, and (3) unimportant. 
(1) An urgent item must be quickly delivered, (2) the prominent items must be delivered within two days, and (3) the unimportant items are the other items. 
Given the daily and remaining demand, authors designed daily vehicle routes to minimize the routing cost without future demands. 
The proposed model utilizes a heuristic algorithm based on an adaptive extensive neighborhood search. Moreover, the authors do not consider partial fulfillment to simplify the problem; that is, prominent and unimportant items can be either fulfilled or unfulfilled on the day.
A similar problem was addressed by~\cite{ulmer2018value}, who addressed a dynamic multi-period vehicle routing problem with stochastic service requests. 
Over time, a service provider continuously receives new requests following an available temporal and spatial probability distribution. 
The proposed model decides whether to accept the request for same-day service or defer the request owing to resource limitations. 
To satisfy customer expectations, service providers maximize the total number of accepted same-day requests over all periods. 
The problem was formulated as the Markov decision process. 
A dynamic anticipatory policy was generally solved based on approximate dynamic programming.


==> history/transportation_research_partC/Related_work/src/related_main.tex <==
\section{Related Work\label{sec:related}}

\input{2:Related_work/src/1:demand_forecast}
\input{2:Related_work/src/2:delivery_route}

==> history/transportation_research_partC/abstract.tex <==
\begin{abstract}
This study proposes a method for efficient delivery of liquefied petroleum gas cylinders based on demand forecasts of gas usage.
% Gas is one of the essential resources in our daily lives. 
To maintain a liquefied petroleum gas service, gas providers visit each customer to check the gas meter and replace the gas cylinder depending on the remaining amount of gas.
These visits can be categorized into three patterns: non-replacement visit, replacement before the customer runs out of gas, and replacement after the customer runs out of gas. 
The last pattern is a crucial problem in sustaining a liquefied petroleum gas service, and it must be reduced.
By contrast, frequent non-replacement visits are required to prevent the customer from running out of gas, but it requires considerable effort. 
One of the most severe difficulties of this problem is acquiring the gas usages of each customer only by visiting.
However, with the recent spread of smart sensors, the daily gas consumption of each house can be monitored without having to visit customers.
Such sensors can be utilized to solve the above problems.
Our main idea is to categorize all customers into three groups: high-risk, moderate-risk, and low-risk by focusing on an urgent need for cylinder replacement based on the demand forecast. 
Based on this idea, we construct an algorithm to maximize the delivery for moderate-risk customers while ensuring delivery to high-risk customers. 
Long-term optimal delivery planning is realized by achieving workload balancing per day. 
The verification experiment in Chiba prefecture in Japan showed the effectiveness of our algorithm in reducing the number of out-of-gas cylinders.
Moreover, the proposed model is a new generic framework for building an optimal vehicle routing plan, 
consisting of a complementary algorithm, demand forecast, delivery list optimization, and delivery route optimization for realizing a long-term optimal delivery plan by setting the priority.
The delivery optimization of other areas such as the grocery and oil industries incurs similar problems.
Therefore, our model has significant potential for solving real-world delivery problems.
\end{abstract}

==> history/transportation_research_partC/acknowledgement.tex <==
\section*{Acknowledgement}

This research project is supported by the Japan Science and Technology Agency (JST), the Core Research of Evolutionary Science and Technology (CREST), and JSPS KAKENHI Grant Number JP 16H01707 and 21H04599.
It is also supported by SoftBank Corp. and ISG, Inc..

==> history/transportation_research_partC/requirement.tex <==
\usepackage{mathrsfs}
\usepackage{amsmath}
\usepackage{amsfonts}
% \usepackage[option]{colortbl}
\setcounter{secnumdepth}{5}
\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{theorem}
% \theorembodyfont{\normalfont}
\newtheorem{problem}{Problem}
\newtheorem{prop}{Proposition}
\newtheorem{proof}{Proof}

\usepackage{color}

% \usepackage[dviout]{graphicx}
\usepackage{url}
\usepackage{amssymb}
\usepackage{here}

\newcommand{\dsp}{\displaystyle}

==> titlepage.tex <==
\begin{titlepage}
\section*{Title}
Multi-Period Optimal Delivery Planning for Replacing the Liquefied Petroleum Gas Cylinder with Stochastic Gas Usage Demand\\
\section*{Authors}
\begin{itemize}
    \item Akihiro Yoshida$^\mathrm{a}$, akihiro.yoshida.916@kyudai.jp, Corresponding author
    \item Haruki Sato$^\mathrm{a}$, haruki.sato@kyudai.jp
    \item Shiori Uchiumi$^\mathrm{a}$, uchiumi@kyudai.jp
    \item Nariaki Tateiwa$^\mathrm{a}$, n-tateiwa@kyudai.jp
    \item Daisuke Kataoka$^\mathrm{a}$, kataoka.daisuke@kyudai.jp
    \item Akira Tanaka$^\mathrm{a}$, akirat.tanaka@kyudai.jp
    \item Nozomi Hata$^\mathrm{a}$, n.hata@kyudai.jp
    \item Yousuke Yatsushiro$^\mathrm{a}$, yousuke.yatsushiro@kyudai.jp
    \item Ayano Ide$^\mathrm{a}$, ayano.ide.275@kyudai.jp
    \item Hiroki Ishikura$^\mathrm{a}$, tomomi\_ishikura@kyudai.jp
    \item Shingo Egi$^\mathrm{a}$, egi.shingo@kyudai.jp
    \item Miyu Fujii$^\mathrm{a}$, fujii.miyu.144@kyudai.jp
    \item Hiroki Kai$^\mathrm{a}$, hiroki.kai.815@kyudai.jp
    \item Katsuki Fujisawa$^\mathrm{b}$, fujisawa@imi.kyushu-u.ac.jp
\end{itemize}
\subsection*{Affiliation}
\noindent
$^\mathrm{a}$ Graduate School of Mathematics, Kyushu University, 744 Motooka Nishi-ku Fukuoka, Japan\\
$^\mathrm{b}$ Institute of Mathematics for Industry, Kyushu University, 744 Motooka Nishi-ku Fukuoka, Japan

\section*{Acknowledgement}
This research project is supported by the Japan Science and Technology Agency (JST), the Core Research of Evolutionary Science and Technology (CREST), and JSPS KAKENHI Grant Number JP 16H01707 and 21H04599.
It is also supported by SoftBank Corp. and ISG, Inc..
\end{titlepage}
